Maximum likelihood thresholds via graph rigidity

The maximum likelihood threshold (MLT) of a graph $G$ is the minimum number of samples to almost surely guarantee existence of the maximum likelihood estimate in the corresponding Gaussian graphical model. We give a new characterization of the MLT in terms of rigidity-theoretic properties of $G$ and use this characterization to give new combinatorial lower bounds on the MLT of any graph. We use the new lower bounds to give high-probability guarantees on the maximum likelihood thresholds of sparse Erd{\"o}s-R\'enyi random graphs in terms of their average density. These examples show that the new lower bounds are within a polylog factor of tight, where, on the same graph families, all known lower bounds are trivial. Based on computational experiments made possible by our methods, we conjecture that the MLT of an Erd{\"o}s-R\'enyi random graph is equal to its generic completion rank with high probability. Using structural results on rigid graphs in low dimension, we can prove the conjecture for graphs with MLT at most $4$ and describe the threshold probability for the MLT to switch from $3$ to $4$. We also give a geometric characterization of the MLT of a graph in terms of a new "lifting" problem for frameworks that is interesting in its own right. The lifting perspective yields a new connection between the weak MLT (where the maximum likelihood estimate exists only with positive probability) and the classical Hadwiger-Nelson problem.

==> mlt-aossub.tex <==
%% Packages
\RequirePackage{amsthm,amsmath,amsfonts,amssymb}
\RequirePackage[numbers]{natbib}
%\RequirePackage[authoryear]{natbib} %% uncomment this for author-year bibliography
\RequirePackage[colorlinks,citecolor=blue,urlcolor=blue]{hyperref}
\RequirePackage{graphicx}

\startlocaldefs
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%                                          %%
%% Uncomment next line to change            %%
%% the type of equation numbering           %%
%%                                          %%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\numberwithin{equation}{section}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%                                          %%
%% For Axiom, Claim, Corollary, Hypothezis, %%
%% Lemma, Theorem, Proposition              %%
%% use \theoremstyle{plain}                 %%
%%                                          %%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\theoremstyle{plain}
\newtheorem{thm}{Theorem}[section]
%\newtheorem{lemma}{Lemma}[section]
\newtheorem{lemma}[thm]{Lemma}
\newtheorem{prop}[thm]{Proposition}
\newtheorem{cor}[thm]{Corollary}
\newtheorem{conj}[thm]{Conjecture}
\newtheorem*{claim}{Claim}
\newtheorem*{thm*}{Theorem}
\newtheorem*{lemma*}{Lemma}
\newtheorem*{prop*}{Proposition}
\newtheorem*{cor*}{Corollary}
\newtheorem*{conj*}{Conjecture}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%                                          %%
%% For Assumption, Definition, Example,     %%
%% Notation, Property, Remark, Fact         %%
%% use \theoremstyle{remark}                %%
%%                                          %%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\theoremstyle{remark}
\newtheorem{defn}[thm]{Definition}
\newtheorem*{defn*}{Definition}
\newtheorem{ex}[thm]{Example}
\newtheorem{pr}{Problem}
\newtheorem{alg}[thm]{Algorithm}
\newtheorem{ques}[thm]{Question}
\newtheorem{rmk}[thm]{Remark}
\newtheorem{obs}[thm]{Observation}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Please put your definitions here:        %%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\DeclareMathOperator{\mlt}{mlt}
\DeclareMathOperator{\wmlt}{wmlt}
\DeclareMathOperator{\gcr}{gcr}
\DeclareMathOperator{\grn}{grn}
\DeclareMathOperator{\rignum}{lrn}
\DeclareMathOperator{\rank}{rank}
\DeclareMathOperator{\diag}{diag}
\DeclareMathOperator{\tr}{Trace}
\DeclareMathOperator{\intr}{int}
\DeclareMathOperator{\drigid}{$d$-rigid}
\DeclareMathOperator{\drigidity}{$d$-rigidity}


\newcommand*{\NN}{\mathbb{N}}
\newcommand*{\RR}{\mathbb{R}}
\newcommand*{\QQ}{\mathbb{Q}}
\renewcommand{\SS}{\mathbb{S}}
\newcommand{\p}{\mathbf{p}}
\newcommand{\iprod}[2]{\left\langle {#1}, {#2}\right\rangle}

%packages
\usepackage{optidef}
\usepackage[shortlabels]{enumitem}

%Tikz stuff
\usepackage{tikz}
\tikzstyle{vertex}=[circle, draw, inner sep=0pt,minimum size=6pt, fill=black]
\newcommand{\vertex}{\node[vertex]}
\usetikzlibrary{calc}
\tikzstyle{vertex}=[circle, draw, fill=black, inner sep=0pt, minimum size=4pt]
\tikzstyle{redvertex}=[circle, draw, red, fill=red, inner sep=0pt, minimum size=4pt]
\tikzstyle{bluevertex}=[circle, draw, cyan, fill=cyan, inner sep=0pt, minimum size=4pt]
\tikzstyle{lnode}=[circle,white,draw, inner sep=1pt, font=\scriptsize]
\tikzstyle{edge}=[line width=1pt]
\endlocaldefs

\begin{document}

\begin{frontmatter}
\title{Maximum likelihood thresholds via graph rigidity}
\runtitle{MLT via graph rigidity}

\begin{aug}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%Only one address is permitted per author. %%
%%Only division, organization and e-mail is %%
%%included in the address.                  %%
%%Additional information can be included in %%
%%the Acknowledgments section if necessary. %%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\author[daniel]{\fnms{Daniel Irving} \snm{Bernstein}},
\author[sean]{\fnms{Sean} \snm{Dewar}},
\author[shlomo]{\fnms{Steven J.} \snm{Gortler}},
\author[tony]{\fnms{Anthony} \snm{Nixon}},
\author[meera]{\fnms{Meera} \snm{Sitharam}}
\and
\author[louis]{\fnms{Louis} \snm{Theran}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Addresses                                %%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\address[daniel]{Department of Mathematics,
Tulane University}
\address[sean]{Johann Radon Institute for Computational 
and Applied Mathematics,
Austrian Academy of Sciences}
\address[shlomo]{School of Engineering 
and Applied Sciences,
Harvard University}
\address[tony]{Department of Mathematics and Statistics,
Lancaster University}
\address[meera]{Department of Computer Science,
University of Florida}
\address[louis]{School of Mathematics and Statistics,
University of St Andrews}
\end{aug}

\begin{abstract}
The maximum likelihood threshold (MLT) of a graph $G$ is the minimum number of samples to almost 
surely guarantee existence of the maximum likelihood estimate in the corresponding Gaussian graphical 
model. We give a new characterization of the MLT in terms of rigidity-theoretic properties of 
$G$ and use this characterization to give new combinatorial lower bounds on the MLT of any graph.  
Our bounds, based on global rigidity, generalize existing bounds and are 
considerably sharper.  We  classify the graphs with MLT at most 
three, and compute the MLT of every graph with at most $9$ vertices. 
Additionally, for each $k$ and $n\ge k$, we describe graphs with 
$n$ vertices and MLT $k$, adding substantially to a previously
small list of graphs with known MLT.
We also give a purely geometric characterization of the MLT of a 
graph in terms of a new ``lifting'' problem for frameworks that 
is interesting in its own right.  The lifting perspective 
yields a new connection between the weak MLT (where the maximum likelihood estimate 
exists only with positive probability) and the classical 
Hadwiger-Nelson problem.
\end{abstract}

\begin{keyword}[class=MSC2020]
\kwd[Primary ]{62H12}
\kwd{52C25}
\kwd[; secondary ]{90C25}
\end{keyword}

\begin{keyword}
\kwd{Gaussian graphical models}
\kwd{Number of observations}
\kwd{Maximum likelihood threshold}
\kwd{Combinatorial rigidity}
\kwd{Algebraic statistics}
\end{keyword}

\end{frontmatter}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Please use \tableofcontents for articles %%
%% with 50 pages and more                   %%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\tableofcontents

\section{Introduction}
Modern statistical applications often require researchers to make inferences about a large number of variables from few observations (see e.g.~\cite[Chapter 18]{hastie}).
For example, certain biological network modeling problems, 
including those related to gene regulation~\cite{dobra2004sparse,schafer2005empirical,wu2003interactive} and metabolic 
pathways~\cite{krumsiek2011gaussian},
can be approached by fitting a Gaussian graphical model to a 
dataset that has fewer datapoints than variables.
This invites one to ask the motivating question of this paper, which 
was previously explored by Uhler \cite{uhler2012geometry}, who 
attributes recent interest in it to Lauritzen: 
\emph{given a fixed Gaussian graphical model, 
what is the minimum number of datapoints required to fit it}? 
We now define some terms and state the question more precisely.

Let $G$ be a graph with $n$ vertices.  The Gaussian graphical model
associated with $G$ is the set of $n$-variate normal distributions 
$\mathcal{N}(0,\Sigma)$ so that if $ij$ is \emph{not} an edge of $G$,
then $(\Sigma^{-1})_{ij} = 0$, i.e.~the corresponding 
random variables are conditionally independent
given all of the other random variables.
Suppose now that we have iid samples $X_1, \ldots, X_d$
from a Gaussian graphical model.  
The MLE of the covariance is, then, the inverse of the matrix $K$ that solves the 
following optimization problem (see, e.g., \cite[p. 632]{hastie})
\begin{mini}|l|
   {K}{\tr(SK) - \log \det K}{}{\label{eq: mlt optimization}}
  \addConstraint{K \in \mathcal{S}^n_{++} \ {\rm and} \ K_{ij} = 0 \ {\rm if} \ ij \notin E(G)}
\end{mini}
where $S$ is the sample covariance\footnote{The sample covariance is $S = \frac{1}{d}XX^T$.}
and $\mathcal{S}^n_{++}$ is the set of positive definite $n\times n$ matrices.  
This is a convex problem that can be solved efficiently in practice
\cite{vandenberghe1998determinant}.
Computing the MLE is a common way to fit a Gaussian graphical model to data.
If $d\ge n$ and $G$ is complete then the 
MLE of the covariance is $K = S^{-1}$.  Indeed, almost surely $S^{-1}$
exists and then
\[
    \frac{d}{dK}\left(\tr(SK) - \log \det K\right) = S - K^{-1}
\]
vanishes at $S^{-1}$.  As a warmup for some of the 
ideas in Section \ref{sec: lifting}, now consider the case
of $d < n$ and $G$ complete. Since $S$ has rank at most $d$,
 we can find a non-zero vector $v$ in the kernel of $S$.  For all 
$t\ge 0$, $I + tvv^T$ is positive definite and
\[
    \tr(S(I + tvv^T)) - \log \det (I + tvv^T)\to -\infty
    \qquad \text{(as $t\to\infty$)}
\]
so the MLE of the covariance does not exist.  
If $G$ is not complete, however, the MLE might exist 
even when $d < n$.  This prompts the following definition.

\begin{defn}\label{def: mlt}
The \emph{maximum likelihood threshold} (MLT) of a graph $G$, denoted 
$\mlt(G)$, is the smallest number of samples\footnote{Here, we are assuming that the 
samples are i.i.d.~from a distribution whose probability measure is mutually absolutely 
continuous with respect to Lebesgue measure.} required for the MLE of the 
Gaussian graphical model associated with $G$ to exist almost surely.
\end{defn}

\subsection{Existing bounds on the MLT}
The discussion above implies that $\mlt(K_n) = n$.
For any $G$, 
$1\le \mlt(G)\le n$, since if $H$ is a subgraph of 
$G$, then $\mlt(H) \le \mlt(G)$.
Heuristically, if $G$ is 
very sparse, we could hope that $\mlt(G)$ is much less than $n$.
However, counting edges is not enough to get good bounds, since, 
as we will see, small subgraphs or sparse can push the MLT up.

Ideally, one would like an efficient algorithm to 
compute $\mlt(G)$, but this seems difficult and the complexity 
of computing $\mlt(G)$ remains open.\footnote{It follows from Dempster's work 
\cite{dempster1972covariance} that one can compute $\mlt(G)$ using, e.g., 
cylindrical decomposition of a semi-algebraic set, but the algorithms 
for this task are not fast enough to be of practical interest.}

Instead, the literature, which we now review, focuses on 
finding combinatorial properties that bound the MLT, a 
problem first raised by Dempster \cite{dempster1972covariance}
and, more recently, popularized by 
Lauritzen (see \cite{uhler2012geometry,bendavid}).
The first nontrivial bounds on the MLT are due to 
Buhl \cite{buhl1993existence}.

\begin{thm}[\cite{buhl1993existence}]\label{thm: buhl}
Let $G$ be a graph with clique number $\omega(G)$ and treewidth $\tau(G)$.
Then 
\[
    \omega(G) \le \mlt(G) \le \tau(G) + 1.
\]
\end{thm}
We will see presently that both of these estimates are unsatisfactory:
computing clique number and treewidth are NP-hard problems and 
both inequalities are extremely weak.  As a running example to 
compare inequalties, we will use the complete bipartite 
graph $K_{m,m}$.  Theorem \ref{thm: buhl} implies 
that
\[
    2 = \omega(K_{m,m}) \le \mlt(K_{m,m}) \le \tau(K_{m,m}) + 1 = m+1.
\]

In a landmark paper that introduced maximum-likelihood geometry, 
Uhler \cite{uhler2012geometry} used tools from algebraic 
geometry to bound the MLT.
\begin{defn}\label{def: gcr}
Let $G$ be a graph with $n$ vertices and $m$ edges.  Let 
$\mathcal{S}^{d+1}$ be the set of symmetric matrices of rank 
$d+1$.  The \emph{generic completion rank of $G$}, denoted $\gcr(G)$, 
is the smallest 
$d+1$ so that the orthogonal projection of $\mathcal{S}^{d+1}$
onto the diagonal entries and the entries corresponding 
to the edges of $G$ is $(m + n)$-dimensional.
\end{defn}
\begin{thm}[\cite{uhler2012geometry}]\label{thm: uhler gcr mlt}
Let $G$ be a graph.  Then $\mlt(G)\le \gcr(G)$.
\end{thm}
Uhler formulated the generic completion rank 
in terms of a certain 
elimination ideal being empty, but one can compute
$\gcr(G)$ with a randomized algorithm 
and linear algebra (see \cite{gross2018maximum}).
The upper bound from Theorem~\ref{thm: uhler gcr mlt} is 
very much tighter than the one from Theorem~\ref{thm: buhl}.
It can also be used to extract other combinatorial 
bounds on the MLT.  For example, via~\cite[Corollary~4.5]{BBS-typical}, Uhler's bound implies that if $k$ is the minimum integer such that the $k$-core of $G$ is empty, then $\mlt(G) \le k-1$.

In our running example, we have 
\[
    \mlt(K_{m,m}) \le \gcr(K_{m,m}) = m - 2
\]
(see Theorem \ref{thm: blekherman Kmn} below
for the GCR of $K_{m,m}$).  Thus, on our running 
example, Uhler's bound is better than Buhl's
\emph{and} it is much easier to compute.

For some time, it was open whether, in fact, 
$\mlt(G) = \gcr(G)$ for every graph $G$.
Blekherman and Sinn \cite{blekherman2019maximum} provided
a negative answer as part of a detailed 
study of bipartite graphs.  We will give a more detailed 
account of \cite{blekherman2019maximum}, but here is one summary result.
\begin{thm}[\cite{blekherman2019maximum}]\label{thm: blekherman Kmn}
Let $m, D\in \NN$ so that $m > 2$ and $D$ is largest number 
satisfying $2m > \binom{D+1}{2}$. Then
\[
    \gcr(K_{m,m}) = m\qquad \text{and}
    \qquad
    \mlt(K_{m,m}) = D.
\]
\end{thm}
Comparing with Theorem \ref{thm: buhl}, 
we see that $K_{m,m}$ has clique number $2$ and MLT $\Theta(\sqrt{m})$.  Comparing 
with Theorem \ref{thm: uhler gcr mlt}, 
we see that the upper
bound from generic completion rank is also off by an $O(\sqrt{m})$
factor, making $\gcr(G)$ far from tight as 
an upper bound.

\subsection{MLT and rigidity}
In this paper, we give new lower bounds on the MLT, 
which are more general and sharper than those mentioned above.
Our methods are based on a connection to graph rigidity theory, 
which we briefly introduce.
Figure~\ref{fig:rigidity} illustrates the following definitions for $d=2$.


\begin{defn}\label{def: framework}
Let $d\in \NN$ be a dimension.  A \emph{framework in $\mathbb{R}^d$} is 
a pair $(G,p)$ where $G$ is a graph with $n$ vertices $\{1, \ldots, n\}$ and 
$p = (p(1), \ldots, p(n))$ is a configuration of $n$ points in $\RR^d$.
Two frameworks $(G,p)$ and $(G,q)$ are \emph{equivalent} if 
\[
    \|p(j) - p(i)\| = \|q(j) - q(i)\|\qquad 
    \text{ for all edges $ij$ of $G$}
\]
and \emph{congruent} if $p$ and $q$ are related by a Euclidean isometry,
i.e.~if there exists a Euclidean isometry $T:\mathbb{R}^d\rightarrow\mathbb{R}^d$
such that $q(i)=T(p(i))$ for $i = 1,\dots,n$.
If two frameworks are congruent, then they are also equivalent but the converse need not hold.
Frameworks for which the converse \emph{does} hold are called \emph{globally  rigid} in dimension $d$,
i.e.~$(G,p)$ is globally rigid if all equivalent $d$-dimensional 
frameworks are congruent.
If this happens only for some neighborhood $U$ around $p$,
i.e.~if $(G,p)$ and $(G,q)$ are congruent whenever $q \in U$ and $(G,q)$ and $(G,p)$ are equivalent,
then $(G,p)$ is said to be \emph{rigid} in dimension $d$.
\end{defn}


\begin{figure}[t]
    \centering
        \begin{tikzpicture}
        \vertex (1) at (0,0){};
        \vertex (2) at (1,0){};
        \vertex (3) at (1,1){};
        \vertex (4) at (0,1){};
        \path
            (1) edge (2) edge (4)
            (2) edge (3)
            (3) edge (4)
        ;
        \node at (1.7,1/2){$\leftrightarrow$};
        \vertex (1a) at (0+2.3,0){};
        \vertex (2a) at (1+2.3,0){};
        \vertex (3a) at ($ (3/2+2.3,{sqrt(3)/2}) $){};
        \vertex (4a) at ($ (1/2+2.3,{sqrt(3)/2}) $){};
        \path
            (1a) edge (2a) edge (4a)
            (2a) edge (3a)
            (3a) edge (4a)
        ;      
    \end{tikzpicture}
    \qquad\quad
    \begin{tikzpicture}
        \vertex (1c) at (0,0){};
        \vertex (2c) at (1,0){};
        \vertex (3c) at (.3,.9){};
        \vertex (4c) at (.9,.6){};
        \path
            (1c) edge (2c) edge (3c)
            (2c) edge (3c) edge (4c)
            (3c) edge (4c)
        ;
        \node at (1.7,1/2){$\leftrightarrow$};
        \vertex (1c) at (0+2.3,0){};
        \vertex (2c) at (1+2.3,0){};
        \vertex (3c) at (.3+2.3,.9){};
        \vertex (4c) at (.46+2.3,.3){};
        \path
            (1c) edge (2c) edge (3c)
            (2c) edge (3c)
            (4c) edge (3c) edge (2c)
        ;
    \end{tikzpicture}
    \qquad\quad
    \begin{tikzpicture}
        \vertex (a) at (0,0){};
        \vertex (b) at (1,0){};
        \vertex (c) at (0.5,1){};
        \vertex (d) at (0.5,0.5){};
        \path
            (a) edge (b) edge (c) edge (d)
            (b) edge (c) edge (d)
            (c) edge (d)
        ;
    \end{tikzpicture}
    \caption{Above are some frameworks in $\mathbb{R}^2$. The framework on the left fails to be rigid because there exist arbitrarily close frameworks that are equivalent but not congruent - one can deform it an arbitrarily small amount as indicated. The frameworks in the middle fail to be globally rigid since they are equivalent but not congruent. They are, however, rigid. Indeed, neither can be perturbed an infinitesimally small amount without changing edge lengths. Finally, the framework on the right is globally rigid and therefore also rigid.}
    \label{fig:rigidity}
\end{figure}

On an intuitive level, rigidity of a $d$-dimensional framework $(G,p)$ means that
if one were to physically build $G$ in $\mathbb{R}^d$ using rigid bars for the edges
and universal joints for the vertices, placed according to $p$, then the resulting structure
could not deform.
Rigidity of a specific framework is difficult to check \cite{abbot}, but 
for each dimension $d$, every graph has a generic behavior.
Following \cite{uhler2012geometry,gross2018maximum}, 
we use the following notion of 
generic, which comes from algebraic geometry.
\begin{defn}\label{def: generic}
Let $p$ be a configuration of $n$ points in $\RR^d$.  We 
say that $p$ is \emph{generic} if the coordinates of $p$ do not 
satisfy any polynomial with rational coefficients.
\end{defn}
The following theorem is fundamental in combinatorial or graph rigidity theory.
It tells us that by invoking a genericity assumption, we can treat rigidity and global rigidity
as properties of a graph rather than as properties of a framework.
\begin{thm}[\cite{asimow1978rigidity,gortler2010characterizing}]
Let $d$ be a fixed dimension and $G$ a graph.  Then either 
every generic $d$-dimensional 
framework $(G,p)$ is (globally) rigid or every generic $d$-dimensional framework
$(G,p)$ is not (globally) rigid.
\end{thm}
\begin{defn}\label{def: generic rigid / independent}
Let $d$ be a fixed dimension and $G$ be a graph with $m$ edges.  
We call $G$ \emph{(globally) $d$-rigid} if its generic $d$-dimensional
frameworks are (globally) rigid.  We call $G$ \emph{$d$-independent}
if there is an $m$-dimensional space of differential changes 
to the edge lengths of a (or any) generic framework $(G,p)$.
\end{defn}

In Figure~\ref{fig:rigidity}, the graphs underlying the frameworks in the middle and on the left are $2$-independent, whereas the graph of the framework on the right is not. To see this, note that in frameworks in the middle and left, it is possible to increase or decrease the length of any edge a small amount without changing any other edge lengths.
This is not the case for the framework on the right.

An important fact in rigidity theory is that the  
$d$-independent graphs form the independent sets of a matroid.  Gross and 
Sullivant \cite{gross2018maximum} reformulated Theorem \ref{thm: uhler gcr mlt}
in the language of algebraic matroids (see \cite{MONTHLY} for an
introduction) and proved the following.

\begin{thm}[\cite{gross2018maximum}]\label{thm: gross sullivant}
Let $G$ be a graph.  Then the generic completion rank of 
$G$ is $d+1$ if and only if $d$ is the smallest 
dimension in which $G$ is $d$-independent.
\end{thm}
This result does not improve Uhler's upper bound on the
MLT, but it does open up the possibility 
of employing graph rigidity-theoretic ideas to understand it better.  
An interesting example is:
\begin{thm}[\cite{gross2018maximum}]\label{thm: gross sullivant planar}
If $G$ is a planar graph, then $\mlt(G) \le 4$.
\end{thm}
The proof uses the  Cauchy--Dehn--Alexandrov theorem (see \cite{gluck})
which implies that any planar graph is 
  $3$-independent.
One can immediately deduce the same bound for the slightly wider 
class of $K_5$-minor free graphs using  a result of Nevo \cite{nevo}. 

Graph rigidity theory also makes it easier to compare 
treewidth to the generic completion rank.  
It is well-known that, for $d\ge 2$,
almost every $(d+1)$-regular graph $G$ with $n$ 
vertices has treewidth $\tau(G) > cn$
for some $c > 0$ (see, e.g, \cite{kloks-treewidth}).  
Since, for $d\ge 2$, the only $(d+1)$-regular 
graph that is not $d$-independent is 
$K_{d+2}$ \cite{JJ},
%\footnote{More precisely \cite{JJ} shows that any $(d+1)$-regular $d$-circuit is $d$-rigid and hence we have $\frac{(d+1)|V|}{2}=d|V|-{d+1\choose 2}+1$. Solving, for all $d>1$, gives $|V|=d+2$.}
Theorem~\ref{thm: gross sullivant} implies that
\[
    \gcr(G) \le d + 1  < cn < \tau(G) + 1
\]
for almost every $(d+1)$-regular graph $G$.
This shows just how far away from tight Buhl's upper bound can be.

\subsection{Results and guide to reading}
In this paper, we will 
reformulate the MLT of a graph in terms of equilibrium 
stresses, a graph rigidity theoretic concept that plays an important 
role in global rigidity.
Given vertices $i$ and $j$ of a graph $G$, we write $i\sim j$ to indicate that $G$ has an edge between $i$ and $j$.
\begin{defn}\label{def: eq stress}
Let $G$ be a graph with $n$ vertices.  Let $(G,p)$ be a framework.  An \emph{equilibrium stress}
$\omega$ of $(G,p)$ is 
an assignment of  weights $\omega_{ij}$ to the edges of $G$ so that,
for all vertices $i$
\[
    \sum_{j\sim i} \omega_{ij}(p(j) - p(i)) = 0 \qquad \text{(sum over neighbors of $i$).}
\]
The \emph{equilibrium stress matrix} associated to an equilibrium stress $\omega$ is the 
matrix $\Omega$ obtained by setting $\Omega_{ji} = \Omega_{ij} = -\omega_{ij}$ for all edges $ij$ of $G$,
$\Omega_{ii} = \sum_{j} \omega_{ij}$ and all other entries zero.
The \emph{rank} and \emph{signature} of $\omega$ are defined to be the rank 
and signature of $\Omega$, and $\omega$ is said to be \emph{PSD} if $\Omega$ is positive semi-definite.
\end{defn}
A fact going back to Maxwell \cite{maxwell} is that a 
framework $(G,p)$ in dimension $d$ is independent 
if and only of it has no non-zero equilibrium stress.  
Similarly, a graph is $d$-independent   
if and only if no generic framework $(G,p)$ has a 
non-zero equilibrium stress.

To see the relation with Uhler's bound (Theorem \ref{thm: uhler gcr mlt}), 
we can use Theorem \ref{thm: gross sullivant} and the discussion above
to get the following formulation.
\begin{thm}[\cite{uhler2012geometry,gross2018maximum}]
Let $G$ be a graph with $n$ vertices.  Suppose that no generic framework 
in dimension $d$ supports a non-zero equilibrium stress.  Then the 
MLT of $G$ is at most $d+1$.
\end{thm}
To obtain a lower bound on the MLT, 
we will need to consider the signature of 
the equilibrium stress. Our central new tool will be the following
theorem, proved in Section \ref{sec: lifting}.
\begin{thm}\label{thm: main mlt stress}
Let $G$ be a graph with $n$ vertices. Then the MLT of $G$ is 
$d+1$ if and only if $d$ is the smallest dimension in which 
no generic $d$-dimensional framework supports non-zero 
PSD equilibrium stress.
\end{thm}
This technical theorem along with some known 
graph rigidity-theoretic results and arguments will allow us to 
significantly expand our understanding of the MLT (as well as 
directly reproduce most of what is already understood).

To return to our running example, Theorem \ref{thm: blekherman Kmn}
implies that $K_{m,m}$ generically supports equilibrium stresses
in dimension $m-2$, but that they are all indefinite.  In 
Section \ref{sec: complete bipartite}, we will re-derive 
Theorem \ref{thm: blekherman Kmn} by first understanding 
their equilibrium stresses.

There is a geometric counterpart to Theorem \ref{thm: main mlt stress}, originally conjectured by Gross and Sullivant \cite{gross2018maximum}.
A $d$-dimensional framework $(G,p)$ \emph{has full affine span} if 
$p
$ affinely spans $\mathbb{R}^d$.
\begin{thm}\label{thm: main mlt lift}
Let $G$ be a graph with $n$ vertices. Then the MLT of $G$ is 
$d+1$ if and only if $d$ is the smallest dimension in which 
every generic $d$-dimensional framework $(G,p)$
is equivalent to an $(n-1)$-dimensional framework 
$(G,\tilde{p})$ with full affine span.
\end{thm}

\begin{figure}[t]
    \centering
    \begin{tikzpicture}
        \node at (0,0.5){};
        \draw[gray,dashed] (-0.5,0)--(2,0);
        \vertex (1b) at (0,0){};
        \vertex (2b) at (0.5,0){};
        \vertex (3b) at (1,0){};
        \vertex (4b) at (1.5,0){};
        \path
            (1b) edge[bend left = 40] (3b)
            (2b) edge[bend right = 40] (4b)
            (3b) edge (4b)
            (1b) edge (2b)
        ;
        \node at (2.5,0){$\leftrightarrow$};
        \vertex (1a) at (0+3.2,0){};
        \vertex (2a) at (1+3.2,0){};
        \vertex (3a) at ($ (3/2+3.2,{0.5*sqrt(3)/2}) $){};
        \vertex (4a) at ($ (1/2+3.2,{0.5*sqrt(3)/2}) $){};
        \path
            (1a) edge (2a) edge (4a)
            (2a) edge (3a)
            (3a) edge (4a)
        ;
    \end{tikzpicture}
    \qquad
    \begin{tikzpicture}
        \node at (0,0.5){};
        \vertex (1a) at (0,0){};
        \vertex (2a) at (0.5,0){};
        \vertex (3a) at (1,0){};
        \vertex (4a) at (1.5,0){};
        \path
            (1a) edge (2a)
            (2a) edge (3a)
            (3a) edge (4a)
            (1a) edge[bend left=40] (4a)
        ;
    \end{tikzpicture}
    \qquad
    \begin{tikzpicture}
        \node at (0,0.5){};
        \vertex (1a) at (0,0){};
        \vertex (2a) at (0.5,0){};
        \vertex (3a) at (1,0){};
        \vertex (4a) at (1.5,0){};
        \path
            (1a) edge (2a)
            (2a) edge (3a)
            (3a) edge (4a)
        ;
        \node at (2.25,0){$\leftrightarrow$};
        \vertex (1a) at (3+0,0){};
        \vertex (2a) at (3+0.5,0){};
        \vertex (3a) at (3+1,0){};
        \vertex (4a) at (3+1,0.5){};
        \path
            (1a) edge (2a)
            (2a) edge (3a)
            (3a) edge (4a)
        ;
    \end{tikzpicture}
    \caption{The framework in $\mathbb{R}^1$ on the left is equivalent to a framework in $\mathbb{R}^3$ with full-dimensional affine span. To see this, first note that it is equivalent to the framework in $\mathbb{R}^2$ to the right of it. Then note that this two-dimensional framework is equivalent to a framework in $\mathbb{R}^3$ with full-dimensional affine span since we can lift one of the vertices into the third dimension without changing edge-lengths. However, the maximum likelihood threshold of the underlying graph, the four-cycle, is \emph{not} two since every framework equivalent to the framework in the middle has a one-dimensional affine span.
    On the other hand, the path with four vertices has an MLT of $2$ because any generic one-dimensional framework on it can be folded out to three dimensions. On the right, we see such a one-dimensional framework folding out into two dimensions. We can further fold it into three by bringing the vertex on the left out of the affine plane spanned by the other vertices.
    }
    \label{fig: lifting}
\end{figure}

See Figure~\ref{fig: lifting} for an illustration of Theorem~\ref{thm: main mlt lift}.


There is a link between  globally
rigid graphs and PSD equilibrium stresses, established 
in \cite{cgt1}.  This will allow us to obtain bounds on the
MLT using global rigidity.
To this end we define a new graph parameter.
\begin{defn}\label{def: grn}
    The \emph{global rigidity number} of $G$, denoted $\grn(G)$, is the maximum $d$ such that $G$ is globally $d$-rigid and has at least
    $d+2$ vertices.
    The \emph{globally rigid subgraph number} of $G$, denoted $\grn^*(G)$ is the maximum $d$ so that $G$ contains a subgraph $H$ on at least $d+2$ vertices that 
    is   globally rigid.
\end{defn}
We obtain the following new lower bound on the MLT of a 
graph.
\begin{thm}\label{thm: grn mlt}
Let $G$ be a graph.  Then $\grn(G) + 2\le\grn^*(G) + 2\le \mlt(G)$.
\end{thm}
Since complete graphs are globally $d$-rigid for all $d$, Theorem \ref{thm: grn mlt} generalizes the lower 
bound of Theorem \ref{thm: buhl}.  
To our knowledge, this is the 
first unconditional improvement of Buhl's lower bound  
from 1993 (Theorem \ref{thm: buhl}).

In our running example of $K_{m,m}$, the 
lower bound from Theorem \ref{thm: grn mlt} 
gives the right answer: by Theorem \ref{thm: blekherman Kmn},
$\mlt(K_{m,m}) = \grn(K_{m,m}) + 2$.

The families of graphs for which the MLT has 
been computed exactly are quite limited in the 
literature.  
As mentioned above, Buhl \cite{buhl1993existence}
computes $\mlt(K_{d+2}) = d + 1$ and Bleckhermann and Sinn 
\cite{blekherman2019maximum} compute $\mlt(K_{m,n})$ (see 
Section \ref{sec: complete bipartite}).  Uhler \cite{uhler2012geometry}
provides, in addition, that the MLT of a cycle is $2$.
As an application of Theorem \ref{thm: grn mlt}, 
to this short list, we add infinitely many examples 
for every value of the MLT in Section~\ref{sec: mlt gr}.
All of them arise from a common generalization of trees and cycles, which are examples of 
``minimally rigid graphs'' and ``globally rigid circuits''respectively in the 1-dimensional rigidity matroid.
Section~\ref{sec: mlt gr} also develops the proof of Theorem 
\ref{thm: grn mlt} and direct consequences.
The  technical tools we use, from 
\cite{alfakih2011bar} and \cite{cgt1}, arose in the 
study of universal rigidity.
In Section \ref{sec: mlt 3}, we combine Theorem \ref{thm: grn mlt}
with results on graph rigidity in dimension $2$ to completely
solve the MLT problem for small values of $\mlt(G)$ and $\gcr(G)$.
The main result (which is best possible -- see Remark~\ref{rmk: best possible}) is as follows.
\begin{thm}\label{thm: equality of gcr and mlt}
If $G$ is a graph and $\mlt(G) \le 3$ or $\gcr(G) \le 4$, then $\mlt(G) = \gcr(G)$.
\end{thm}

Theorem \ref{thm: grn mlt} is also strong enough to give a 
quick proof of the results in \cite{blekherman2019maximum}.
Section \ref{sec: complete bipartite} explores the connection.
We can also show that the Blekherman--Sinn example of $K_{5,5}$
is the smallest possible graph where the MLT and GCR do not 
coincide. This is done in Section~\ref{sec: many / few}, as 
a corollary of the following.
\begin{thm}\label{THM:SMALL}
	For any graph $G=(V,E)$ with $n \leq 9$ vertices,
	we have $\mlt(G) = \gcr(G)$.
\end{thm}

We conclude in Section~\ref{sec: weak MLT} with some comments and conjectures on the 
weak maximum likelihood threshold.

\section{Stress geometry of the MLT}\label{sec: lifting}
In this section we develop a detailed geometric understanding
of the MLT.  Our main tool for doing this is the theory 
of PSD equilibrium stresses of frameworks. The 
importance of PSD equilibrium stresses has long 
been known in rigidity \cite{c1} 
and graph theory \cite{tutte-howtodraw,LLW}.
Uhler \cite{uhler2012geometry} has pointed out the 
semi-algebraic nature of the MLT problem.  Here we make 
the connection precise enough to exactly describe the MLT
in terms of equilibrium stresses.

\subsection{Linear equilibrium stresses}
To connect to the optimization problem underlying the 
MLT, we introduce the notion of a linear equilibrium 
stress, which is implicit in a number of works around 
rigidity in geometries with projective models (see
\cite{NW-metricchange} and the references therein).
We start with some notation relating to vector configurations.

\begin{defn}\label{def: flattenable}
Let $q$ be a configuration of $n$ vectors in $\RR^{d+1}$.
Denote by $t_i$ the last coordinate of $q(i)$ and by $Q$
the $(d+1)\times n$ matrix with the $q(i)$ as its columns.
We say that $q$ is \emph{flat} if all the $t_i$ are one, 
and that $q$ is \emph{flattenable} if all the $t_i$ 
are non-zero.
\end{defn}
Generic configurations are clearly flattenable.
There is a unique flat configuration associated 
with a flattenable configuration $q$ arising from scaling 
$q(i)$ by $1/t_i$.
Flat vector configurations in $\mathbb{R}^{d+1}$ are naturally associated with 
affine point configurations in $\mathbb{R}^d$.

\begin{defn}\label{def: std lifting}
Let $p$ be a configuration of $n$ points in $\RR^d$.
We denote by $\hat p$, the vector configuration 
in $\RR^{d+1}$ defined by the standard homogeneous 
coordinates for $p$, i.e.
\[
    \hat p(i) = \begin{pmatrix} p \\ 1\end{pmatrix}.
\]
The matrix $\hat P$ is $(d+1)\times n$ with the 
vectors $\hat p(i)$ as its columns.
\end{defn}


\begin{defn}\label{def: linear stress}
Let $d$ be a dimension. Let $G$ be a graph with $n$ vertices and 
let $q$ be a vector configuration of $n$ 
vectors in $\RR^{d+1}$.
An assignment $\omega$ of weights $\omega_{ij}$ to the 
edges $ij$ of $G$ and $\omega_{ii}$ to the vertices 
of $G$ is a \emph{linear equilibrium stress}
for $q$ if 
\begin{equation}\label{eq:linearStress}
   \sum_{j\sim i} \omega_{ij}q(j) = \omega_{ii}q(i) 
    \qquad 
    \text{(all $i\in V(G)$).}
\end{equation}
For a fixed $\omega$, we say that
\emph{$q$ satisfies $\omega$} if \eqref{eq:linearStress} holds.
A \emph{linear equilibrium stress matrix} $\Omega$ for
$q$ is a symmetric $n$-by-$n$ matrix with
$\Omega_{ij} = 0$ for non-edges of $G$ such that
\[
    \Omega  Q^T = 0,
\]
where $Q$ is the $(d+1)\times n$ matrix with the 
$q(i)$ as its columns.
Given a linear equilibrium stress $\omega$ for $q$,
we can
make a linear equilibrium stress matrix for it
by setting $\Omega_{ij}=\Omega_{ji}=-\omega_{ij}$
on the edges
and setting the diagonals $\Omega_{ii}=\omega_{ii}$.
Hence the vector configurations satisfying a given set of 
weights arise from the kernel of the associated linear 
equilibrium stress matrix.
\end{defn}

The following lemma is immediate. It gives the precise relationship between equilibrium stresses and \emph{linear} equilibrium stresses.

\begin{lemma}\label{lem: affine to linear stress}
Let $G$ be a graph with $n$ vertices and let $(G,p)$
be a $d$-dimensional framework.  Then for any 
equilibrium stress $\omega$ of $(G,p)$, the 
associated stress matrix gives a linear equilibrium 
stress of $\hat p$.  Any linear equilibrium stress 
matrix $\Omega$ for $\hat p$ is also an equilibrium 
stress matrix for $(G,p)$.
\end{lemma}

Linear equilibrium stresses are well-behaved 
under scaling. Results similar to the following can be 
found in e.g.~\cite{cgt2,connelly2010global}.

\begin{lemma}\label{lem: linear stress scale}
Let $G$ be a graph with $n$ vertices and let $q$ be a vector configuration in $\RR^{d+1}$.  If $\Omega$
is a linear equilibrium stress matrix for $q$
and $s_1, \ldots, s_n$ are any non-zero real 
numbers, then the configuration $\tilde q$, defined
by 
\[
    \tilde q(i) = \frac{1}{s_i}q(i)
\]
has a linear equilibrium stress matrix with the 
same signature as $\Omega$.
\end{lemma}

\begin{proof}
Take $q$ and the $s_i$ as in the statement, and let 
$\omega$ be the linear equilibrium stress for $q$
from the statement. For each vertex $i$ and edge $ij$, define
\[
    \tilde\omega_{ij} = s_i s_j \omega_{ij}
    \qquad 
    \text{and}
    \qquad 
    \tilde\omega_{ii} = s^2_i\omega_{ii}.
\]
Then $\tilde\omega$ is a linear equilibrium stress for $\tilde{q}$ because for each vertex $i$ we have
\[
    \sum_{j\sim i} \tilde\omega_{ij}\tilde q(j) 
    = s_i  \sum_{j\sim i} \omega_{ij}q(j)
    = s_i \omega_{ii}q(i) = s_i^2 \omega_{ii}\tilde q(i)
    = \tilde\omega_{ii} q(i).
\]
Let $\tilde{\Omega}$ be the stress matrix associated to $\omega$
and let $S$ be the diagonal matrix whose diagonal entries are $s_1,\dots,s_n$.
Then $\tilde{\Omega}=S\Omega S$ and thus $\Omega$ and $\tilde{\Omega}$ have the same signature.
\end{proof}

We get an important special case when $s_i$ is the last coordinate of $q(i)$ for each $i$.

\begin{lemma}\label{lem: flattening stress}
Let $G$ be a graph with $n$ vertices, let $q$ be a
flattenable configuration of $n$ vectors in $\RR^{d+1}$, and let 
$(G,p)$ be the framework in $\RR^d$ that arises from 
flattening $q$ and deleting the all-ones coordinate.
If there is a linear equilibrium stress matrix $\Omega$
for $q$, then $p$ has an equilibrium stress matrix of the same signature as $\Omega$.
\end{lemma}

\begin{proof}
If we denote by $\hat p$ the flattening of $q$, then 
by Lemma \ref{lem: linear stress scale}
there is a linear equilibrium stress for $\hat p$ with 
the same signature as $\Omega$.  This stress is
an equilibrium stress of $(G,p)$ by Lemma 
\ref{lem: affine to linear stress}.
\end{proof}

\subsection{The optimization problem}
We now describe the MLT optimization problem.  For convenience, 
we write the inner product $\tr(AB)$ on the set of symmetric $n\times n$
matrices using the standard notation $\iprod{A}{B}$. 
\begin{defn}\label{def: opt problem}
Let $G$ be a graph with $n$ vertices.  
Let $D$ be an $n\times (d+1)$ matrix with columns representing
$(d+1)$ samples from an $n$-variate probability distribution.
Let $S = \frac{1}{d}DD^T$ be the sample covariance matrix.
\emph{The MLT optimization problem for $(G,D)$} is to find an $n\times n$ 
positive definite matrix $K$
minimizing $f(K) = \iprod{S}{K} - \log \det K$, 
subject to $K_{ij} = 0$ for all $ij\notin E(G)$.
\end{defn}

The rigidity-theoretic viewpoint requires us to transpose our view of the data matrix. In particular, instead of thinking about $S$ as the sample covariance obtained from $(d+1)$ samples of an $n$-variate distribution, we will think about $S$ as the Gram matrix of a configuration of $n$ points in $(d+1)$-dimensional space.
This allows us to recast the MLT optimization problem in the following equivalent way.

\begin{defn}\label{def: modified opt problem}
Let $G$ be a graph with $n$ vertices and let 
$q$ be a configuration of $n$ vectors in dimension $d+1$.
Let $S = Q^T Q$ be the Gram matrix of $q$.
\emph{The Gram MLT optimization problem for $(G,q)$} is to find an 
$n\times n$ positive definite matrix 
$K$, minimizing $g(K) = \iprod{S}{K} - \log \det K$, subject to 
$K_{ij} = 0$ if $ij\notin E(G)$.
\end{defn}

\begin{lemma}\label{lem: unbounded iff stress}
Let $G$ be a graph with $n$ vertices and let $q$ 
be a configuration of $n$ vectors.
Then the Gram MLT optimization problem (objective function $g$) is unbounded if and only if
there is a nonzero PSD linear equilibrium stress for $q$.
\end{lemma}
\begin{proof}
Let $S$ be the Gram matrix of $q$.  Suppose that 
$\Omega$ is the PSD stress matrix of a non-zero 
linear equilibrium stress for $q$. 
For any $t > 0$, the matrix $I + t\Omega$ is positive definite and
\[
    g(I + t\Omega) = \iprod{S}{I + t\Omega} - \log \det (I + t\Omega).
\]
Since 
\[
    \iprod{S}{I + t\Omega} = \iprod{S}{I} + t\iprod{S}{\Omega}
    = \iprod{S}{I} + t\tr{Q^T Q\Omega} = 
    \iprod{S}{I} + t\tr{Q^T 0} = \iprod{S}{I}
\]
we conclude that 
\[
    g(I + t\Omega) = \tr{S} - \log \det(I + t\Omega) \to -\infty
    \qquad \text{(as $t\to \infty$)}.
\]
So the optimization problem is unbounded.

For the other direction we prove the contrapositive.
Suppose that there is no non-zero 
PSD linear equilibrium stress matrix for 
$q$. We show that the gram MLT optimization problem has a global minimum. Let $\SS$ be be the set of symmetric 
$n\times n$ matrices $\Omega$ with zeros on the non-edges 
of $G$ satisfying $\iprod{\Omega}{\Omega} = 1$. 
For any $\Omega\in \SS$, there is a $t_0 > 0$
so that $K = I + t_0\Omega$ is a feasible point of the 
Gram MLT optimization problem.  Define $t^* \ge t_0 > 0$ to be 
the supremum over values such that $I + t\Omega$ 
is positive definite. 
We will show that, for any 
$\Omega\in \SS$, 
\[
    g(I + t\Omega)\to \infty \qquad \text{(as $t\to t^*$).}
\]
It then follows that, outside of a compact neighborhood of $I$, 
$g(I + t\Omega) > g(I)$, which implies that $g$ has a 
global minimum.
There are two cases.  If $\Omega\in \SS$ is not
PSD, then $t^*$ is finite, and, as $t\to t^*$, 
\[
    g(I + t\Omega) =\tr S + t\iprod{S}{\Omega} - \log \det(I + t\Omega)\to \infty, 
\]
since the last term grows without bound and the linear terms 
have bounded magnitude.  
If $\Omega$ is PSD, then $I + t\Omega$ is positive 
definite for any $t > 0$, and so $t^* = \infty$.
We then have, as $t\to \infty$,
\[
    g(I + t\Omega) = \tr S + t\iprod{S}{\Omega} - 
        \log \det(I + t\Omega) = 
        \tr S + t\iprod{S}{\Omega} - O(\log t)
\]
because the determinant is a polynomial of degree $n$ in
$t$.  Finally, since $S$ and $\Omega$ are 
PSD and $\Omega$ is not a linear equilibrium stress matrix,
$\iprod{S}{\Omega} > 0$, so 
\[
    g(I + t\Omega) \to \infty \qquad 
    \text{(as $t\to \infty$)}.\qedhere
\]
\end{proof}

\subsection{Proof of Theorem \ref{thm: main mlt stress}}
We are now ready to prove Theorem~\ref{thm: main mlt stress}.
Lemmas \ref{lem: main stress forward} and \ref{lem: main stress backwards} below each give one direction. What is left is to rigorously establish the relationship between ``almost all'' and 
generic. The most technical statements are 
handled in Appendix~\ref{appendix: generic}.
Recall that two measures are \emph{mutually absolutely continuous}
if they have the same null sets.

\begin{lemma}\label{lem: main stress forward}
Let $G$ be a graph with $\mlt(G) = d+1$. Then:
\begin{enumerate}[(a)]
    \item there is a generic framework $(G,p)$ in $\mathbb{R}^{d-1}$ with a nonzero PSD equilibrium stress, and
    \item no generic framework $(G,p)$ in $\mathbb{R}^d$ has a nonzero 
    PSD equilibrium stress.
\end{enumerate}
\end{lemma}

\begin{proof}
Let $n$ be the number of vertices of $G$.
Let $D$ be an $n\times d$ data matrix whose columns are i.i.d.~samples from a distribution whose probability measure $\mu$ is mutually absolutely continuous with respect to the Lebesgue measure.
Let $q$ denote the configuration of $n$ points in $\mathbb{R}^d$ given by the rows of $D$.
Since $\mlt(G) = d+1$, the Gram MLT optimization problem for $(G,q)$ is unbounded with positive probability.
Let $X$ denote the set of vector configurations of $n$ points in $\mathbb{R}^d$
for which the Gram MLT optimization problem is unbounded.
Then $X$ is semi-algebraic and not $\mu$-null,
so Lemma~\ref{lem: semi-alg generic} implies that $X$ contains a generic vector configuration, 
which we continue to call $q$.
By Lemma \ref{lem: unbounded iff stress},
there is a non-zero PSD linear equilibrium stress matrix $\Omega$ for $q$.
Since $q$ is generic, it is flattenable.
By Lemma \ref{lem: flattening stress}, the $(d-1)$-dimensional 
framework $(G,p)$ arising from flattening $q$ has an
equilibrium stress matrix with the same signature as $\Omega$,
so this matrix must also be PSD and non-zero.
Finally, Lemma \ref{lem: gen slicing} implies that 
$p$ is generic.
Hence we have constructed a generic $d-1$-dimensional framework $(G,p)$ with a non-zero PSD equilibrium stress.


Let $W$ denote the set of configurations $w$ of $n$ points in $\mathbb{R}^{d+1}$ for which the Gram MLT optimization problem $(G,w)$ is bounded.
Since $\mlt(G) = d+1$, the complement of $W$ is $\mu$-null.
Let $(G,p)$ be a generic framework in $\mathbb{R}^d$.
Scaling the vectors of $\hat p$ by generic weights
gives, via Lemma~\ref{lem: gen slicing}, a generic  configuration $w$ in $\RR^{d+1}$.  
Since $W$ is semi-algebraic and $w$ is generic,
Lemma~\ref{lem: semi-alg generic} implies $w\in W$.
By Lemma~\ref{lem: unbounded iff stress},
there is no non-zero PSD linear equilibrium stress
for $(G,w)$.  By Lemma~\ref{lem: flattening stress},
there is no non-zero PSD equilibrium stress for $(G,p)$.
\end{proof}

\begin{lemma}\label{lem: main stress backwards}
Let $G$ be a graph with $n$ vertices and suppose that $d$
is the smallest dimension so that no generic 
$d$-dimensional framework $(G,p)$ has a non-zero
PSD equilibrium stress.  Then the MLT of $G$ is $d+1$.
\end{lemma}
\begin{proof}
By assumption, there must be
a generic $(d-1)$-dimensional framework 
with a non-zero PSD equilibrium stress, which we will call
$(G,p)$.
By scaling 
the vectors of $\hat p$ by generic numbers $s_i$, 
we obtain, by Lemma \ref{lem: gen slicing}, 
a generic vector configuration $q$ in 
dimension $d$.  By Lemma \ref{lem: flattening stress},
there must be a non-zero PSD linear equilibrium stress for $q$.
Hence, by Lemmas~\ref{lem: unbounded iff stress} and~\ref{lem: semi-alg generic}, the 
set of configurations for which the Gram MLT optimization problem is 
unbounded must be non-null.  We conclude that $\mlt(G) > d$.

Now we take a generic vector configuration $q$ in 
dimension $d+1$.  As noted above, by genericity, $q$
is flattenable, and the flattened $d$-dimensional
point configuration $p$ is also generic by 
Lemma \ref{lem: gen slicing}.  By Lemma \ref{lem: flattening stress}, since $(G,p)$ does not have a non-zero PSD equilibrium 
stress, there is not a non-zero PSD linear equilibrium 
stress for $q$.  Hence, for every generic vector configuration 
$q$ in dimension $d+1$, the Gram MLT optimization problem is bounded by Lemma~\ref{lem: unbounded iff stress}.
Since the set of all such vector configurations is semi-algebraic and contains all the generic points, 
it must have full measure by Lemma \ref{lem: semi-alg generic}.  
This implies that $\mlt(G)\le d+1$.
\end{proof}
The existence of a generic framework in dimension $d-1$
with a non-zero PSD equilibrium stress implies that the 
Gram MLT optimization problem is unbounded with positive probability.  However, we don't have a lower bound on
this probability.  Any general 
lower bound will be quite bad, since 
Buhl \cite{buhl1993existence} showed that, for $G$ an
$n$ cycle, the MLE exists after $2$ sample points with 
probability $1 - 2n/n!$ (although the MLT of a cycle is $3$).

\subsection{The geometric picture: lifting}
Theorem \ref{thm: main mlt stress}, while precise, and 
as we will see, convenient for deriving bounds on 
the MLT of a graph, is quite technical.  There is 
an underlying geometric idea, that we now 
explain.

\begin{defn}\label{def: liftable}
Let $G$ have $n$ vertices.  Let $(G,p)$ be a 
$d$-dimensional framework.  We say that 
$(G,p)$ is \emph{liftable} if there is an equivalent
$n-1$ dimensional framework $(G,\tilde{p})$
with full affine span.
\end{defn}

The following Lemma is due to Alfakih~\cite{alfakih2011bar}.
For completeness, we provide a proof in the appendix that uses 
convex geometry ideas from \cite{gt1}.

\begin{lemma}[\cite{alfakih2011bar}]\label{lem: psd lift}
A $d$-dimensional framework $(G,p)$ is liftable if and only if 
it does not have a non-zero PSD equilibrium stress.
\end{lemma}

Theorem \ref{thm: main mlt lift} is immediate 
from Theorem \ref{thm: main mlt stress} and 
Lemma \ref{lem: psd lift}.

\subsection{Remarks}
To close a circle of ideas, we note that much of the
literature on the MLT, including \cite{uhler2012geometry,gross2018maximum,bendavid,blekherman2019maximum}
does not work directly with the MLT optimization problem.
Instead, the starting point is the following matrix 
completion problem.
\begin{defn}\label{def: mlt matcomp}
Let $G$ be a graph with $n$ vertices and $S$ an 
$n\times n$ PSD matrix of rank $d+1$.
The \emph{MLT matrix completion problem for $(G,S)$} is to find an $n\times n$ 
positive definite matrix $A$ that has the same diagonal entries as 
$A$ and the same off diagonal entries corresponding to edges of $G$.
\end{defn}
Dempster \cite{dempster1972covariance}
showed that the MLT optmization problem is 
bounded if and only if the MLT matrix completion 
problem is feasible.\footnote{One can also derive Dempster's result via convex duality, see e.g.~\cite{bendavid}.}
A less direct path to our results is to relate the 
MLT matrix completion for $G$ problem to liftability 
of ``coned'' frameworks $(v_0*G,p)$ in one dimension 
higher that have a new vertex $v_0$ connected to 
all the others (see, e.g., \cite{W83,connelly2010global}, for 
details about  coning).

Finally, we note that we could have allowed the vector configurations in our optimization problems to satisfy a condition strictly weaker than flattenability.
In particular, it would have been enough to only require that the Gram 
matrix $Q^T Q$ have \emph{some} factorization that 
is flattenable, which happens so long as none 
of the vectors in $q$ are zero.  
At the level of frameworks, changing 
factorizations corresponds to projective transformations.
We elected to use the stronger condition to keep the proofs
simpler, and in particular, to avoid
having to define and work with generic low-rank PSD matrices.





% \subsection{Older stuff}
% % \begin{defn}\label{defn: linear stress}
% %     Given $d \le n$, a graph $G$, and an $n\times d$ matrix $X$, a \emph{linear $G$-stress of $X$} is a symmetric matrix $\Omega$ with $\Omega_{ij} = 0$ for all non-edges $ij$ of $G$ such that $\Omega X = 0$.
% % \end{defn}

% \begin{lemma}\label{lemma: infeasible iff linear psd stress}
%     Let $G$ be a graph and let $X$ be an $n\times d$ matrix.
%     The corresponding MLE optimization problem~\eqref{eq: mlt optimization} with $S = XX^T$ is unbounded below if and only if there exists a non-zero PSD linear $G$-stress of $X$.
% \end{lemma}
% \begin{proof}
%     First assume that a PSD linear $G$-stress $\Omega$ exists.
%     Then $I + t\Omega$ is feasible for all $t$. Moreover, the value of the objective function evaluated at $I + t\Omega$ diverges to $-\infty$ as $t\rightarrow \infty$.
%     Now assume that \eqref{eq: mlt optimization} is unbounded below.
%     Let $\mathcal{O}_G$ denote the set of matrices $\Omega$ satisfying $\tr(\Omega\Omega) = 1$ and $\Omega_{ij} = 0$ for all non-edges of $G$.
%     For each $\Omega \in \mathcal{O}_G$, define $t_\Omega$ to be the optimal value of the following optimization problem, which could be $-\infty$
%     \begin{mini*}|l|
%     {t\ge 0}{\tr(S(I+t\Omega)) - \log \det (I+t\Omega)}{}{\label{eq: mlt on a ray}}
%     \addConstraint{I + t\Omega \in \mathcal{S}^n_{++}}.
%     \end{mini*}
%     The optimal value of \eqref{eq: mlt optimization}, which is $-\infty$, is then the infimum of $t_\Omega$ over $\Omega \in \mathcal{O}_G$.
%     Since $\mathcal{O}_G$ is compact, this implies that $t_\Omega = -\infty$ for some $\Omega$.  Let us fix this 
%     $\Omega$.
    
%     If $\Omega$ is not PSD, then $t_\Omega > -\infty$ because $\tr(S(I+t\Omega)) - \log \det (I+t\Omega)\rightarrow \infty$ as $t\rightarrow t^*$ where $t^*$ is the supremum of the values of $t$ such that $I+t\Omega$ is nonsingular (and hence positive definite).
    
%     Now we know that $\Omega$ is PSD.  Then $\tr(S\Omega) \ge 0$, since both $S$ and $\Omega$ are PSD.  Hence, 
%     as $t\to \infty$, $\tr(S(I + t\Omega)) = \tr(S) + t\tr(S\Omega)$ grows linearly in $t$, unless $\tr(S\Omega) = 0$.
    
%     Hence, if $\tr(S\Omega)\neq 0$, we must have $\tr(S(I+t\Omega)) - \log\det(I+t\Omega)\rightarrow \infty$ as $t\rightarrow \infty$ 
%     because $|\log \det (I+t\Omega)|$ grows logarithmically in $t$, since the determinant is a polynomial in $t$.  
%     Therefore $t_\Omega > -\infty$, whenever $\tr(S\Omega)\neq 0$.  Because we have assumed  that $t_\Omega = -\infty$, we have  $\tr(S\Omega) = \tr(X^T\Omega X) = 0$. Since $\Omega$ is PSD, this implies $\Omega X = 0$.
%     So $\Omega$ is a PSD linear $G$-stress.
% \end{proof}

% \begin{defn}\label{def: eq stress}
% Let $G$ be a graph with $n$ vertices.  Let $(G,p)$ be a framework.  An \emph{equilibrium stress}
% $\omega$ of $(G,p)$ is 
% an assignment of  weights $\omega_{ij}$ to the edges of $G$ so that,
% for all vertices $i$
% \[
%     \sum_{j\sim i} \omega_{ij}(p(j) - p(i)) = 0 \qquad \text{(sum over neighbors of $i$).}
% \]
% The \emph{equilibrium stress matrix} associated to an equilibrium stress $\omega$ is the matrix $\Omega$ obtained by setting $\Omega_{ji} = \Omega_{ij} = \omega_{ij}$ for all edges $ij$ of $G$,
% $\Omega_{ii} = -\sum_{j} \omega_{ij}$ and all other entries zero.
% The \emph{rank} and \emph{signature} of $\omega$ are defined to be the rank and signature of $\Omega$.
% \end{defn}

% In Definition~\ref{defn: linear stress}, if the first column of $X$ is the all-ones vector, then a linear stress $\Omega$ of $X$ is an equilibrium stress matrix of the configuration of $n$ points in $\mathbb{R}^{d-1}$ consisting of the rows of the matrix obtained from $X$ by deleting the first column.

% \begin{rmk}\label{rmk: no stress means independent}
%     A graph $G$ is $d$-independent if and only if $(G,p)$ has no nonzero equilibrium stress for all generic $d$-dimensional point configurations $p$. This is because the space of equilibrium stresses of $(G,p)$ is the orthogonal complement of the space of differential changes to the edge lengths of $(G,p)$.
% \end{rmk}

% {\color{red} Insert appropriate remarks about generic vs almost surely, either here or in the following proof.}

% \begin{prop}\label{prop: psd mlt}
% Let $G$ be a graph with $n$ vertices.  Suppose that $d-1$ is 
% the largest dimension such that there is a generic 
% framework $(G,p)$ with a non-zero PSD equilibrium stress.  Then 
% $\mlt(G) = d + 1$.
% \end{prop}
% {\color{red} need to make iff}
% \begin{proof}
%     Let $(G,p)$ be a generic framework of $n$ points in $d-1$ dimensions with a nonzero PSD equilibrium stress $\hat \Omega$.
%     Let $\hat X$ be the $n\times (d-1)$ matrix whose rows are given by the points in $p$ and let $X$ be obtained from $\hat X$ by adjoining a column of all ones, then multiplying on the left by a generic diagonal $n\times n$ matrix $D$. Define $\Omega = D^{-1} \Omega D^{-1}$. Then $X$ is a generic $n\times d$ matrix with PSD linear stress $\Omega$ and so lemma~\ref{lemma: infeasible iff linear psd stress} implies that the MLE in the graphical model associated to $G$ does not exist when the data consists of the $d$ generic observations given by the columns of $X$.
    
%     Now let $X$ be an $n\times (d+1)$ matrix.
%     In light of Lemma~\ref{lemma: infeasible iff linear psd stress} it suffices to show that $X$ does not have a PSD linear $G$-stress.
%     So assume for the sake of contradiction that $X$ has a PSD linear $G$-stress $\Omega$.
%     Let $D$ be the diagonal matrix such that the first column of $DX$ is the all-ones vector
%     and let $q$ be the point configuration consisting of the rows of the matrix obtained from $DX$ by removing the first column.
%     Then $(G,q)$ is a generic $d$-framework and $D^{-1} X D^{-1}$ is a PSD equilibrium stress.
% \end{proof}

% \begin{rmk}\label{rmk: Uhler's inequality alternate proof}
%     Combining Proposition~\ref{prop: psd mlt} with Remark~\ref{rmk: no stress means independent} gives a rigidity-theoretic proof for Uhler's inequality $\mlt(G) \le \gcr(G)$. Indeed, Remark~\ref{rmk: no stress means independent} tells us that if $\gcr(G) = d+1$, then any generic $d$-dimensional framework $(G,p)$ has no nonzero equilibrium stress, and therefore no nonzero PSD equilibrium stress. Proposition~\ref{prop: psd mlt} now tells us that $\mlt(G) \le d+1$.
% \end{rmk}

% \begin{defn}
% Let $G$ have $n$ vertices.  Let $(G,p)$ be a $d$-dimensional framework.  We say that 
% $(G,p)$ is \emph{liftable} if there is an $n-1$ dimensional framework $(G,\tilde{p})$
% with full affine span equivalent to $(G,p)$.
% \end{defn}

% The following Lemma is due to Alfakih~\cite{alfakih2011bar}.
% For completeness, we provide a proof in the appendix that uses 
% convex geometry ideas from \cite{gt1}.

% \begin{lemma}[\cite{alfakih2011bar}]\label{lem: psd lift}
% A $d$-dimensional framework $(G,p)$ is liftable if and only if 
% it does not have a non-zero PSD equilibrium stress.
% \end{lemma}

% We are now ready to prove Theorem~\ref{thm: correspond}.

% \begin{proof}[Proof of Theorem~\ref{thm: correspond}]
%     Lemma~\ref{lem: psd lift} implies that $d-1$ is the largest dimension such that some generic framework has a PSD stress. Proposition~\ref{prop: psd mlt} now gives the theorem.
%     {\color{red} need to make iff}
% \end{proof}

% \section{Maximum likelihood thresholds and lifting}\label{sec: lifting}
% In this section we detail some relationships between 
% rigidity and the maximum likelihood threshold. In particular, we will prove Theorem~\ref{thm: correspond}.
% We will develop the proof along with the necessary technology.  For 
% convenience, we introduce the following notion.
% \begin{defn}
% Let $G$ have $n$ vertices.  Let $(G,p)$ be a $d$-dimensional framework.  We say that 
% $(G,p)$ is \emph{liftable} if there is an $n-1$ dimensional framework $(G,\tilde{p})$
% with full affine span equivalent to $(G,p)$.
% \end{defn}
% In the language of \cite{alfakih2011bar}, a liftable $(G,p)$ is not ``dimensionally rigid'' in 
% any dimension except $n-1$.  In the terminology of \cite{gross2018maximum}, a $d$-dimensional 
% framework which is not liftable is ``$d$-dependently rigid''.

% To understand liftability, we need equilibrium stresses.

% \begin{defn}\label{def: eq stress}
% Let $G$ be a graph with $n$ vertices.  Let $(G,p)$ be a framework.  An \emph{equilibrium stress}
% $\omega$ of $(G,p)$ is 
% an assignment of  weights $\omega_{ij}$ to the edges of $G$ so that,
% for all vertices $i$
% \[
%     \sum_{j\sim i} \omega_{ij}(p(j) - p(i)) = 0 \qquad \text{(sum over neighbors of $i$).}
% \]
% The \emph{equilibrium stress matrix} associated to an equilibrium stress $\omega$ is the matrix $\Omega$ obtained by setting $\Omega_{ji} = \Omega_{ij} = \omega_{ij}$ for all edges $ij$ of $G$,
% $\Omega_{ii} = -\sum_{j} \omega_{ij}$ and all other entries zero.
% The \emph{rank} and \emph{signature} of $\omega$ are defined to be the rank and signature of $\Omega$.
% \end{defn}

% \begin{rmk}\label{rmk: no stress means independent}
%     A graph $G$ is $d$-independent if and only if $(G,p)$ has no nonzero equilibrium stress for all generic $d$-dimensional point configurations $p$. This is because the space of equilibrium stresses of $(G,p)$ is the orthogonal complement of the space of differential changes to the edge lengths of $(G,p)$.
% \end{rmk}

% We also have the following result of Alfakih.
% \begin{lemma}[\cite{alfakih2011bar}]\label{lem: psd lift}
% A $d$-dimensional framework $(G,p)$ is liftable if and only if 
% it does not have a non-zero PSD equilibrium stress.
% \end{lemma}
% For completeness, we provide a proof in the appendix that uses 
% convex geometry ideas from \cite{gt1}. We also record
% the following, which combines Lemma \ref{lem: psd lift}
% and Theorem \ref{thm: correspond}.

% \begin{cor}\label{cor: psd mlt}
% Let $G$ be a graph with $n$ vertices.  Suppose that $d-1$ is 
% the largest dimension such that there is a generic 
% framework $(G,p)$ with a non-zero PSD equilibrium stress.  Then 
% $\mlt(G) = d + 1$.
% \end{cor}

% \begin{rmk}\label{rmk: Uhler's inequality alternate proof}
%     Combining Proposition~\ref{prop: psd mlt} with Remark~\ref{rmk: no stress means independent} gives a rigidity-theoretic proof for Uhler's inequality $\mlt(G) \le \gcr(G)$. Indeed, Remark~\ref{rmk: no stress means independent} tells us that if $\gcr(G) = d+1$, then any generic $d$-dimensional framework $(G,p)$ has no nonzero equilibrium stress, and therefore no nonzero PSD equilibrium stress. Proposition~\ref{prop: psd mlt} now tells us that $\mlt(G) \le d+1$.
% \end{rmk}

% Now that we have Alfakih's 
% characterization of liftable frameworks, we need to 
% make a translation to matrix completion.  As an 
% intermediate step, we use coning.
% \begin{defn}
% Let $G = (V,E)$ be a graph and $v_0\notin V$.  The \emph{cone graph}
% $v_0 * G$ is the graph obtained by adding a new vertex $v_0$
% and connecting it to all vertices $v\in V$.
% If $(G,p)$ is a $d$-dimensional framework, then a $(d+1)$-dimensional 
% framework $(v_0*G, \hat p)$ is a \emph{non-degenerate coning of $(G,p)$} if $(G,\hat p|_V)$
% has $d$-dimensional affine span and is congruent to $(G,p)$ and 
% $\hat p(v_0)$ lies outside the affine span of $\hat p|_V$.
% \end{defn}
% \begin{lemma}\label{lem: cone lift}
% A $d$-dimensional framework $(G,p)$ is liftable (to dimension $n-1$) if and only if all of its 
% non-degenerate conings are liftable (to dimension $n$).
% \end{lemma}
% \begin{proof}
% A result of Whiteley \cite{W83} is that the equilibrium stresses of a
% non-degenerate coning are all supported on edges of $G$ and 
% the same as those of $(G,p)$.  Because adding a row and column of zeros 
% to a stress matrix preserves PSD-ness, the coning $(v_0*G,\hat p)$
% has a non-zero PSD equilibrium stress if and only if $(G,p)$ 
% does.  The statement now follows from Lemma~\ref{lem: psd lift}.
% \end{proof}
% Next we look at frameworks on coned graphs in general.
% \begin{defn}
% Let $v_0*G$ be a coned graph.  A \emph{sliding} of a $(d+1)$-dimensional 
% framework $(v_0*G, \hat p)$
% is a framework obtained by moving the $\hat p(i)$, $i\in V$, 
% along the lines spanned by $\hat p(v_0)$ and $\hat p(i)$.  We disallow 
% slidings so that any other vertex ends at $\hat p(v_0)$.
% A \emph{non-degenerate flattening} of $(v_0*G, \hat p)$ is a sliding so 
% that all the vertices lie in a $d$-dimensional affine plane 
% that does not contain the cone point $p(v_0)$.  A \emph{slicing} $(G,p)$
% of $(v_0*G,\hat p)$ is a non-degenerate flattening, followed 
% by removing the cone vertex.
% \end{defn}
% \begin{lemma}\label{lem: cone graph lift}
% A $(d+1)$-dimensional cone 
% framework $(v_0*G,\hat p)$ is liftable if and 
% only if all of its slicings are.
% \end{lemma}
% \begin{proof}
% It is shown in \cite{cgt2} that sliding and slicing 
% preserves the existence of an equilibrium stress with a 
% given rank and signature.  The statement follows 
% from Lemmas \ref{lem: psd lift} and \ref{lem: cone lift}.
% \end{proof}
% While Lemmas \ref{lem: cone lift} and \ref{lem: cone graph lift}
% seem to be new, the underlying ideas are implicit in \cite{jjt1,jjt2}.
% Now we are ready to connect with the MLT matrix
% completion problem (Definition \ref{def: mlt matcomp}).
% \begin{lemma}\label{lem: matcomp cone equiv}
% Let $G$ be a graph with $n$ vertices.  The MLT matrix completion 
% problem for an $n\times n$ PSD matrix $A = \hat P^T \hat P$ of rank $d+1$ 
% is feasible if and only if the framework $(v_0*G,\hat p)$ is liftable 
% where $\hat p(v_0)$ is the origin and $\hat p(i)$
% is the $i$th column of $\hat P$ for vertices $i$ of $V$.
% \end{lemma}
% \begin{proof}
% Expanding the norm, we may write 
% \[
%  A_{ii} = \|\hat p(i) - \hat p(v_0)\|^2 = \|\hat p(i)\|^2   \qquad \text{and} \qquad A_{ij} = \frac{1}{2}(\|\hat p(i)\|^2 + \|\hat p(j)\|^2 - \|\hat p(i) - \hat p(j)\|^2)
% \]
% % $A_{ii} = \|\hat p(i) - \hat p(v_0)\|^2 = \|\hat p(i)\|^2$
% % and $A_{ij} = \frac{1}{2}(\|\hat p(i)\|^2 + \|\hat p(j)\|^2 - \|\hat p(i) - \hat p(j)\|^2)$.  
% Now suppose that $(v_0*G,\hat p)$ is liftable to a framework $(v_0*G,\tilde p)$ with $n$ dimensional
% affine span, 
% and with $\tilde p(v_0)$ at the origin.
% %in dimension $n+1$.  
% The Gram matrix $S$ of the vector configuration $\{\hat p(i) : i\in V\}$
% has rank $n$ from the assumed affine span and satisfies
% \[
%     S_{ii} = \|\tilde p(i)\|^2 = \|\hat p(i)\|^2 = A_{ii}
% \]
% and, for all edges $ij$ of $G$,
% \[
%     S_{ij} = \frac{1}{2}(\|\tilde p(i)\|^2 + \|\tilde p(j)\|^2 - \|\tilde p(i) - \tilde p(j)\|^2) = 
%     \frac{1}{2}(\|\hat p(i)\|^2 + \|\hat p(j)\|^2 - \|\hat p(i) - \hat p(j)\|^2) = A_{ij}
% \]
% where we have used equivalence of $(v_0*G,\hat p)$ and $(v_0*G,\tilde p)$.  Hence, $S$ is a 
% feasible solution for the MLT matrix completion problem for $A$.

% For the other direction, if $S$ is a feasible solution to the MLT matrix completion 
% problem for $A$, we can factorize $S = \tilde{P}^T\tilde{P}$ to recover a lifting 
% $(v_0*G, \tilde{p})$ of $(v_0*G,\hat p)$ by reversing the computations above.
% \end{proof}
% We remark that the proof of Lemma \ref{lem: matcomp cone equiv} relies crucially on 
% knowing the diagonal entries of $A$ (equivalently, that we used coning).  See 
% \cite{lv,singer} for similar relationships between PSD matrix 
% completion and coned frameworks.

% The next thing we need to do is take care of a technical 
% issue.  The MLT is defined in terms of an ``almost all''
% statement for PSD matrices, and Theorem \ref{thm: correspond}
% in terms of generic frameworks.  To switch between them, 
% we need a definition and then technical result.

% \begin{defn}\label{def: generic psd}
% Let $S\subseteq \RR^d$ be an irreducible semi-algebraic set.  
% We say that a point $x\in S$ is \emph{generic} if it does not satisfy 
% any polynomial defined over $\QQ$ that is not satisfied by every point in 
% $S$.
% \end{defn}

% \begin{lemma}\label{lem: generic vs almost all}
% The MLT of a graph $G$ is $d+1$ if and only if the MLT 
% matrix completion problem $(G,S)$ is not feasible for some 
% generic PSD matrix $A$ of rank $d$ and is feasible for every 
% generic PSD matrix $A$ of rank $d+1$.
% \end{lemma}
% The proof uses some general facts on semi-algebraic 
% sets and measure that we collect in Appendix~\ref{appendix: generic}.
% \begin{proof}
% Let $G$ be fixed.  For any rank $r$, the set $X_r$ of 
% rank $r$ PSD matrices $A$ for which the MLT matrix completion 
% problem $(G,A)$ is infeasible is semi-algebraic and defined 
% over $\QQ$.  Also note that any multivariate normal distribution 
% is Borel and mutually absolutely continuous with respect to 
% Hausdorff measure on the the set $S(r)$ of PSD matrices of 
% rank at most $r$.  The set $S(r)$ is an irreducible 
% semi-algebraic set defined over $\QQ$.

% Now suppose that the MLT of $G$ is $d+1$.  Then 
% the set $X_d$ is non-null, so, by Lemma \ref{lem: semi-alg generic} (c) contains a generic point of $S(d)$.  Also, the set 
% $X_{d+1}$ is null, so Lemma \ref{lem: semi-alg generic} (a)
% implies that no generic point of $S(d+1)$ is in $X_{d+1}$.

% In the other direction, suppose that there is a generic 
% point $A$ of $S$ for which $(G,A)$ is not feasible.  Then 
% Lemma \ref{lem: semi-alg generic} (a) implies that 
% $X_d$ is non-null.  If every, for generic PSD matrix $A$ of 
% rank $d+1$ (all generic $A\in S(r)$ have rank $r$), 
% the MLT matrix completion problem $(G,A)$ is 
% feasible, then  $X_{d+1}$ 
% consists of only non-generic points of $S(d+1)$.  
% Lemma \ref{lem: semi-alg generic} (b) then implies that 
% the complement of $X_{d+1}$ has full measure.
% \end{proof}
% At this point, we are ready for the section's main result.
% \begin{proof}[Proof of Theorem \ref{thm: correspond}]
% From   
% Theorem \ref{thm: dempster complete} we can use the MLT
% matrix completion problem to study  the MLT.
% Lemma \ref{lem: generic vs almost all} implies that 
% it is sufficient to consider generic PSD matrices of 
% rank $d$ and $d+1$ in the MLT matrix completion
% problem and then relate them to generic frameworks.

% First we suppose that the MLT of $G$ is $d+1$.  Then there 
% is a generic PSD matrix $S$ of rank $d$ so that the associated 
% matrix completion problem is infeasible.  Let us now 
% consider a coned framework $(v_0*G, \hat p)$ in dimension $d$ 
% as in Lemma \ref{lem: matcomp cone equiv}.  We know that this 
% coned framework is not liftable, and, 
% by Lemma \ref{lem: cone graph lift}
% neither is any slicing $(G,p)$ 
% of $(v_0*G, \hat p)$ (in dimension $d-1$).  By 
% Lemmas \ref{lem: gen psd factor} and then \ref{lem: gen slicing}
% both $(v_0*G, \hat p)$ and $(G,p)$ can be chosen to 
% be generic.  Hence, there is a generic framework $(G,p)$
% in dimension $d-1$ that is not liftable.

% Since the MLT of $G$ is $d+1$, we know that  MLT 
% matrix completion problem 
% is feasible for any generic PSD matrix of rank $d+1$.
% Consider a generic framework $(G,p)$ in dimension $d$.
% We pick a generic coning  $(v_0*G,\hat p)$ of $(G,p)$  
% with $\hat p(v_0)$ at the origin.  By Lemma \ref{lem: gen psd factor},
% the Gram matrix $A$ of $\hat p$ is a generic PSD matrix of rank $d+1$.
% By assumption, its MLT completion problem is feasible.
% By Lemma \ref{lem: matcomp cone equiv} and then Lemma~\ref{lem: cone lift}, $(G,p)$ is liftable.
% % Since $(G,p)$ was an arbitrary generic 
% % framework, all of them all.

% % The reasoning in the other direction (going from the liftibility 
% % properties of $G$ to the MLT)
% % is similar, just exchanging the order
% % of where we use Lemmas \ref{lem: cone lift} and \ref{lem: cone graph lift}.

% Now we suppose that there is a generic framework 
% $(G,p)$ in dimension $d-1$ that is not liftable and 
% that every generic framework $(G,p)$ in dimension $d$
% is liftable.

% Let us begin with a generic $(d-1)$-dimensional framework 
% $(G,p)$ that is not liftable.  A generic coning 
% $(v_0* G,\hat p)$ of $(G,p)$ in dimension $d$ is 
% not liftable either by Lemma \ref{lem: cone graph lift}.
% Now we apply Lemmas \ref{lem: matcomp cone equiv} and 
% \ref{lem: gen psd factor} to conclude that there is a 
% generic rank $d$ PSD matrix $A$ for which the MLT 
% matrix completion problem is infeasible.

% Finally, suppose that every generic $d$-dimensional
% framework $(G,p)$ is liftable.  Start with a 
% generic PSD matrix $A$ of rank $d+1$.  By Lemma 
% \ref{lem: gen psd factor}, we can find a generic 
% vector configuration $\hat p$ that has $A$ 
% as its gram matrix.  We then obtain a cone 
% framework $(v_0*G,\hat p)$ with $v_0$ at
% the origin and $\hat p$ generic.  This cone framework 
% has a generic slicing  $(G,p)$ in dimension $d$
% by Lemma \ref{lem: gen slicing}.  Since we assume that
% $(G,p)$ is liftable, so is $(v_0*G,\hat p)$ by 
% Lemma \ref{lem: cone graph lift}.  Finally, the MLT 
% matrix completion problem $(G,A)$ is feasible by 
% Lemma \ref{lem: matcomp cone equiv}.
% Having dealt with all four cases, the theorem is proved.
% \end{proof}

\section{MLT bounds from global rigidity}\label{sec: mlt gr}

We can use the results of the previous section along with some facts about global 
rigidity to get improved bounds for the MLT and compute it exactly for some 
interesting families.
% \begin{defn}\label{def: global rigdity}
% A $d$-dimensional framework $(G,p)$ is globally rigid if any other 
% $d$-dimensional framework $(G,q)$ that is equivalent to $p$ is 
% congruent to $p$; i.e., there is a Euclidean isometry $T$ of $\RR^d$ 
% so that $q(i) = T(p(i))$ for all vertices $i$ of $G$.
% \end{defn}
% Let us recall two results about  global rigidity.  
% The first is that global rigidity is a generic property.
% \begin{thm}[\cite{gortler2010characterizing}]\label{thm: ght}
% Let $G$ be a graph with $n\ge d+2$ vertices 
% and $d$ a dimension.  Then either every generic framework $(G,p)$
% is globally rigid and has an equilibrium stress of rank $n - d -1$ or 
% every generic framework $(G,p)$ 
% is not globally rigid and does not have an equilibrium stress of 
% rank $n - d -1$.
% \end{thm}
% \begin{defn}\label{def: ggr}
% A graph $G$ is called generically globally rigid in $d$-dimensions if every generic 
% $d$-dimensional framework $(G,p)$ is globally rigid.
% \end{defn}
The main technical tool of this section relates generic global rigidity to 
PSD equilibrium stresses.
\begin{thm}[\cite{cgt1}]\label{thm: gen ur}
Let $G$ be a graph with $n\ge d + 2$ vertices and $d$ a dimension.  If $G$ globally $d$-rigid, then there is a generic framework $(G,p)$ with a 
PSD equilibrium stress of rank $n - d - 1$.
\end{thm}
We also need a straightforward lemma.
\begin{lemma}\label{lem: mlt monotone}
Let $G$ be a graph and $H$ a subgraph of $G$.  Then $\mlt(H)\le \mlt(G)$.
\end{lemma}
\subsection{Lower bounds}
The main results of this section are new lower 
bounds on the MLT of a graph arising from 
global rigidity in terms of the global rigidity 
number (Def. \ref{def: grn}.)

\begin{proof}[Proof of Theorem \ref{thm: grn mlt}]
Suppose that $G$ is globally $d$-rigid. By Theorem \ref{thm: gen ur}, 
there is a generic framework $(G,p)$ with a non-zero PSD equilibrium stress.  By Theorem \ref{thm: main mlt stress}, $\mlt(G) > d + 1$.
Taking $d$ as large as possible for $G$ to remain   globally $d$-rigid we get 
$\mlt(G) >  \grn(G) + 1$.  The same argument works for any subgraph $H$ of $G$, so Lemma \ref{lem: mlt monotone}
implies that $\mlt(G)\ge \mlt(H) > \grn(H) + 1$.  Maximizing the right-hand side over $H$ we get $\mlt(G) > \grn^*(G) + 1.$
Since $G$ is a subgraph of itself, plainly $\grn^*(G)\ge \grn(G)$.
\end{proof}

We can efficiently compute $\grn(G)$ \cite{gortler2010characterizing}, 
but we do not know the complexity of computing $\grn^*(G)$.  A 
related graph parameter, which may be more computationally tractable is 
the local rigidity analogue.
\begin{defn}\label{def: rigidity number}
Let $G$ be a graph with $n$ vertices.  
The \emph{rigidity number} $\rignum(G)$ is the largest 
$d$ so that $G$ is $d$-rigid and has at least $d+1$ vertices.  
The \emph{subgraph rigidity 
number} $\rignum^*(G)$ is the largest $d$ so 
that $G$ has a subgraph $H$ on at least $d+1$
vertices that is $d$-rigid.
\end{defn}
\begin{thm}\label{thm: rnr mlt}
Let $G$ be a graph.  Then $\rignum(G) + 1\le \rignum^*(G) + 1\le \mlt(G)$.
\end{thm}
The proof needs a result of Jordán.
\begin{lemma}[\cite{J17}]\label{lem: inf rigid d to gr d -1}
Let $G$ be a graph that is $(d+1)$-rigid.  Then $G$ is globally $d$-rigid.
\end{lemma}
\begin{proof}[Proof of Theorem \ref{thm: rnr mlt}]
By Lemma \ref{lem: inf rigid d to gr d -1} one has $\rignum^*(G)\le \grn^*(G)+1$.
Theorem \ref{thm: grn mlt} then implies that 
$\rignum^*(G) + 1 \le \mlt(G)$.
Plainly 
$\rignum(G)\le \rignum^*(G)$, 
giving the last inequality.
\end{proof}
Theorem \ref{thm: rnr mlt} is strictly weaker than 
Theorem \ref{thm: grn mlt}.  For example, for every $n\ge 4$
there are globally rigid graphs in dimension $2$ that have 
$2n - 2$ edges \cite{bergjordan,Bob05}, but if $n>4$ then 
$2n - 2 < 3n - 6$, so these graphs cannot be $3$-rigid. 

The rigidity number of a graph is also easy to compute 
\cite{asimow1978rigidity}.  We do not know the complexity
of computing $\rignum^*(G)$, but, since local rigidity 
is matroidal in nature, tools from submodular optimization 
may apply.

\subsection{Combined bounds and examples}
Combining what we know so far gives the following.
\begin{thm}\label{rigidityBounds}
For any graph $G$, the following inequalities hold
\begin{enumerate}[(a)]
    \item $\omega(G)\le \rignum^*(G)+1 \le   \grn^*(G)+2 \le \mlt(G)\le\gcr(G)\le \tau(G) + 1$, and
    \item $\rignum(G)+1 \le \grn(G)+2 \le \grn^*(G)+2$.  
\end{enumerate}

\end{thm}

\begin{cor}\label{cor:gr+ind}
If $G$ is both globally $d$-rigid and $(d+1)$-independent, then $\mlt(G) = d+2$.
\end{cor}
We now exhibit new two infinite families of 
graphs $G$ for which the inequalities $\grn(G)+2 \le \grn^*(G)+2 \le \mlt(G) \le \gcr(G)$ are tight.
By applying Lemma \ref{lem: inf rigid d to gr d -1} and Corollary \ref{cor:gr+ind},
we obtain our first infinite family of graphs,
which are the higher dimensional analogue of trees.

\begin{cor}\label{cor:min rigid implies gcr=mlt}
If $G$ is minimally $d$-rigid, then $\mlt(G) = \gcr(G) = d+1$.
\end{cor}

Our next example is, in essence, an extension of the cycle graphs to higher dimensions.

\begin{defn}\label{defn: circuit}
    $G$ is a \emph{$d$-circuit} if it is not $d$-independent, but every proper subgraph is.
\end{defn}

\begin{cor}\label{cor:gr+cir}
    Let $G$ be a $d$-circuit.  Then $\gcr(G)=d+2$.
    If, furthermore, $G$ is globally $d$-rigid, 
    then $\mlt(G) = d+2$ also.
\end{cor}
\begin{proof}
    Whiteley \cite{W83} proved that $G$ is $d$-independent if and only if the coned graph $v_0*G$, that adds a new vertex $v_0$ connected to 
    every other vertex, is $(d+1)$-independent.
    Since $G$ is a $d$-circuit,
    for any vertex $v$, $G - v$ must be $d$-independent.
    Hence, $v_0*(G - v)$ is $(d+1)$-independent by Whiteley's result.  
    Since $G$ is isomorphic to a subgraph of  $v_0*(G - v)$, 
    it is also $(d+1)$-independent.
    The claim now follows from Corollary \ref{cor:gr+ind}.
\end{proof}

As promised in the introduction, we now can construct, for 
each $d$ and $n\ge k-1$, a graph $G$ with MLT $k$. 
We need a definition from combinatorial rigidity.
\begin{defn}\label{def: 0-ext and 1-ext}
    A \emph{($d$-dimensional) $0$-extension} of a graph $G$ is the graph obtained from $G$ by adding a new vertex of degree $d$. A \emph{($d$-dimensional) $1$-extension} of $G$ is the graph obtained from $G$ by removing an edge $xy$, and adding a new vertex adjacent to $x$, $y$ and $d-1$ other vertices.
    The inverse of these operations are called \emph{($d$-dimensional) $0$- and $1$-reductions}.
\end{defn}
It is a basic exercise to show that both $d$-dimensional 0- and 1-extensions will preserve $d$-rigidity and $d$-independence, and Connelly \cite{Bob05} 
proved that if $G$ is a globally $d$-rigid $d$-circuit, 
then any graph obtained via a $1$-extension on $G$ is also 
a globally $d$-rigid $d$-circuit.
By performing 0- and 1-extensions starting from $K_{d+1}$,
we can obtain a minimally $d$-rigid graph for each $n \ge d+1$.
Similarly, by performing $1$-extensions starting from $K_{d+2}$,
we obtain a globally rigid $d$-circuit for each $n\ge d+1$.
By Corollaries \ref{cor:min rigid implies gcr=mlt} and \ref{cor:gr+cir},
each of these has MLT equal to $d+1$ and $d+2$ respectively.

As mentioned, globally $d$-rigid graphs (or $d$-circuits) are not always locally $(d+1)$-rigid, hence the above construction for globally $d$-rigid $d$-circuits does not always give graphs for which $\rignum(G)+1 = \mlt(G)$. Additionally, we have not attempted to optimize the number of graphs in either of the above constructions,
and it is known that there exist graphs in either family that cannot be constructed this way.
By observing all the possible constructions from $K_{d+1}$ solely by 0-extensions,
it can be seen that the number of minimally $d$-rigid graphs on $n$ vertices grows exponentially with $n$.
Also a more careful analysis,
say of the degree sequences,
seems likely to yield exponentially many globally $d$-rigid $d$-circuits.
%similar to that found with minimally $d$-rigid graphs. 

\section{Complete bipartite graphs}\label{sec: complete bipartite}
To test the upper bound from Theorem \ref{thm: uhler gcr mlt} and the 
lower bound from \ref{thm: buhl}, 
Blekherman and Sinn \cite{blekherman2019maximum}
considered the case of complete bipartite graphs.
They were able to compute the MLT and generic completion ranks exactly, 
obtaining a number of strong results, including 
the first examples of graphs $G$ with $\mlt(G) < \gcr(G)$.

Since, equilibrium stresses of complete bipartite graphs are 
very well understood \cite{bolker1980bipartite,CGbipartite}, 
we have an alternative path to the results from 
\cite{blekherman2019maximum}.
We require the two following results on the 
rigidity theory of bipartite graphs.

\begin{lemma}[\cite{CGTunpublished}]\label{lem: Kmn ggr}
    Fix a $d\in \NN$ and let $m, n\ge d + 1$.  
    If $m + n \ge \binom{d+2}{2} + 1$
    then $K_{m,n}$ is   globally rigid
    in dimension $d$.
\end{lemma}

Given a finite subset $S$ of a vector space, let $D(S)$ denote the linear space of affine dependencies among $S$
and let $S^2$ be the image of $S$ under the \emph{Veronese map} $x\mapsto xx^T$.
The following theorem collects what we need from Bolker and Roth's classic paper~\cite{bolker1980bipartite}.


\begin{thm}\label{thm: bolker roth}
    Let $m,n,d \in \NN$ and let $(K_{m,n},p)$ be a $d$-dimensional framework.
    Let $A,B\subseteq \mathbb{R}^d$ denote the images under $p$ of the partite sets of $K_{m,n}$.
    Then the linear space of equilibrium stresses of $(K_{m,n},p)$ has dimension
    \[
        \dim(D(A))\dim(D(B)) + \dim(D((A\cup B)^2)).
    \]
    Moreover, if $p$ is generic and $m + n \le \binom{d+2}{2}$, then every equilibrium stress matrix has zeros along its diagonal.
\end{thm}
\begin{proof}
    The first claim follows from \cite[Theorem~1]{bolker1980bipartite}.
    The second claim follows from~\cite[Lemma~5]{bolker1980bipartite} and the fact that any set of $\binom{d+2}{2}$ generic symmetric matrices of rank~$1$ is a basis of the space of symmetric $(d+1)\times (d+1)$ matrices.
\end{proof}

\begin{thm}[\cite{blekherman2019maximum}]\label{thm: bipartite 1}
Let $d,m,n\in \NN$ with $m, n\ge d + 2$.
If $m + n \le \binom{d+2}{2}$, then $\mlt(K_{m,n}) \le d + 1$ and $\gcr(K_{m,n}) \ge d + 2$.
\end{thm}
\begin{proof}
Let $(K_{m,n},p)$ be a generic $d$-dimensional framework.
Since $m + n \le \binom{d+2}{2}$, Theorem~\ref{thm: bolker roth} implies that every stress matrix has zeros along its diagonal and is therefore indefinite. Theorem \ref{thm: main mlt stress} 
then implies that $\mlt(K_{m,n}) \le d + 1$.
On the other hand, Theorem~\ref{thm: bolker roth} implies that the space of stresses has dimension at least
$\dim(D(A))\dim(D(B))$, which is positive as $m,n \ge d+2$.
The existence of an equilibrium stress implies that $\gcr(K_{m,n}) \ge d + 2$.
\end{proof}
At this point Theorem \ref{thm: blekherman Kmn} follows quickly.
\begin{proof}[Proof of Theorem~\ref{thm: blekherman Kmn}]
    Theorem \ref{thm: bolker roth} implies that $K_{m,m}$, for $m > 2$,
    is $(m-1)$-independent but not $(m-2)$-independent.  Hence 
    $\gcr(K_{m,m}) = m$.
    By Lemma \ref{lem: Kmn ggr}, for $n > 2$, 
    the global rigidity number of $K_{m,m}$ is the maximum $d$ so that $2m\ge \binom{d+2}{2}+1$.
    For this $d$, Theorem \ref{thm: grn mlt} implies 
    that $\mlt(K_{m,m}) \ge d + 2$.  For any 
    larger $d'$, we have $2m \le \binom{d'+2}{2}$.
    Theorem \ref{thm: bipartite 1} then tells us 
    that $\mlt(K_{m,m})\le (d + 1) + 1 = d + 2$.
    Combining both bounds, we conclude that the MLT of $K_{m,m}$ is the largest 
    $D$ so that $2m > \binom{D+1}{2}$
    as desired.
\end{proof}

\section{A gluing construction}\label{sec: gluing}

In this section we prove some specialized results about giving lower bounds on MLT of graphs. We do this by constructing PSD equilibrium stresses on generic frameworks of a graph obtained by
gluing together smaller frameworks that each have a PSD equilibrium stress.
We will need the following construction from rigidity theory.

\begin{defn}
    Let $G$ be a graph with $n$ vertices and $m$ edges.
    The \emph{rigidity matrix} $R(G,p)$ of a $d$-dimensional framework $(G,p)$ is the $m\times dn$ matrix
    whose rows are indexed by the edges of $G$, columns indexed by the coordinates of $p(1),\dots,p(n)$,
    where the entry corresponding to edge $e$ and $p(v)_i$
    is $p(v)_i-p(u)_i$ if $e = vu$, and $0$ if $v$ is not incident to $e$.
\end{defn}

Given a $d$-dimensional framework $(G,p)$ on a graph $G$ with $n$ vertices, $R(G,p)$ is the Jacobian of the map sending $n$ points in $\mathbb{R}^d$ to the pairwise squared distances corresponding to the edges of $G$, evaluated at $p$.
Equilibrium stresses of $R(G,p)$ are the elements of the left kernel of $R(G,p)$.
% It is well-known that $G$ is generically rigid if and only if $R(G,p)$ has rank $dn-\binom{d+1}{2}$ for generic $p$, and that $G$ is generically independent if the rows of $R(G,p)$ are linearly independent for generic $p$.


\begin{defn}\label{def: clique sum}
A graph $G$ is a \emph{$k$-sum} of two induced 
subgraphs $G_1$ and $G_2$ each with at least $k+1$ vertices 
if $G$ is the union of $G_1$ and $G_2$ and  $G_1\cap G_2$ is isomorphic to $K_k$.
\end{defn}
The following result on equilibrium stresses of frameworks on $k$-sums is standard.
\begin{lemma}\label{lem: d-sum stress}
Let $1\le k\le d+1$ be integers and $G$ a $k$-sum of subgraphs $G_1$ and $G_2$.
Let $(G,p)$
be a $d$-dimensional framework with the vertices of $G_1\cap G_2$ affinely 
independent.
Let $S$ be the space of equilibrium stresses of $(G,p)$ and 
$S_i$ the space of equilibrium stresses of $(G,p)$ supported on the edges of $G_i$.  
Then $S = S_1\oplus S_2$.
\end{lemma}
\begin{proof}
Let $K = G_1\cap G_2$.  
First observe that any equilibrium stress $\omega\in S_1\cap S_2$ 
must be supported by the edges of $K$ and so is an 
equilibrium stress of $(K,p|_K)$.
Since $K$ has at most $d+1$ vertices and is in general affine position, 
$(K,p|_K)$ supports only the zero equilibrium 
stress.  Hence $S_1 + S_2 = S_1\oplus S_2$.


Denote $R_i = R(G_i,p|_{G_i})$.  
The row spans of $R_1$ and $R_2$ are naturally included in the row span 
of $R(G,p)$.  Both of these 
spans include $R(K,p|_K)$.  By general position of the vertices 
corresponding to $K$, this latter space has dimension $\binom{k}{2}$.
So by the interpretation of $S$ and the $S_i$ as cokernels 
of the rigidity matrix and rank-nullity, 
we have
\begin{align*}
    \dim(S) &= m - \rank R(p)\\
    &= m_1 + m_2 - \binom{k}{2} - \rank R(p)\\
    &= m_1 + m_2 - \binom{k}{2} - \rank R_1 - \rank R_2 + \binom{k}{2}\\
    &= m_1 - \rank R_1 + m_2 - \rank R_2\\
    &= \dim(S_1 \oplus S_2)
\end{align*}
and so we can conclude $S = S_1 + S_2 = S_1\oplus S_2$.
\end{proof}


A framework $(G,p)$ is \emph{regular} if its rigidity matrix 
has maximum rank over all frameworks $(G,q)$.
Regularity is preserved 
under non-singular projective transforms applied to $p$.
The converse of the following corollary also true, but we do not need it.

\begin{cor}\label{cor: d-sum rank}
Let $1\le k\le d+1$ and $G$ be a $k$-sum of $G_1$ and $G_2$.  Let $(G,p)$ 
be a $d$-dimensional framework.  If $(G_1,p|_{V(G_1)})$ and 
$(G_2,p|_{V(G_2)})$ are regular then $(G,p)$ is regular.
\end{cor}

\begin{proof}
Let $G_i$ have $n_i$ vertices and $m_i$ edges.  Assume that $p$ is 
such that $(G_1,p|_{V(G_1)})$ and 
$(G_2,p|_{V(G_2)})$ are both regular.  Let $r_i$ be the rank of the 
rigidity matrix of each of these frameworks and $s_i$ the dimension 
of the space of equilibrium stresses.
Observing that $G$ has $n_1 + n_2 - k$
vertices and $m_1 + m_2 - \binom{k}{2}$ edges, we can see that the maximum 
possible rank of the rigidity matrix for $(G,p)$ is $r_1 + r_2 - \binom{k}{2}$.
Since $K = G_1\cap G_2$ is complete and has at most $d+1$ vertices in dimension $d$, 
regularity of $(G_1,p|_{V(G_1)})$ and 
$(G_2,p|_{V(G_2)})$ implies that the vertices of $K$ are affinely independent.  Otherwise there is 
an equilibrium stress supported only on $K$ that is not present in all frameworks.
Hence, we may apply Lemma \ref{lem: d-sum stress} to $(G,p)$ to conclude that its space of 
equilibrium stresses is the direct sum of equilibrium stresses supported on $G_1$ and 
$G_2$ respectively.  The dimension of the space of equilibrium stresses of 
$(G,p)$ is then $s_1 + s_2$.  Then $(G,p)$ is regular since the rank of its rigidity matrix is
\[
    m_1 + m_2 - \binom{k}{2} - s_1 - s_2
    = 
    m_1 + m_2 - \binom{k}{2} - (m_1 - r_1) - (m_2 - r_2)
    = r_1 + r_2 - \binom{k}{2}.\qedhere
\]
\end{proof}
We also have some control of the signs of stress coefficients in PSD 
equilibrium stresses.  The following is from 
 \cite[Lemma 4.9]{cgt2} and the 
discussion around it.
\begin{lemma}\label{lem: psd stress sign}
Let $(G,p)$ be a $d$-dimensional framework and $\omega$ a PSD 
equilibrium stress of $(G,p)$ and $ij$ and edge of $G$ so that 
$\omega_{ij} > 0$.  Then there is a non-singular 
projective transformation $T$ on $\RR^d$ so that $(G,T(p))$
has a PSD equilibrium stress $\psi$ so that $\psi_{ij} < 0$.
\end{lemma}
% The following sketch is based on
% \begin{proof}[Sketch]
% We can model projective transformations on $\RR^d$ acting on a framework $(G,p)$ 
% by first making a non-degenerate coning $(G,p)$ 
% from the origin in $\RR^{d+1}$, then slicing.  

% It is shown in \cite{cgt2} if the sliding coefficients 
% are $s_i$, then equilibrium stress coefficients $\omega_{ij}$ transform as $s_is_j\omega_{ij}$,
% while the rank and signature of an equilibrium stress are preserved.
% In particular, if we want to change the sign of $\omega_{ij}$, we can take $s_i$ negative and 
% $s_j$ positive.
% \end{proof}

We have things in place for the main result of this section.
Given a graph $G$ with edge $ij$, we let $G-ij$ denote the graph obtained from $G$ by deleting the edge $ij$.

\begin{lemma}\label{lem: psd clique sum}
Let $1\le k\le d$ and $G$ be a $k$-sum of subgraphs $G_1$ and $G_2$
and $ij$ and edge of $G_1\cap G_2$.
Suppose that there are generic $d$-dimensional frameworks
$(G_1,p^1)$ and $(G_2,p^2)$ that, respectively, support 
non-zero PSD equilibrium stresses $\omega^1$ and $\omega^2$,
such that $\omega^k_{ij} \neq 0$ for $k = 1,2$.
Let $G' = G- ij$.
Then there is a generic $d$-dimensional framework $(G',p)$
that supports a non-zero PSD equilibrium stress.
\end{lemma}
\begin{proof}
First assume that $\omega^1_{ij} < 0$ and $\omega^2_{ij} > 0$.  
Since $G_1\cap G_2$ has at most $d$ vertices, any 
affinely independent framework on $G_1\cap G_2$ cannot support 
an equilibrium stress.  Hence, both $\omega^1$ and $\omega^2$ 
have some support outside of $G_1\cap G_2$.
We create a framework $(G,p^0)$ from the frameworks 
$(G_1,p^1)$ and $(G_2,p^2)$ as follows.  Pick a 
non-singular affine map $T$ sending the vertices of 
 $G_1\cap G_2$ in $(G_1,p^1)$ to the corresponding vertices 
in $(G_2,p^2)$ and apply it to $p^1$.  The defines a 
framework $(G,p^0)$.

By Corollary \ref{cor: d-sum rank} and the  
genericity of $(G_i,p^i)$, the framework $(G,p^0)$ 
is regular.  
Since equilibrium stresses are preserved under affine maps, 
$\omega^1$ and $\omega^2$ are both equilibrium stresses of $(G,p^0)$. 
Our assumptions about the 
signs imply that some positive linear combination $\omega$ of 
$\omega^1$ and $\omega^2$
has vanishing coefficient on the edge $ij$.  Because the $\omega^i$ 
have some necessarily disjoint support, $\omega$ is non-zero.
Since a positive 
combination of PSD equilibrium stresses is PSD, we conclude that $\omega$ is.  Since $\omega$ is not supported on $ij$, it 
is also an equilibrium stress of $(G',p^0)$.
Potentially, $(G',p^0)$ is not generic, but since it is regular, a  
small perturbation $(G,p)$ 
that is generic will have an equilibrium stress 
close to $\omega$ that is also PSD.

If $\omega^1_{ij} > 0$, we reduce to the previous case by 
applying a projective transformation, as in Lemma \ref{lem: psd stress sign}.
The argument is then the same as before, since we only used that the $(G_i,p^i)$
are generic to make them regular.  Regularity is preserved by 
projective transformations.
\end{proof}

\subsection{Remarks}
A natural question is whether the lower bound in Theorem \ref{thm: grn mlt}
is tight.  The results of this section show that it is not.  By Lemma 
\ref{lem: psd clique sum}, if we let $G$ be the $2$-sum of two copies
of $K_{d+2}$ over an edge $ij$, and $G'$ the graph $G-ij$,
there is a generic framework $(G',p)$ in dimension $d$ with a non-zero 
PSD equilibrium stress.  Theorem \ref{thm: main mlt stress}, 
then implies that $\mlt(G')\ge d + 2$.  On the other hand,
since every induced subgraph of $G'$ is independent in dimension 
$d$, $\grn^*(G')\le d-1$.  Hence, $\grn^*(G') + 2 < \mlt(G')$.

\section{Equality of small $\mlt(G)$ and $\gcr(G)$}\label{sec: mlt 3}
In this section, we prove Theorem \ref{thm: equality of gcr and mlt}, which rests on the rich combinatorial theory of  2-rigidity of graphs (see e.g.~\cite{lee-streinu} for an overview).
The cornerstone of this theory is Theorem~\ref{thm: LPG}, the Laman--Pollaczek-Geiringer theorem.
We begin with the necessary definitions.

\begin{defn}\label{def: laman}
A graph $G$ with $n$ vertices is $(2,3)$-sparse if, for all subgraphs 
with $n'$ vertices and $m'>0$ edges, $m' \le 2n' - 3$.
%If $G$ is $(2,3)$-sparse and, in addition has $2n - 3$ edges, it is called a\emph{Laman graph}.
A graph that is not $(2,3)$-sparse, but becomes so after removing any 
edge is called a \emph{Laman circuit}.
\end{defn}

\begin{thm}[\cite{LAMAN,HPG}]\label{thm: LPG}
A graph $G$ is $2$-independent if and only if $G$ is $(2,3)$-sparse.
\end{thm}

% A straightforward consequence of circuit minimality and Theorem \ref{thm: LPG} is:
% \begin{cor}\label{cor: circuit stress}
% Let $G$ be a Laman circuit and $(G,p)$ a generic $2$-dimensional 
% framework.  Then $(G,p)$ has a unique (up to scale) equilibrium 
% stress, supported on all the edges of $G$.
% \end{cor}

Via Theorem~\ref{thm: gross sullivant}, Theorem~\ref{thm: LPG} immediately gives us a combinatorial characterization of the graphs with $\gcr(G) = 3$; these are the $(2,3)$-sparse graphs that contain a cycle.
As we will see in Proposition~\ref{prop: mlt 3 laman}, this also characterizes graphs with $\mlt(G) = 3$.
In order to prove this, we need the following lemma which makes crucial use of Berg and Jordan's~\cite{bergjordan}
combinatorial characterization of global rigidity in two dimensions.

\begin{lemma}\label{lem: 2d PSD circuit stress}
Let $G$ be a Laman circuit.  Then there are generic $2$-dimensional
frameworks $(G,p)$ satisfying a non-zero PSD equilibrium stress.
\end{lemma}

\begin{proof}
If $G$ is $3$-connected, a result of Berg and Jordán \cite{bergjordan}  implies that $G$ is 
  globally rigid.  The desired statement then follows from Theorem \ref{thm: gen ur}.
If $G$ is not $3$-connected, we can find a $2$-separation $\{x,y\}\subseteq V(G)$ in $G$.
A counting argument \cite[Lemma 2.4, inter alia]{bergjordan} 
implies that
$xy$ is not an edge of $G$ and that $G\cup \{xy\}$ 
is a $2$-sum of smaller 
Laman circuits $G_1$ and $G_2$.  
By induction, we may assume that there are generic $2$-dimensional frameworks 
$(G_1,p^1)$ and $(G_2,p^2)$ that each support a PSD equilibrium stress $\omega^1$ and 
$\omega^2$. Since $G_1$ and $G_2$ are circuits, the supports of $\omega^1$ 
and $\omega^2$ include the edge $xy$.  By Lemma \ref{lem: psd clique sum}, there is then a generic framework $(G,p)$ with a non-zero 
PSD equilibrium stress.
\end{proof}

\begin{prop}\label{prop: mlt 3 laman}
Given a graph $G$, the following are equivalent:
\begin{enumerate}[(a)]
    \item\label{item: combinatorial} $G$ is $(2,3)$-sparse and contains a cycle,
    \item\label{item: gcr 3} $\gcr(G) = 3$, and
    \item\label{item: mlt 3} $\mlt(G) = 3$.
\end{enumerate}
\end{prop}

\begin{proof}
Theorems~\ref{thm: LPG} and~\ref{thm: gross sullivant} imply that $\gcr(G) = 3$ if and only if
$G$ is $(2,3)$-sparse and contains a cycle.
Now assume $\gcr(G) = 3$.
Since cycles are globally $1$-rigid, 
any graph $G$ with a cycle has $\grn^*(G)\ge 1$, so 
$\mlt(G)\ge 3$ by Theorem \ref{thm: grn mlt}.
On other other hand, if a graph $G$ is  
$(2,3)$-sparse then $\gcr(G)\le 3$ and so $\mlt(G)\le 3$ follows from Theorem~\ref{thm: uhler gcr mlt}.

If $\gcr(G) \le 2$ or $\mlt(G) \le 2$, then $G$ cannot have a cycle.
So assume $\gcr(G) \ge 4$.
Theorems~\ref{thm: LPG} and~\ref{thm: gross sullivant} now imply that $G$ contains a Laman circuit $H$ as a subgraph.
By Lemma \ref{lem: 2d PSD circuit stress},
$H$ has a generic $2$-dimensional framework $(H,p)$ with non-zero PSD equilibrium stress.
Theorem \ref{thm: main mlt stress} 
implies $\mlt(H) \ge 4$ and therefore Lemma~\ref{lem: mlt monotone} implies $\mlt(G) \ge 4$.
\end{proof}

We are now ready to prove the main result of this section.

\begin{proof}[Proof of Theorem~\ref{thm: equality of gcr and mlt}]
    As noted in~\cite{gross2018maximum}, $\mlt(G) = 1$ if and only if $G$ has no edges and $\mlt(G) = 2$ if and only if $G$ has no cycles.
    In both cases, it is easy to see that $\gcr(G) = \mlt(G)$.
    If $\mlt(G) = 3$ or $\gcr(G) = 3$, then $\mlt(G) = \gcr(G)$ follows from Proposition~\ref{prop: mlt 3 laman}.
    If $\gcr(G) = 4$, then
    Theorem~\ref{thm: LPG} and Lemma~\ref{lem: 2d PSD circuit stress} together imply that $\mlt(G) \ge 4$
    and equality follows from Theorem~\ref{thm: uhler gcr mlt}.
\end{proof}

\begin{rmk}\label{rmk: best possible}
Theorem~\ref{thm: equality of gcr and mlt} is best possible in the sense that if $a \ge 4$ and $b \ge 5$,
then there exist graphs $G,H$ such that $\mlt(G) = a < \gcr(G)$ and $\mlt(H) < b = \gcr(H)$.
In particular, let $n = \left\lfloor\frac{1}{2}\binom{a+1}{2}\right\rfloor$,
and let $D$ be the smallest $k$ such that $\binom{k+1}{2} \ge 2b$.
Then, Theorem~\ref{thm: blekherman Kmn} implies $\mlt(K_{n,n}) = a < n = \gcr(K_{n,n})$ and that $\gcr(K_{b,b}) = b > D =\mlt(K_{b,b})$.
\end{rmk}

%Gross and Sullivant showed that $\mlt(G) \le 4$ whenever $G$ is planar~\cite{gross2018maximum}. 
%Using Theorem~\ref{thm: equality of gcr and mlt}, we can strengthen this a bit as follows.

%\begin{cor}\label{cor:planar}
%	If $G$ is a $K_5$-minor free graph,
%	then $\mlt(G) = \gcr(G) \leq 4$.
%\end{cor}

%\begin{proof}
%Nevo \cite{nevo} showed that  $K_5$-minor free graphs are $3$-independent.
%Hence, Theorem~\ref{thm: gross sullivant} implies $\gcr(G) \leq 4$ and Theorem~\ref{thm: equality of gcr and mlt} now gives the result.
%\end{proof}

\section{Few vertices, many edges or bounded degree}\label{sec: many / few}

We now apply our tools to demonstrate that if $G$ has sufficiently few vertices, is sufficiently close to being complete, or has sufficiently small vertex degrees then $\mlt(G) = \gcr(G)$.
The proofs of the three following lemmas involve heavy case analysis so we defer them to Appendix~\ref{app:b}.
Recall the definition of $d$-circuit (Definition~\ref{defn: circuit}).

\begin{lemma}\label{lemma: 6 regular}
    Every $6$-regular graph on $9$ vertices is globally $4$-rigid.
\end{lemma}

\begin{lemma}\label{lem:d+5circcut}
    Suppose $G$ is a $d$-rigid $d$-circuit with $d+5$ vertices and minimum degree $d+1$. Then $G$ has a $d$-dimensional generic realization with a PSD equilibrium stress of rank at least~$3$.
\end{lemma}

\begin{lemma}\label{lem:3d9circcut}
    Suppose $G$ is a 3-rigid 3-circuit with $9$ vertices.
    Then $\mlt(G) \geq 5$.
\end{lemma}

\begin{figure}[h]
	\begin{center}
		\begin{tikzpicture}
			\node[vertex] (L1) at (-1,-0.5) {};
			\node[vertex] (L2) at (-1,0.5) {};
			\node[vertex] (C1) at (0,-1) {};
			\node[vertex] (C2) at (0,0) {};
			\node[vertex] (C3) at (0,1) {};
			\node[vertex] (R1) at (1,-0.5) {};
			\node[vertex] (R2) at (1,0.5) {};
	
			\draw[edge] (L1)edge(C1);
			\draw[edge] (L1)edge(C2);
			\draw[edge] (L1)edge(C3);
			
			\draw[edge] (L2)edge(C1);
			\draw[edge] (L2)edge(C2);
			\draw[edge] (L2)edge(C3);
			
			\draw[edge] (L1)edge(L2);
			
			\draw[edge] (R1)edge(C1);
			\draw[edge] (R1)edge(C2);
			\draw[edge] (R1)edge(C3);
			
			\draw[edge] (R2)edge(C1);
			\draw[edge] (R2)edge(C2);
			\draw[edge] (R2)edge(C3);
			
			\draw[edge] (R1)edge(R2);
			
			\draw[edge] (C1)edge(C2);
			\draw[edge] (C2)edge(C3);
		\end{tikzpicture}
	\end{center}
	\caption{The graph $H_3$.}
	\label{fig:h3}
\end{figure}

Let $H_d$ denote the graph obtained by gluing two copies of $K_{d+2}$ along a common $K_d$ subgraph and removing a common edge -- see Figure \ref{fig:h3} for an illustration of the $d=3$ case.

\begin{lemma}[\cite{egres-20-01}]\label{lemma: H_n}
    $H_d$ is the unique graph on at most $d+4$ vertices that is a $d$-rigid $d$-circuit and not $(d+1)$-connected.
\end{lemma}

\begin{lemma}\label{lemma: d circuit d+4 vertices}
    Let $G$ be a $d$-circuit on at most $d+4$ vertices.
    Then $\mlt(G) \ge d+2$.
\end{lemma}
\begin{proof}
    By Lemma~\ref{lemma: H_n}, if $G$ is not $(d+1)$-connected, then $G=H_d$.
    Since $K_{d+2}$ has a PSD equilibrium stress it follows from Lemma \ref{lem: psd clique sum} that $H_d$ has a PSD equilibrium stress and hence Theorem 
    \ref{thm: main mlt stress} implies that $\mlt(H_d)\ge d+2$.
    If $G$ is $(d+1)$-connected, then $G$ is globally rigid by Theorem~\ref{thm:tibor} and Corollary \ref{cor:gr+cir} gives the result.
\end{proof}

\begin{proof}[Proof of Theorem \ref{THM:SMALL}]
If $\gcr(H)=d+2$ then $H$ is not $d$-independent and therefore contains a $d$-circuit.
In light of Lemma~\ref{lem: mlt monotone}, it therefore suffices to prove any $d$-circuit $G$ with $9$ or fewer vertices has $\mlt(G) \geq d+2$.
By Theorem~\ref{thm: equality of gcr and mlt}, we may assume $d \ge 3$ and by Lemma~\ref{lemma: d circuit d+4 vertices}, we may assume $n \ge d+5$.
Thus either $d=3$ and $n\in \{8,9\}$, or $d=4$ and $n=9$. 

Assume that $G$ is $d$-rigid, i.e.~that it has $dn-\binom{d+1}{2}+1$ edges.
If $d=3$ and $n=9$ then $\mlt(G) \geq d+2$ by Lemma \ref{lem:3d9circcut}.
If $G$ has a vertex of degree $d+1$ and $d = 3$ and $n = 8$, or $d=4$ and $n=9$,
then $\mlt(G) \geq d+2$ by Lemma \ref{lem:d+5circcut} and Theorem 
\ref{thm: main mlt stress}.
If $G$ does not have a vertex of degree $d+1$, then $d=4$, $n=9$, and $G$ is $6$-regular.
In this case, Lemma~\ref{lemma: 6 regular} implies $G$ is globally rigid and
Corollary~\ref{cor:gr+cir} gives the result.

Thus we may assume that $G$ is not $d$-rigid.
Since $n\leq 9$ and $d\geq 3$, \cite[Theorem 1]{grasegger2020flexible} implies that $G$ is obtained from two rigid $d$-circuits by gluing them together over a common complete subgraph on $(d-1)$ or $(d-2)$ vertices and deleting exactly one edge from the intersection.  From above, the two rigid $d$-circuits that we glue
are globally $d$-rigid.  Theorem \ref{thm: gen ur} implies that there is a generic framework for each of these with 
a non-zero PSD equilibrium stress.  We may then apply  Lemma \ref{lem: psd clique sum} and Theorem \ref{thm: main mlt stress}
to conclude that $\mlt(G) = d+2$.
\end{proof}

\begin{cor}\label{c:manyedges}
    Let $G$ be a graph on $n$ vertices.
    If the complement of $G$ has at most 5 edges,
    then $\gcr(G)=\mlt(G)$.
\end{cor}

\begin{proof}
%As any graph with $\gcr=d+2$ is $d$-dependent and any $d$-dependent graph contains a $d$-circuit,
%it suffices to prove any $d$-circuit with 9 or less vertices has $\mlt \geq d+2$.
%DOESN'T WORK, BELOW SPECIAL CASE IS OKAY:
%Suppose $G$ is a $d$-circuit.
%By Theorems \ref{THM:SMALL} and \ref{prop: mlt 3 laman} we may assume $n\geq 10$ and $d\geq 3$ respectively. Then Theorem \ref{thm: gross sullivant} implies that $\gcr(G)=d+2$. We may assume $G\neq H_d$ and hence
%\cite[Theorem 3.2]{egres-20-01} implies that $G$ is globally $d$-rigid when $n\leq d+4$. Hence Corollary \ref{cor:gr+cir} gives the result.
%, Theorem \ref{thm: gen ur} and the fact that $H_d$ has a PSD stress, every $d$-circuit with $n\leq d+4$ has a PSD stress. 
%We may now assume that $n\geq d+5$.
%Since $G$ is a $d$-circuit
%$$|E|\leq dn-{d+1 \choose 2} + 1=\frac{(2n-1)d-d^2+2}{2}\leq \frac{n^2-n-18}{2}.$$
%Since 
%$$|E(K_n)|-|E|\geq {n \choose 2}-\frac{n^2-n-18}{2}=9,$$
%this contradicts the hypothesis of the theorem.
%=========
%\textcolor{red}{SEAN: This could be one method for extending the result but there are blanks to fill in.
%If this doesn't work, we have the result for 5 missing edges at the very least.
%We can also see if we can obtain a result for 6 or 7 missing edges.}
Fix $d = \gcr(G)-2$.
The graph $G$ is $(n-4)$-dependent since it has at least
\begin{align*}
    \binom{n}{2} -5 > (n-4)n - \binom{n-3}{2}
\end{align*}
edges, hence $d \geq n-4$. It follows that $G$ contains a $d$-circuit on at most $d+4$ vertices.
Lemmas~\ref{lem: mlt monotone} and~\ref{lemma: d circuit d+4 vertices} now imply $\mlt(G) = d+2$.
%Now suppose $d=n-5$.
%If $G$ contains a $d$-circuit on at most $d+5$ vertices then $\mlt(G)=d+2$ as previously stated,
%We are done unless every $d$-circuit of $G$ is spanning.
%\textcolor{red}{TO DO: Show that any such graph must be globally $d$-rigid. I think that any such graph cannot have a vertex of degree $d+1$ because we could do some cancellation of the stresses to obtain a smaller $d$-dependent subgraph.}
\end{proof}

The next corollary requires the following result of Jackson and Jord\'{a}n.
Given a graph $G$ and a subset $X$ of vertices,
$i(X)$ denotes the number of edges in the subgraph induced by~$X$.

\begin{thm}[\cite{JJ}]\label{thm:jacksonjordan}
    Let $G$ be a connected graph with minimum degree at most $d+1$ and maximum degree at most $d+2$.
    Then $G$ is $d$-independent if and only if $i(X) \leq d |X| - \binom{d+1}{2}$ for any vertex set $X \subset V$ with $|X| \geq d+2$.
\end{thm}

\begin{cor}\label{cor:degbounded}
    Let $G$ be a connected graph with minimum degree at most 4 and maximum degree at most 5.
    Then $\mlt(G) = \gcr(G) \leq 5$.
\end{cor}

\begin{proof}
    The degree hypothesis implies that any set $X \subset V$ satisfies $i(X) \leq \frac{1}{2}(5|X| - 1)$.
    Hence $i(X) \leq 4|X| -10$ for all $|X|\geq 6$ and $i(X) \leq 3|X| -6$ for all $|X| \geq 10$. Applying these two observations with Theorem \ref{thm:jacksonjordan} implies that we have $\gcr(G) \leq 5$,
    with equality if and only if $G$ contains a 3-circuit on at most 9 vertices (since no 4-circuit exists on at most 5 vertices).
    Suppose $\gcr(G) =5$ and let $H$ be a 3-circuit contained in $G$ with $|V(H)| \leq 9$.
    % We note that $|E(H)| = 3|V(H)|-5$, as otherwise $H$ will be 3-independent by Theorem \ref{thm:jacksonjordan}.
    % If $|V(H)|=10$ then $H$ 
    % contradicts the degree assumptions for $G$.
    % Hence $|V(H)| \leq 9$,
    The result follows from applying Theorem \ref{THM:SMALL} to $H$.
\end{proof}

The example of $K_{5,5}$ shows that the bound on $n$ in Theorem \ref{THM:SMALL} and the degree constraints in Corollary \ref{cor:degbounded} are tight. On the other hand one might expect that Corollary \ref{c:manyedges} remains valid for graphs whose complement has several more edges.




%\subsection{$d$-circuits with at most $d+4$ vertices}

%We will use the following characterisation of Jord\'an for global $d$-rigidity of graphs which are small relative to the dimension.

%\begin{thm}\label{thm:jordangr}\cite{egres-20-01}
%	Let $G=(V,E)$ be a graph with $|V| \leq d+4$.
%	Then $G$ is globally $d$-rigid if and only if $G$ is redundantly $d$-rigid and $(d+1)$-connected.
%\end{thm}

%When equality holds and $G$ is a $d$-circuit, $G = K_{d+4} - F$, where $F$ is a set of edges of size $5$ and no three edges of $F$ share a vertex.
%\begin{prop}\label{prop:jordancirc}\cite{egres-20-01}
%	Let $G=(V,E)$ be a $d$-circuit with $|V|=d+4$. 
	%If $|V|= d+3$ then $G = K_{d+3} - \{e,f\}$, where $e,f$ do not share a vertex, and 
%If $|V|=d+4$ then $G = K_{d+4} - F$, where $|F| = 5$ and no three edges of $F$ share a vertex.
%\end{prop}
%We define $H_d := G_1 \cup G_2 -e$,
%where $G_1,G_2 \cong K_{d+2}$, $|V(G_1) \cap V(G_2)|=d$ and $e \in G_1 \cap G_2$;
%see Figure \ref{fig:h3} for an illustration of the case when $d=3$.
%We extract from Theorem \ref{thm:jordangr} that $H_d$ is the only $d$-circuit on at most $d+4$ vertices that is not globally $d$-rigid.

%\begin{lemma}\label{lem:cird3}
%	Every $d$-circuit on at most $d+4$ vertices, distinct from $H_d$, is globally $d$-rigid.
%\end{lemma}

%\begin{proof}
%	Let $G=(V,E)$ be a $d$-circuit with $|V|\leq d+4$. If $|V|\leq d+3$ then it is easy to see that $G$ is $d$-rigid and $(d+1)$-connected. Hence Theorem \ref{thm:jordangr} implies that $G$ is globally $d$-rigid. So $|V|=d+4$. 
%	As discussed above, $G = K_{d+4}-F$ where no three edges of $F$ share a vertex. Since $G\neq H_d$ it is $(d+1)$-connected. Since $G$ is $d$-rigid, Theorem \ref{thm:jordangr} gives the result.
%\end{proof}

%\begin{proof}
%DELETE?
%	Let $G=(V,E)$ be a $d$-circuit with at most $d+3$ vertices.
%	By Proposition \ref{prop:jordancirc},
%	$G$ is redundantly $d$-rigid.
%	As the case $|V|=d+2$ is trivially true (the only $d$-circuit is the complete graph), we may assume $|V|=d+3$.
%	Any separating set $S$ of size strictly less than $d$ would imply $G$ was $d$-flexible,
%	and any separating set $S$ of size $d$ would imply $G$ has a vertex of degree $d$.
%	Since both contradict that $G$ is redundantly $d$-rigid,
%	$G$ must be $(d+1)$-connected.
%	We now apply Theorem \ref{thm:jordangr}.
%\end{proof}

%SEAN: Not needed, mentioned in Theorem \ref{THM:SMALL}
% \begin{lemma}\label{lem:smallcirc}
% 	Let $G=(V,E)$ be a $d$-circuit with $|V| \leq d+4$.
% 	Then $\mlt(G) = \gcr(G) = d+2$.
% \end{lemma}

% \begin{proof}
% 	By Corollary \ref{cor:gr+cir},
% 	$\gcr(G)=d+2$.
% 	The result now follows from Lemmas \ref{lem:cird3} and \ref{lem:hd} and Theorem \ref{mltFromPSDStress}.
% \end{proof}

% \begin{lemma}\label{lem:gcrvertexclose}
%     Let $G=(V,E)$ be any graph with $\gcr(G) = k$ and $|V| \leq k +2$.
%     Then $\mlt(G) =k$ also.
% \end{lemma}

% \begin{proof}
%     As $\gcr(G)=k$,
%     there exists a $(k-2)$-circuit $G'=(V',E')$ contained in $G$.
%     As $|V'| \leq |V| \leq k+2$,
%     then $\mlt(G') = k$ by Lemma \ref{lem:smallcirc}.
%     The result now follows as $\mlt(G') \leq \mlt(G) \leq \gcr(G)$.
% \end{proof}

%Proof for missing 5 edges
% \begin{proof}[Proof of Theorem \ref{t:manyedges}]
%     The graph $G$ is $(n-4)$-dependent as
%     \begin{align*}
%         |E| \geq \binom{n}{2} -5 > (n-4)n - \binom{n-3}{2},
%     \end{align*}
%     hence $\gcr(G) \geq n-2$.
%     The result now follows from Lemma \ref{lem:gcrvertexclose}.
% \end{proof}





%\subsection{$d$-circuits with $d+5$ vertices}

%SEAN: Not needed, mentioned in Theorem \ref{THM:SMALL}
% \begin{lemma}\label{lem:flexiblecirc}
%     Let $G=(V,E)$ be a flexible $d$-circuit with $|V| \leq 9$ for some $d \in \{3,4\}$.
%     Then $\mlt(G)=\gcr(G)=d+2$.
% \end{lemma}

% \begin{proof}
%     By checking the flexible 3- and 4-circuits on at most 9 vertices as characterised in \cite{grasegger2020flexible},
%     we have that $G$ is a $k$-sum of two smaller $d$-circuits for some $k \leq d-1$.
%     The result now follows from Lemma \ref{lem:cird3} and \textcolor{red}{(REF NEEDED $k$-sums preserve PSD stresses)}.
% \end{proof}



%\subsection{Graphs with at most 9 vertices}

%SEAN: Not needed, result added to Theorem \ref{THM:SMALL}
% \begin{lemma}\label{lem:5con3cir}
%     (a) There are no 3-rigid 3-circuits with 9 vertices or less with minimum degree 5.
    
%     (b)  All 4-rigid 4-circuits with minimum degree of at least 6 and 9 or less vertices have exactly 9 vertices, and are 6-regular and globally 4-rigid.
% \end{lemma}

% \begin{proof}
%     (a) Suppose for contradiction that there does exist a 3-rigid 3-circuit $G=(V,E)$ with $|V|\leq 9$ and $\delta(G) \geq 5$.
%     Then $3|V|-5 = |E| \geq 5|V|/2$, which implies that $|V| \geq 10$.
    
%     (b)    \textcolor{green}{TO DO -- Finish and add figure of graphs.}
    
%     Suppose that $G =(V,E)$ is a 4-rigid 4-circuit with $\delta(G) \geq 6$ and $|V|\leq 9$.
%   Then $4|V|-9 = |E| \geq 3|V|.$
%     It follows that $|V|=9$ and $G$ is 6-regular.
%     There are only four 6-regular graphs on 9 vertices (see Figure XXX)
%     and we can easily check that all four graphs are globally 4-rigid by giving specific realisations with maximum rank stresses. ADD these as an appendix?
% \end{proof}


%\begin{lemma}\label{lem:6con4cir}
%    All 4-rigid 4-circuits with minimum degree of at least 6 and 9 or less vertices have exactly 9 vertices, and are 6-regular and globally 4-rigid.
%\end{lemma}

%\begin{proof}
 %   \textcolor{green}{TO DO -- Finish and add figure of graphs.}
    
 %   Suppose that $G =(V,E)$ is a 4-rigid 4-circuit with $\delta(G) \geq 6$ and $|V|\leq 9$.
  % Then $4|V|-9 = |E| \geq 3|V|.$
 %   It follows that $|V|=9$ and $G$ is 6-regular.
  %  There are only four 6-regular graphs on 9 vertices (see Figure XXX)
    %the complement of a 9-cycle, the complement of two disjoint cycles of length 4 and 5, the complement of two disjoint cycles of length 3 and 6, and the complement of 3 disjoint 3-cycles.
 %   and we can easily check that all four graphs are globally 4-rigid by giving specific realisations with maximum rank stresses. ADD these as an appendix?
%\end{proof}

% We are now ready to prove Theorem \ref{THM:SMALL};
% i.e., maximum likelihood threshold and generic completion rank agree for graphs with at most 9 vertices.

% \begin{proof}[Proof of Theorem \ref{THM:SMALL}]
% 	Choose any graph $G$ with $|V| \leq 9$ and $\gcr(G) = n$.
% 	If $\gcr(G) \leq 4$ then $\mlt(G)=\gcr(G)$ by \textcolor{red}{(REF NEEDED Small GCR results)},
% 	and if $\gcr(G) \geq 7$ then $\mlt(G)=\gcr(G)$ by Theorem \ref{t:manyedges}.
% 	Hence we may suppose $5 \leq \gcr(G) \leq 6$.
	
% 	First suppose $\gcr(G)=5$.
% 	Then $G$ contains a 3-circuit $H$ with at most 9 vertices.
% 	If $H$ is 3-flexible then $\mlt(H) = 5$ by Lemma \ref{lem:flexiblecirc}.
% 	If $H$ is 3-rigid then $\mlt(H) \geq 5$ by Lemmas \ref{lem:5con3cir}(a), \ref{lem:d+5circcut} and \ref{lem:3d9circcut}.
% 	Hence $5 \leq \mlt(H) \leq \mlt(G) \leq \gcr(G) =5$.
	
% 	Now suppose $\gcr(G)=6$.
% 	Then $G$ contains a 4-circuit $H$ with at most 9 vertices.
% 	If $H$ is 4-flexible then $\mlt(H) = 6$ by Lemma \ref{lem:flexiblecirc}.
% 	If $H$ is 4-rigid then $\mlt(H) \geq 5$ by Lemma \ref{lem:d+5circcut} if $\delta(H)=5$, or Lemma \ref{lem:5con3cir}(b) and Theorem \ref{rigidityBounds} if $\delta(H) >5$.
% 	Hence $6 \leq \mlt(H) \leq \mlt(G) \leq \gcr(G) =6$.
% \end{proof}

%Theorem \ref{THM:SMALL} cannot be improved upon as $K_{5,5}$ has 10 vertices but it can be shown that $4=\mlt(K_{5,5}) < \gcr(K_{5,5})=5$;
%\textcolor{red}{(REF NEEDED either have as example earlier or reference the paper where this is proven)}.












\section{Weak maximum likelihood threshold}\label{sec: weak MLT}
This section includes connections between the \emph{weak} maximum likelihood threshold of a graph, and two areas of classical combinatorics: partially ordered sets, and graph dimension (i.e.~the minimum dimension in which a graph can be realized as a unit-distance graph).

\begin{defn}\label{def: wmlt}
The \emph{weak maximum likelihood threshold} of a graph $G$, denoted 
$\wmlt(G)$ is the 
smallest number of samples\footnote{Again, we are assuming that the samples are i.i.d.~from a distribution whose probability measure is mutually absolutely continuous with respect to Lebesgue measure.} required for 
the MLE of the Gaussian graphical model associated with $G$ to exist
with positive probability.
\end{defn}
The definition of $\wmlt(G)$ is the same as that of $\mlt(G)$, but with the phrase ``almost surely'' swapped out for ``with positive probability.'' 
Arguments along the lines of Section \ref{sec: lifting} then yield
the analogue of Theorem \ref{thm: main mlt lift}.
Since the proof is very similar, we skip it.

\begin{prop}\label{prop:wmlt liftable}
Let $G$ be a graph with $n$ vertices.  The WMLT of $G$ is $d+1$
if and only if $d$ is the smallest 
dimension such that some generic $d$-dimensional framework $(G,p)$
is liftable.  
\end{prop}

The following implies that we can ignore genericity of our witness (cf.~\cite[Definition~5.1]{gross2018maximum}).

% \begin{proof}
%     Lemma~\ref{lem: cone lift} implies that the cone framework $(v_0*G,\hat{p})$ in $\mathbb{R}^{d+1}$ is liftable. Lemma~\ref{lem: cone graph lift} then implies that the MLT matrix completion problem for the rank-$(d+1)$ matrix $P^TP$ is feasible, where the columns of $P$ are the elements of a slicing of $\hat{p}$.
% \end{proof}


% The following alternate characterization of $\wmlt(G)$ will be easier to work with.

\begin{prop}%[\cite{gross2018maximum}]\label{prop: wmlt matrix completion}
\label{prop: wmlt matrix completion}
Let $d\in \NN$ be a dimension and $G$ be a graph with $n\ge d+1$ vertices.  
If there is any liftable $d$-dimensional framework $(G,p)$ then there 
is a generic liftable $d$-dimensional framework.  In particular, 
$\wmlt(G) \le d+1$.

% {\color{gray}
%     Given a graph $G$, $\wmlt(G)$ is the smallest $r$ such that there exists a PSD matrix $A$ of rank $r$ such that the MLT matrix completion problem $(G,A)$ is feasible.}
\end{prop}
\begin{proof}
Let $(G,p)$ be a liftable $d$-dimensional framework.  By Lemma 
\ref{lem: psd lift}, $(G,p)$ does not have a non-zero PSD equilibrium 
stress.  By lower semi-coniuity of the rank of the rigidity 
matrix, there is a nbd $U$ of $p$ so that if $q\in U$, the space of 
equilibrium stresses of $(G,q)$ has dimension at most that of $(G,p)$.
Hence any equilibrium stress of $(G,q)$ is a small perturbation of a 
stress of $(G,p)$.  For sufficiently small perturbations, signature is
preserved, so some neighborhood of $p$ consists of only frameworks
without non-zero PSD equilibrium stresses.  This neighborhood 
contains a generic framework.
The second statement follows from Proposition \ref{prop:wmlt liftable}.
\end{proof}


% LST comment: this is fishy.  
% \begin{proof}
%     Let $n$ be the number of vertices of $G$.
%     By results in~\cite{dempster1972covariance}, $\wmlt(G)$ is the minimum $r$ such that there exists an open set $U \subseteq \mathbb{R}^{n\times r}$ such that for all $X \in U$, the MLT matrix completion problem $(G,XX^T)$ is feasible.
%     Since the interior of the PSD cone is open, this is equivalent to the existence of a single matrix $A$ that is PSD of rank $r$ such that the MLT matrix completion problem $(G,A)$ is feasible.
% \end{proof}

% The following proposition gives us a slightly more work
% By exploiting Dempster's characterization of when the maximum likelihood estimate exists~\cite{dempster1972covariance}, and the fact that $\mathcal{S}^n_{++}$ is open, this is equivalent to the following.

% \begin{defn}
%     The \emph{weak maximum likelihood threshold} of a graph $G = ([n],E)$, denoted $\wmlt(G)$, is the smallest $r$ such that
%     there exists a positive semidefinite matrix $A$ of rank $r$ and a positive definite matrix $B$ such that $A_{ij} = B_{ij}$ whenever $i=j$ or $ij \in E$.
% \end{defn}

\subsection{Existing bounds on the WMLT}
The weak maximum likelihood threshold of a graph is one 
if and only if it has no edges. Examples of graphs for which MLT = WMLT = $d+1$ are the \emph{$d$-laterations}; i.e.,
graphs formed from $K_{d+1}$ by a sequence of $d$-dimensional 0-extensions.
Other than this, very little is known.
Gross and Sullivant~\cite{gross2018maximum} showed that $\wmlt(G)$ is at most the chromatic number of $G$.
Buhl~\cite{buhl1993existence} characterized the weak maximum likelihood thresholds of cycles, showing that $\wmlt(G) = 3$ if $G$ is a three-cycle, and $\wmlt(G) = 2$ when $G$ is a cycle of length four or greater.
Gross and Sullivant~\cite{gross2018maximum} use Buhl's results on cycles to show that if $\wmlt(G) = 2$,
then $G$ satisfies a property they call \emph{Buhl's cycle condition}, which is actually equivalent to the existence of an orientation of the edges of $G$ making it into the diagram of a partially ordered set.
% We will show how this result follows from some known results on PSD stresses of frameworks on the line.

% \begin{prop}\label{prop:wmlt liftable}
%     Let $G$ be a graph with at least $d+1$ vertices such that there exists a liftable framework $(G,p)$ in $\mathbb{R}^d$.
%     Then $\wmlt(G) \le d+1$.
% \end{prop}
% \begin{proof}
%     Lemma~\ref{lem: cone lift} implies that the cone framework $(v_0*G,\hat{p})$ in $\mathbb{R}^{d+1}$ is liftable. Lemma~\ref{lem: cone graph lift} then implies that the MLT matrix completion problem for the rank-$(d+1)$ matrix $P^TP$ is feasible, where the columns of $P$ are the elements of a slicing of $\hat{p}$.
% \end{proof}

\begin{defn}
    Given a directed graph, a cycle in the underlying undirected graph is \emph{stretched} if it is of the form $v_1\rightarrow v_2 \rightarrow \dots \rightarrow v_k \leftarrow v_1$.
    Given $(G,p)$ is a framework in $\mathbb{R}^1$ with no edges of length zero, a cycle in $G$ is \emph{stretched} if the corresponding cycle is stretched in the orientation of $G$ obtained by directing each edge $i$ 
    $j$ towards $j$ if $p(j) > p(i)$ and otherwise toward $i$.
\end{defn}

A graph with an orientation free of stretched cycles was said to satisfy \emph{Buhl's cycle condition} by Gross and Sullivant~\cite{gross2018maximum}.

The following proposition can be seen as the rigidity-theoretic version of~\cite[Theorem 4.3]{buhl1993existence}, Buhl's characterization of which datasets with two observations have a maximum likelihood 
estimate for the Gaussian graphical model corresponding to a
cycle. It is well-known among researchers who study universal rigidity.
\begin{prop}\label{prop:stretchedCycleStress}
    Let $G$ be a cycle and let $(G,p)$ be a generic framework in $\mathbb{R}^1$.
    Then $(G,p)$ has a PSD equilibrium stress if and only if it is a stretched cycle.
\end{prop}
It seems difficult to locate a published proof, and, in 
fact, this proposition follows from a more general 
statement due Kapovich and Millson \cite{kapovich}
which we discuss in Appendix~\ref{appendix: cycle stress signature}.

Proposition~\ref{prop:stretchedCycleStress} immediately 
implies the following result of Gross and Sullivant.

\begin{cor}[{\cite[Corollary 5.4]{gross2018maximum}}]\label{cor: no stretched cycles}
    If $\wmlt(G) = 2$, then $G$ has an acyclic orientation with no stretched cycles.
\end{cor}


\subsection{A conjecture and a connection}
Based on extensive computations, we believe that the converse to Corollary~\ref{cor: no stretched cycles} is true, as stated in the following conjecture.

\begin{conj}\label{conj: wmlt 2}
    If $G$ has at least one edge and an acyclic orientation with no stretched cycles, then $\wmlt(G) = 2$.
\end{conj}

Directed acyclic graphs with no stretched cycles are well-studied objects in combinatorics: they are  diagrams
of partially ordered sets. It is NP-hard to determine whether a given undirected graph has an acyclic orientation with no stretched cycles~\cite{brightwell1993complexity}. Thus Conjecture~\ref{conj: wmlt 2} would imply that the decision problem of whether a given graph has $\wmlt(G) = 2$ is NP-hard. Via the coning construction \cite{W83}, 
this would imply that determining weak MLT is NP-hard in general.

The following definition is due to Erd\"os, Harary, and Tutte.

\begin{defn}[\cite{erdos1965dimension}]
The \emph{dimension} of a graph $G$, denoted $\dim(G)$, is the minimum 
$d$ such that there exists a framework $(G,p)$ in $\mathbb{R}^d$ such 
that $\|p(i)-p(j)\| = 1$ for all edges $ij \in E(G)$.
\end{defn}

The \emph{Hadwiger-Nelson problem} is a longstanding open problem in
combinatorics which asks for the maximum chromatic number of a graph 
$G$ with $\dim(G) = 2$. See~\cite{de2018chromatic} for the most 
recent progress and a brief account of the history. The connection 
to weak maximum likelihood thresholds is given by the following.


\begin{prop}
    Let $G$ be a graph.
    Then $\wmlt(G) \le \dim(G)+1$.
\end{prop}
\begin{proof}
Let $(G,p)$ be a framework in $\mathbb{R}^{\dim(G)}$ so that every 
edge of $G$ has length $1$. Then $(G,p)$ is liftable. 
A suitable witness is the framework $(G,q)$ in 
$\mathbb{R}^{n-1}$ where the $q(i)$s are the vertices of a 
suitably scaled unit simplex. The result now follows 
from Proposition~\ref{prop:wmlt liftable}.
\end{proof}
It is well-known that $\dim(G) + 1 \le \chi(G)$.  Indeed, if $G$ 
has chromatic number $d+1$, then there is a unit-distance embedding 
of $G$ in dimension $d$ by putting each of the $d+1$ 
color classes on a distinct vertex of a regular simplex in 
dimension $d$.  Hence, this result improves the 
inequality $\wmlt(G) \le \chi(G)$ from \cite{gross2018maximum}.



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Example with multiple Appendixes:        %%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{appendix}

\section{Appendix: ``almost all'' vs ``generic''}\label{appendix: generic}
In this appendix, we prove some technical 
results needed for Theorem \ref{thm: main mlt stress}.
We begin with a precise definition of genericity.

\begin{defn}
    A point $x \in \mathbb{R}^n$ is \emph{generic} if its coordinates are algebraically independent over $\mathbb{Q}$.
    If $S \subseteq \mathbb{R}^n$ is an irreducible semi-algebraic set, then a point $x \in S$ is \emph{generic in $S$}
    if whenever a polynomial $f$ with rational coefficients satisfies $f(x) = 0$, then $f(y) = 0$ for all $y \in S$.
%    If $S \subseteq \mathbb{R}^n$ is reducible, then $x \in S$ is generic in $S$ if its generic in an irreducible component of $S$.
\end{defn}

We record some facts about semi-algebraic sets (see,
e.g.~\cite{bochnak,stasica}). Recall that a \emph{finite boolean combination} of sets $\{S_\alpha\}_{\alpha \in J}$
is a set obtained using finitely many unions and intersections of sets in $\{S_\alpha\}_{\alpha \in J}$.

\begin{lemma}\label{lem: semi-alg facts}
Let $S$ be an irreducible semi-algebraic set and $X\subseteq S$
%irreducible and 
semi-algebraic. Then:
\begin{enumerate}[(a)]
    \item $X$ is a finite boolean combination of open and closed (standard topology) subsets of $S$,
    \item $X$ contains an open subset of $S$ if and only if it has the same dimension as $S$,
    \item if $X$ is of lower dimension than $S$, then each $x \in X$ satisfies some polynomial with coefficients in the field of definition for $X$ that is not satisfied by some points in $S$, and
    \item $X$ has finitely many irreducible components.
\end{enumerate}
\end{lemma}

\begin{lemma}\label{lem: semi-alg measure}
Let $S\subseteq \RR^N$ be an irreducible semi-algebraic 
set, $X\subseteq S$ semi-algebraic, and suppose that $\mu$
is a Borel measure on $S$ that is mutually absolutely 
continuous with respect to Lebesgue measure on $S$.
Then $X$ is $\mu$-null if and only if every irreducible component
of $X$ is of lower dimension than $S$.
\end{lemma}

\begin{proof}
From Lemma \ref{lem: semi-alg facts} and the fact that $\mu$
is a Borel measure, we know that each irreducible component $Y$
of $X$ is measurable.  Since $\mu$ is a  
Borel measure and Lebesgue measure on $S$ is absolutely 
continuous with respect to $\mu$, if $Y$ contains an open subset of 
$S$, $\mu(Y) > 0$.  Hence, if $Y$ has the same dimension as
$S$, we must have $\mu(Y) > 0$.  On the other hand, if 
$Y$ is of lower dimension then the 
(standard topology)
closure 
$\overline{Y}$ is closed and nowhere dense.  Absolute continuity of $\mu$
with respect to Lebesgue measure
then implies that $\mu(Y) \le \mu(\overline{Y}) = 0$.
Repeating this argument for each irreducible component
of $X$ completes the proof.
\end{proof}

To translate between generic statements 
and measure theoretic ones, we use the following.

\begin{lemma}\label{lem: semi-alg generic}
Let $S$ be an irreducible semi-algebraic subset of $\RR^N$ and let $X$ be 
a semi-algebraic subset of $S$, with both $S$ and $X$ defined over $\QQ$.
Let $\mu$ be a Borel measure on $S$ mutually absolutely
continuous with respect to Lebesgue measure.
Then:
\begin{enumerate}[(a)]
    \item if $X$ is $\mu$-null, then no generic points of $S$ are in $X$,
    \item if $X$ has full $\mu$-measure, then every generic point of $S$ is in $X$, and
    \item if neither $X$ nor its complement are $\mu$-null, then some generic points of $S$ are in $X$ and some are not.
\end{enumerate}
\end{lemma}
\begin{proof}
Suppose, for the moment, that $X$ is 
irreducible.  By Lemma \ref{lem: semi-alg measure} if $X$ is $\mu$-null 
it is of lower dimension than $S$.  By Lemma \ref{lem: semi-alg facts},
no point of $X$ can be generic.
In general, we repeat the argument for each irreducible component, 
which gives (a).  Part (b) follows from (a) via complementation.

For (c), Lemma \ref{lem: semi-alg measure} implies that a $\mu$-non-null
semi-algebraic set contains an open set.  Any non-generic point 
must lie in a nowhere dense algebraic subset of $S$, so if both $X$
and its complement are $\mu$-non-null both contain a generic point.
\end{proof}

\begin{lemma}\label{lem: gen slicing}
Let $v$ be a generic configuration of $n$ vectors in
$\RR^{d+1}$.  Then $v$ is flattenable, and the flattened
configuration $p$ in $\RR^d$ is also generic.
Conversely, if $p$ is a generic configuration of $n$ 
points in $\RR^d$, then there is a generic vector configuration 
$v$ in $\RR^{d+1}$ so that $p$ is the flattening of $v$.
\end{lemma}

\begin{proof}
First suppose that $v$ is a generic configuration of $n$
vectors in $\RR^{d+1}$.  Letting $t_i$ be the last coordinate 
of $v(i)$, we notice that if $t_i = 0$ for any $i$, 
then $v$ satisfies a non-trivial polynomial equation 
and so is non-generic.  Hence, $v$ is flattenable.  
The map sending a flattenable vector configuration 
$v$ to its flattening $p$ is rational and surjective
onto configurations of $n$ points in $\RR^d$.
The result now follows from \cite[Lemmas 2.7 and 2.8]{gortler2010characterizing}.
\end{proof}

\section{Appendix: Equilibrium stresses and convexity}\label{sec:sep}

The goal of this appendix is to give a self-contained proof of Lemma~\ref{lem: psd lift},
which originally appeared in~\cite{alfakih2011bar}.
We will denote the interior of a set $S$ by $\intr(S)$.

\begin{lemma}
\label{lem:convProj}
Let $K$ be a convex $n$-dimensional set in $\RR^n$,
let $\pi$ be a rank-$m$ linear projection from $\RR^n$ to $\RR^m$, and
let $k:=\pi(K)$ be the $m$-dimensional image.
The following are equivalent:
\begin{enumerate}[(a)]
    \item 
$\pi^{-1}(x) \cap \intr(K)$ is nonempty,
\item $x  \in \intr(k)$, and
\item  $x$ does not lie on a supporting hyperplane for $k$.
\end{enumerate}
\end{lemma}
\begin{proof}
Equivalence of the latter two conditions follows from the supporting hyperplane theorem \cite[Ch. 8]{simon-convexity}.

If $\pi^{-1}(x) \cap \intr(K)$ is nonempty, then there is a point $X \in \pi^{-1}(x)$ with open neighborhood $N$ satisfying
$N \subseteq \intr(K)$. Because $\pi$ is a linear 
map it is open onto its image, which is $\RR^m$,
so $\pi(N)$ is open.  Since $x\in \pi(N) \subseteq k$, 
it is interior in $k$ (here we used that $K$ is full-dimensional, 
so that $\intr(K)$ is open and nonempty in $\RR^n$).


Now assume $\pi^{-1}(x) \cap \intr(K) = \emptyset$.
Since $\pi^{-1}(x)$ is convex,  
there must be an affine
hyperplane $H$ in $\RR^n$
weakly separating $\pi^{-1}(x)$ from $\intr(K)$.  
Since $\pi^{-1}(x)$ is an affine subspace, we have 
$\pi^{-1}(x) \subseteq H$.
Let $\ell$ be the linear functional and $\alpha$ the real number so that
\[
    H = \{y\in \RR^N : \ell(y) = \alpha\}.
\]
Since $\pi^{-1}(x)$ is parallel to the kernel of 
$\pi$, we have that $\ker \ell \supseteq \ker \pi$.
Hence, we have a well-defined linear map 
$\overline{\ell} : \RR^m\cong \RR^n/\ker \pi \to \RR$ given 
by 
\[
    \overline{\ell}(x') = \ell(y') \qquad \text{(any $y'\in \pi^{-1}(x')$)}.
\]
Hence, since $H$ supports $K$, the hyperplane $\{y \in \mathbb{R}^m: \overline{\ell}(y) = \alpha\}$ supports $k$ at $x$.
\end{proof}


% {\color{gray} old version of previous lemma, with proof:
    
%     \begin{lemma}
%         The following are equivalent:
%         \begin{itemize}
%             \item $x \in k$ lifts
%             \item $x\in \intr(k)$
%             \item $x$ does not lie on a supporting hyperplane for $k$.
%         \end{itemize}
%     \end{lemma}
% \begin{proof}
% If $x$ lifts, then by definition, there is a point $X$
% which is in the fiber and in some open neighborhood 
% $N \subseteq \intr(K)$. Because $\pi$ is a linear 
% map it is open onto its image, 
% so $x \in \pi(N) \subseteq \intr(k)$ (here, we need that $K$ is 
% full dimensional, so $N$ is open in $\RR^N$).

% If $x$ does not lift, then there is no intersection
% between the fiber, $\pi^{-1}(x)$, and the 
% open convex
% set $\intr(K)$. Since the fiber is convex,  
% there must be an affine
% hyperplane and associated linear functional in $\RR^N$
% weakly separating $\pi^{-1}(x)$ from $\intr(K)$.
% Since the fiber is an affine set, this also means that 
% $\pi^{-1}(x) \subseteq H$. This inclusion
% gives us a well defined
% functional over fibers of $\pi$, which also 
% corresponds, under $\pi$, to 
% a well defined hyperplane and linear functional in $\RR^n$ {\color{red} what if $\pi$ is the projection onto $H$?}.
% Downstairs, this hyperplane also supports $k$ {\color{red}why is this true?} and contains $x$.
% This places $x$ on the boundary of $k$.
% \end{proof}

% }

\begin{proof}[Proof of Lemma~\ref{lem: psd lift}]
Let $K$ be the PSD cone.
Points in $K$ are Gram matrices of
$n$-point configurations in $\RR^n$; points in 
the interior correspond to configurations with 
$n$-dimensional linear span. Such configurations 
will have an $n-1$-dimensional affine span.
Fixing a graph $G$ with $m$ edges,
$\pi$ will be the map to $\RR^m$, which measures the 
squared lengths of the corresponding framework; i.e.~indexing $\mathbb{R}^m$ by the edges of $G$,
for each edge $ij$ of $G$, we have
\[
    \pi(X)_{ij} = X_{ii} + X_{jj} - 2X_{ij}.
\]
The image $\pi(K)$ is an $m$-dimensional convex cone $k \subseteq \mathbb{R}^{m}$.
Using Lemma~\ref{lem:convProj}, it now suffices to show that $\pi(p)$ lies on the boundary of $k$ if and only if $(G,p)$ has a PSD equilibrium stress.

Given a configuration $q$ of $n$ points in $\mathbb{R}^n$,
let $q^{l}$ denote the vector $q(1)_l,\dots,q(n)_l$ consisting of the $l^{\rm th}$ coordinate of each point in $q$.
Now assume $\pi(p)$ lies on the boundary of $k$,
let $\omega$ be the normal vector of the hyperplane tangent to $k$ at $\pi(p)$, and let $\Omega$ be the matrix obtained by setting $\Omega_{ij} = \Omega_{ji} = -\omega_{ij}$ for all edges $ij$ of $G$, $\Omega_{ii} = \sum_{j} \omega_{ij}$ for $i = 1,\dots, n$, and all other entries zero.
This means that for any configuration $q$ of $n$ points in $\mathbb{R}^n$,
the following inequality holds, and is moreover an equality when $q = p$:
\begin{align}\label{eq: supporting hyperplane configuration}
0 \le  
 \sum_{ij {\rm \ edge \ of \ } G} \omega_{ij} ||(q_i-q_j)||^2 =
\sum_{l} (q^l)^T\Omega q^l.
\end{align}
This implies that $\Omega$ is PSD and that $(p^l)^T\Omega p^l = 0$ for all $l$.
Together, these imply that $\Omega p^l = 0$ for each $l$, which is exactly the condition for $\omega$ to be an equilibrium stress of $p$.
Thus $\omega$ is a PSD equilibrium stress for $p$.

Finally, note that if $\Omega$ is a PSD equilibrium stress of $p$, then the above arguments can be reversed to show that $\Omega$ defines a supporting hyperplane of $k$ at $p$.
\end{proof}

% The incidence condition means that 
%  	\begin{align*}
%     \sum_{ij} \omega_{ij} ||(p_i-p_j)||^2=0.
% 	\end{align*}
% This energy can be written using the 
% $n$-by-$n$, non-zero 
% stress matrix $\Omega$
% corresponding to the stress vector $\omega$ as
%  	\begin{align*}
% \sum_{k} (p^k)^T\Omega p^k=0,
% 	\end{align*}
% where the superscript $k$ represents each of the $d$ spatial 
% coordinates. By construction, the all-ones vector is in the
% kernel of $\Omega$.

% The supporting condition means that for all configurations $q$ 
% in any dimension, we have
% \begin{align*}
% 0 &\le  
%  \sum_{ij} \omega_{ij} ||(q_i-q_j)||^2 \\
% &=
% \sum_{k} (q^k)^T\Omega q^k. 
% \end{align*}
% This means that $\Omega$ must be PSD.
% Going back to $p$, this means that 
% for all $k$, we have
%  	\begin{align*}
% \Omega p^k=0
% 	\end{align*}
% which is the condition of an equillibrium stress matrix.

% In this context, Lemma~\ref{lem:convProj} says that either $p$ is 
% equivalent to a framework with an $n-1$-dimensional span, or it
% has a non-zero PSD equillibrium stress matrix.



\section{Appendix: the signature of a cycle stress}\label{appendix: cycle stress signature}
\begin{defn}
    Let $C_n$ denote the directed cycle on vertex set $\{1,\dots,n\}$ with
    edges $1\rightarrow 2, 2\rightarrow 3,\dots,(n-1)\rightarrow n, n\rightarrow 1$.
    A \emph{framework} $(C_n,p)$ on $C_n$ refers to a framework on the undirected graph underlying $C_n$.
    In a general position framework $(C_n,p)$ in $\mathbb{R}^1$, an edge $i \rightarrow (i+1)$ is \emph{forwards} if $p(i) < p(i+1)$ and \emph{backwards} otherwise.
\end{defn}

Note that every general position framework $(C_n,p)$ in $\mathbb{R}^1$ has at least one forwards edge and at least one backwards edge.
Proposition~\ref{prop:stretchedCycleStress} is a corollary of the following, which classifies the signatures of the stresses of cycles in $\RR^1$.

\begin{thm}[\cite{kapovich}]\label{thm: cycle stress}
Let $(C_n,p)$ be a generic framework in $\mathbb{R}^1$ and let $f$ be the number of forwards edges and $b$ the number of backwards edges.
Then, for every nonzero equilibrium stress matrix $\Omega$ of $(C_n,p)$, the signature of $\Omega$ is either $(f-1,2,b-1)$ or $(b-1,2,f-1)$.
\end{thm}

It is easy to see from Theorem~\ref{thm: cycle stress} that any cycle framework 
$(C_n,p)$ with exactly one backwards edge, or exactly one forwards edge, must be stretched and vice versa. Since the proof in \cite{kapovich} uses Hodge theory, we provide a linear-algebraic argument.



\begin{lemma}\label{lem: cycle stress signs}
Let $(G,p)$ be a general position framework in $\RR^1$ with the edge $\{1,n\}$, 
wlog (after cyclic relabeling) backwards and $p(n)$ the rightmost vertex.
Then $(G,p)$ has a unique, up to nonzero scaling, equilibrium stress $\omega$, and this scaling can be chosen such that every forward edge has positive coefficient and every negative edge has 
negative coefficient.
\end{lemma}
\begin{proof}
Without loss of generality, set the coefficient $\omega_{1,n}$ on the edge $\{1,n\}$ to 
$-1$.  Now walk, in cyclic order, starting from vertex $1$, 
solving the equilibrium condition locally, by setting 
$\omega_{i,1+1}$ to solve (indices taken cyclically):
\[
    \omega_{i,i+1}(p(i+1) - p(i)) = \omega_{i-1,i}(p(i) - p(i-1)).
\]
Notice that the sign changes whenever we switch from forwards to 
backwards edges, so we have the desired sign pattern.  General 
position implies that we do not get any zero coefficients.
We have, automatically, equilibrium at every vertex except, 
possibly $p(n)$.  To check that we have equilibrium, notice that, 
by induction, all the vectors $\omega_{i,i+1}(p(i+1) - p(i))$
have magnitude $|p(n) - p(1)|$ and that $\omega_{n-1,n}$ is 
positive.
\end{proof}
Our next lemma is a general fact that can be verified by 
direct computation.
\begin{lemma}\label{lem: stress energy cut}
Let $H$ be any graph and $\omega$ an equilibrium stress with associated matrix $\Omega$.
For any subset $S$ of vertices of $H$, let $x(S)$ be the characteristic vector of $S$.
Then 
\[
    x(S)^T\Omega x(S) = \sum_{\text{edges $ij$: $i\in S$, $j\notin S$}} \omega_{ij}.
\]
In particular, if $S$ is the set of 
vertices on one side of a cut consisting of edges with positive (resp negative) stress coefficients, then $x(S)$ has positive (resp negative) Rayleigh quotient.
\end{lemma}

\begin{proof}[Proof of Theorem \ref{thm: cycle stress}]
Let $(G,p)$ be as in the statement and $\Omega$ 
scaled as in Lemma \ref{lem: cycle stress signs}.  Uniqueness, up to nonzero scale,
of the equilibrium stress on $(G,p)$ implies this is 
possible.
Now recall that removing any two edges from a cycle determines a 
cut.  If we have $b$ backwards edges, $e_1, \ldots, e_b$, 
each of the cuts $\{e_1, e_j\}$ for $2\le j\le b$ gives 
rise to a collection of $b-1$ independent incidence vectors with negative
Rayleigh quotient, from Lemma \ref{lem: stress energy cut}.  
Hence $\Omega$ has at least $b-1$ negative eigenvalues.
Similarly, the $f$ edges $e'_1, \ldots, e'_f$ with positive stress
coefficients give $f-1$ independent incidence vectors with positive 
Rayleigh quotient.
Since $\Omega$ has a nullity of at least $2$, as an equilibrium 
stress matrix, the proof is complete.
\end{proof}




\section{Appendix: completing the proof of Theorem~\ref{THM:SMALL}}
\label{app:b}
We begin with the easiest of the missing pieces: a proof of Lemma~\ref{lemma: 6 regular}.

\begin{proof}[Proof of Lemma~\ref{lemma: 6 regular}]
    The complement of a $6$-regular graph on $9$ vertices is $2$-regular
    and there are exactly four isomorphism classes of $2$-regular graphs on $9$-vertices.
    In particular, these are the $9$-cycle, the disjoint union of a $6$-cycle and a $3$-cycle, the disjoint union of a $5$-cycle and a $4$-cycle, and the disjoint union of three $3$-cycles.
    
    In all four graphs let the vertex set be $\{v_1,v_2,\dots,v_9\}$. We define $G_1$ by taking the edge set of $K_9$ and deleting the 9-cycle with edges $v_1v_2,v_2v_3,\dots,v_8v_9,v_9v_1$. We define $G_2$ by taking the edge set of $K_9$ and deleting the 6-cycle with edges $v_1v_2,v_2v_3,\dots,v_5v_6,v_6v_1$ and the 3-cycle with edges $v_7v_8,v_8v_9,v_9v_7$. We define $G_3$ by taking the edge set of $K_9$ and deleting the 5-cycle with edges $v_1v_2,v_2v_3,\dots,v_4v_5,v_5v_1$ and the 4-cycle with edges $v_6v_7,v_7v_8,v_8v_9,v_9v_6$. Finally, we define $G_4$ by taking the edge set of $K_9$ and deleting the 3-cycle with edges $v_1v_2,v_2v_3,v_3v_1$, the 3-cycle with edges $v_4v_5,v_5v_6,v_6v_4$ and the 3-cycle with edges $v_7v_8,v_8v_9,v_9v_7$. 

    By~\cite[Theorem~1.3]{Bob05}, it suffices to show that each $G_i$ has an infinitesimally rigid realisation with a maximum rank stress. For $1\leq i \leq 4$ we define the framework $(G_i,p)$ in $\mathbb{R}^4$ by putting $p(v_1)=(0,0,0,0)$, $p(v_2)=(0,0,0,1)$, $p(v_3)=(0,0,4,-1)$, $p(v_4)=(0,2,3,5)$, $p(v_5)=(1,-1,0,-2)$, $p(v_6)=(1,3,7,0)$, $p(v_7)=(2,-4,-1,1)$, $p(v_8)=(-9,0,2,11)$ and $p(v_9)=(-3,3,1,6)$.
    Given these realisations it is simple for the reader to verify that the rigidity matrix has rank $4n-10=26$, that the cokernel of the rigidity matrix is 1-dimensional and that the stress matrix corresponding to any non-zero equilibrium stress of $(G_i,p)$ has rank $n-4-1=4$.
\end{proof}

We now move on to the next easiest missing piece: a proof of Lemma~\ref{lem:d+5circcut}. 
% This requires us to introduce the following terminology.
% \begin{defn}
%     A \emph{($d$-dimensional) $0$-extension} of a graph $G$ is the graph obtained from $G$ by adding a new vertex of degree $d$. A \emph{($d$-dimensional) $1$-extension} of $G$ is the graph obtained from $G$ by removing an edge $xy$, and adding a new vertex adjacent to $x$, $y$ and $d-1$ other vertices.
%     The inverse of these operations are called \emph{($d$-dimensional) $0$- and $1$-reductions}.
% \end{defn}
As discussed above 1-extensions (Def. \ref{def: 0-ext and 1-ext}) 
preserve global $d$-rigidity \cite{Bob05}. In fact one can preserve the existence of a PSD equilibrium stress of full rank \cite[Section 9]{Cquestions}. That proof can be adapted to obtain the following lemma.

\begin{lemma}\label{lem:1ext}
    Let $G=(V,E)$ a $d$-rigid graph that has a generic realisation $(G,p)$ in $\mathbb{R}^d$ with a PSD equilibrium stress $\omega$ with rank $|V|-d-2$.
	Suppose that $G'=(V',E')$ is a $d$-rigid $d$-circuit obtained from $G$ by a 1-extension.
	Then there exists a generic framework $(G',p')$ with a PSD equilibrium stress of rank at least $|V'|-d-2$.
\end{lemma}

We will also make repeated use of the following theorem of Jord{\'a}n. A graph is \emph{redundantly $d$-rigid} if it is $d$-rigid, and remains so after removing any edge.

\begin{thm}[{\cite[Theorem~3.2]{egres-20-01}}]\label{thm:tibor}
   Let $d \ge 1$, let $k \in \{3,4\}$ and let $G$ be a graph on $d+k$ vertices. 
   %For $d\geq 1$, let $G$ be a graph on at most $d+4$ vertices.
   Then $G$ is globally $d$-rigid if and only if $G$ is redundantly $d$-rigid and $(d+1)$-connected.
\end{thm}

We next prove Lemma~\ref{lem:d+5circcut}.
For disjoint vertex sets $A,B$ of a graph $G$,
we will denote the induced subgraph on the vertex set $A$ by $G[A]$,
the non-edges of $G$ by $E^c$,
the non-edges of $G$ induced on the set $A$ by $E^c[A]$,
and the set of non-edges of $G$ with one end in $A$ and the other in $B$ by $E^c(A,B)$.
The minimum degree of a graph $G$ will be denoted $\delta(G)$.
The set of neighbors of a vertex $v$ of $G$ will be denoted $N_G(v)$.
Given a set $V$ of vertices, $K(V)$ denotes the complete graph on vertex set $V$.
Given a subset $S$ of edges or vertices of $G$, we let $G-S$ denote the graph obtained by removing $S$.
Given graphs $G$ and $H$, $G+H$ denotes the graph whose vertex and edge sets are the unions of the vertex and edge sets of $G$ and $H$.

\begin{proof}[Proof of Lemma \ref{lem:d+5circcut}]
 %   We have two possibilities;
 %   either $G$ is $(d+1)$-connected,
  %  or $G$ is $d$-connected but not $(d+1)$-connected.
     First suppose $G$ is a $(d+1)$-connected $d$-rigid $d$-circuit with a vertex $v$ of degree $d+1$.
   Then $G-v$ is $d$-rigid.
    Since $G$ is $(d+1)$-connected and redundantly $d$-rigid,
    the graph $G'=G-v_0+K(N_G(v_0))$ must also be $(d+1)$-connected and redundantly $d$-rigid.
    By Theorem~\ref{thm:tibor},
    $G'$ is globally $d$-rigid,
    and hence by \cite[Lemma 4.1]{t1},
    $G$ is globally $d$-rigid.
    The result follows from Theorem \ref{thm: gen ur}.
    
    Now suppose $G$ is not $(d+1)$-connected.
    Since $G$ is $d$-rigid, there exists a separating set $C \subset V$ of size $d$.
    As $\delta(G)=d+1$,
    $G-C$ will have exactly two connected components $G[A],G[B]$ where $A=\{a_1,a_2\}$ and $B=\{b_1,b_2,b_3\}$. The complement $G^c$ of $G$ has exactly 9 edges. Since $K_{d+2}$ is not a subgraph of $G$, $G[C]$ is not complete. Since $|E^c(A, B)|=6$ it follows that 
   % The induced graph $G[S]$ cannot be complete as then $G[A \cup S]=K_{d+2}$ contradicting the fact that $G$ is a $d$-circuit. Hence the set $E^c[C]$ of non-edges with both ends in $C$ is non-empty.
    %As the complement graph $G^c$ has exactly 9 edges,
  $|E^c[B \cup C]|=3$ and $|E^c[C]| \in \{1,2,3\}$. 
    
    If $|E^c[C]|=1$ and $G[B]\cong K_3$ and wlog $b_1,b_2$ have degree $d+1$ in $G$ and are incident to edges of $E^C(B,C)$. We can apply a 1-reduction at $b_1$ and add the missing edge incident to $b_2$ to result in a smaller $d$-circuit. A similar argument applies if $G[B]$ has 2 edges. In both cases the resulting $d$-circuit has $d+4$ vertices and is not $(d+1)$-connected. Hence it is $H_d$.
    This case is completed by Lemma \ref{lem:1ext}.
    %$G[C]$ must contain $d-2$ vertices of degree $d-1$. By removing these vertices, we obtain a 2-circuit $G'$ that is the 2-sum of the 2-circuits $K_4$ and $K_5-\{e,f\}$ for disjoint $e,f$. By Lemma \ref{lem: 2d PSD circuit stress}, there exists a 2-dimensional generic realization with a PSD equilibrium stress. By observing where the zeroes must lie in the stress matrix, the PSD equilibrium stress must have rank 3. Since coning and sliding preserves the rank and signature of any equilibrium stress (see \cite{cgt2}), we now apply $d-2$ conings to obtain the required result.
    
    Now assume $|E^c[C]| \geq 2$.
    If three non-edges meet at a vertex $c \in C$,
    then $G[B \cup C -c]$ is isomorphic to $K_{d+2}$,
    contradicting that $G$ is a $d$-circuit.
    Hence there are not,
    and there exists a 1-reduction at $a_1$ followed by a 0-reduction at $a_2$ resulting in the graph $K_{d+3}-\{e,f\}$ where $e$ and $f$ do not share a vertex. The result now follows from Theorem~\ref{thm:tibor}, Theorem~\ref{thm: gen ur}, and Lemma~\ref{lem:1ext}.
    % Then $d_G(c)=d+1$, and exactly one of the three non-edges must have an end point $b \in B$; if not, then $G[B \cup C -c]$ is isomorphic to $K_{d+2}$ and $G$ is not a $d$-circuit.
    % It follows that we can apply a 1-reduction at $b$ to obtain $H_d$.
    % The unique equilibrium stress of any generic realization of $H_d$ must have rank 2.
    % The result now follows from Lemma \ref{lem:1ext}.
\end{proof}

For the remainder of the appendix we will prove Lemma \ref{lem:3d9circcut}.
%\begin{lemma}\label{lem:3d9circcut}
 %   Suppose $G=(V,E)$ is a 3-rigid 3-circuit with $|V| =9$.
 %   Then $\mlt(G) \geq 5$.
%\end{lemma}
We first deal with the case when $G$ is 4-connected.
In what follows, we make repeated implicit use of the fact that every vertex in a $d$-circuit has degree at least $d+1$.

\begin{lemma}\label{lem:3d9gr}
    Let $G$ be a 4-connected 3-rigid 3-circuit on 9 vertices.
    Then $G$ has a generic realization in $\mathbb{R}^3$ with a PSD equilibrium stress.
\end{lemma}

\begin{proof}
    A counting argument shows that $G$ has a vertex $v_0$ of degree 4.
    Since $G$ is a 3-circuit,
    there exist distinct vertices $x,y$ adjacent to $v_0$ such that $xy \notin E$. Let $G'$ be the result of the 1-reduction at $v_0$ that adds $xy$. Then $G'$ contains a 3-circuit $H$.
    
    If $|V(H)|=8$ then $H = G'$.
    The connectivity of $H$ is at least $3$ (as otherwise $G$ would not be 4-connected),
    hence by \cite{grasegger2020flexible} $H$ is 3-rigid.
    A counting argument shows that $\delta(G) = 4$.
    The result now follows from Lemmas \ref{lem:1ext} and  \ref{lem:d+5circcut}.
    
    If $|V(H)|=7$ then $G'$ is formed from $H$ by a 0-extension that adds a vertex $v_1$.
    Since $G$ is a 4-connected 3-circuit,
    $v_0$ and $v_1$ must be adjacent in $G$,
    and $v_1 \notin \{x,y\}$.
    We now note that $G$ can be formed from $H$ by two 1-extensions;
    the first will remove the edge $xy$ and connect the vertex $v_0$ to $N_G(v_0) -v_1 + u$ for some vertex $u \in V(H)$,
    and the second will remove the edge $uv_0$ and attach $v_1$ to all its neighbours in $G$. 
    Since $H_3$ has a 3-dimensional generic realization with a PSD equilibrium stress of rank 2 and any globally 3-rigid graph has a PSD equilibrium stress of rank 3 (Theorem \ref{thm: gen ur}),
    the result now follows from Lemmas~\ref{lem:1ext} and~\ref{lemma: H_n} and Theorem~\ref{thm:tibor}.
    
    If $|V(H)|=6$ then $H$ is globally 3-rigid by Theorem~\ref{thm:tibor}.
    Since $|E(G')|= 19$ and $|E(H)|=13$,
    $G'$ has 6 edges not in $H$.
    Given $a,b$ are the two vertices in $G' -V(H)$ with $a$ having equal or higher degree than $b$ in $G'$,
    one of the two possibilities must hold: (i) both $a$ and $b$ have degree 3 in $G'$,
    or (ii) $a$ has degree 4 in $G'$, $b$ has degree 3 in $G'$, and there exists an edge between $a$ and $b$.
    In both cases we have that $v_0 b \in E$, and in (i) we have $v_0a \in E$ also.
    In case (i) we must have distinct vertices $s,t \in V \setminus \{a,b,v_0,x,y\}$ adjacent to $a$ and $b$ respectively as otherwise $G$ would not be 4-connected. Hence in case (i) we can obtain $G$ from $H$ by three 1-extensions;
    the first to add $v_0$ attached to $x,y,s,t$ and the next to split two of the edges $v_0 s$ and $v_0 t$ and add the vertices $a,b$.
    If case (ii) holds then $G$ can be formed from $H$ by a 0-extension to add $b$ adjacent to its neighbours plus a vertex $w$ in the neighbourhood of $a$ in $G$,
    a 1-extension at $w b$ to add $a$,
    and a 1-extension at $xy$ to add $v_0$.
    In either case,
    the result will hold by Lemma \ref{lem:1ext} and Theorem \ref{thm: gen ur}.
    
    Finally,
    suppose $|V(H)|=5$,
    i.e.~$G'$ has a 5-clique. 
    Let $a,b,c$ be the three vertices in $G' -V(H)$.
    We will show that there exists a 1-reduction of $G$ at $a,b$ or $c$ resulting in a graph that does not contain a 5-clique,
    hence reducing the problem to one of the previous cases.
    We first note that $v_0$ can be adjacent to at most two of $a,b,c$ as $x,y \in V(H)$.
    If any of $a,b,c$ are adjacent to four vertices in $H$ then $G$ must contain either $K_6-\{e,f\}$ ($e,f$ independent) or $K_5$ which contradicts that $G$ is a 3-circuit.
    The 4-connectivity of $G$ implies that each of $a,b,c$ has a neighbour in $H$. If $a$ has exactly 1 neighbour in $H$ then $a$ is adjacent to $v_0$ and has degree 4. By a quick case analysis we can see that there is a 1-reduction at $a$ (in $G$) creating a graph with no 5-clique. 
   % if any of $a,b,c$ are adjacent to only two vertices in $H$ then $G$ will have a vertex of degree 3,
    Hence we may assume each of $a,b,c$ has either 2 or 3 neighbours in $H$.
    If all three have 3 neighbours in $H$ then $G$ would have a vertex of degree 3,
    hence we may assume $a$ has only two neighbours in $H$. If $a,b,c$ all have two neighbours in $H$ then we may assume that $av_0\notin E$ and hence $a$ has degree 4. As above, we can apply a 1-reduction at $a$ (in $G$) to create a graph with no 5-clique. Hence we may assume that $b$ has 3 neighbours in $H$. 
    If $c$ has 2 neighbours in $H$, then a quick case analysis shows that one of $a,b,c$ has degree 4 in $G$ and we again reduce that vertex instead of $v_0$. Lastly if $c$ has 3 neighbours in $H$, then $a$ certainly has degree 4 in $G$ (otherwise $G'$ would have too many edges) and we finish in the same manner. 
    %To preserve the correct number of edges, it follows that $ab,ac \in E(G')$ also.
    %\textcolor{red}{FINISH}
    %\textcolor{red}{SEAN: I feel like we can do something similar to what we were discussing recently to prove $G$ is globally 3-rigid.}
\end{proof}

We lastly deal with the case when $G$ is not 4-connected. It will be convenient to define a \emph{node} of $G$ to be a vertex of degree 4 and to use $N$ to denote the set of nodes of $G$.
We also define a \emph{deleted $k$-sum} of two graphs $G_1,G_2$ to be the graph obtained by gluing $G_1$ and $G_2$ along a common $k$-clique, then removing one edge from this common clique.

\begin{lemma}
    Let $G$ be a 3-rigid 3-circuit on 9 vertices with a separating set $C= \{c_1,c_2,c_3\}$.
    Then $G$ has a generic realization in $\mathbb{R}^3$ with a PSD equilibrium stress.
\end{lemma}

\begin{proof}
Let $A,B \subset V$ be chosen such that $|A|\leq|B|$, $A \cup B \cup C = V$,
$A \cap B= A \cap C = B \cap C = \emptyset$,
and there exist no edge joining $A$ and $B$.
As $G$ is a 3-circuit on 9 vertices,
either $|A|=|B|=3$, or $|A|=2$ and $|B|=4$.
Note that $C$ cannot be a clique, as this would imply either $G[A \cup C]$ or $G[B \cup C]$ is a 3-circuit.

Suppose that $G[B]$ is disconnected. Then $|B|=4$ and so $|A|=2$.
%\begin{claim}
%	If $A=\{a_1,a_2\}$ and $B=\{b_1,b_2,b_3,b_4\}$ and $G[B]$ is disconnected,
%	then $G$ has a 3-dimensional generic realization with a PSD equilibrium stress.
%\end{claim}
	Since 3-circuits have minimum degree at least 4, the only 3-circuit that satisfies the above conditions is the graph described in Figure \ref{fig:3k5s}(a).
	This graph can be formed by the union of three copies of $K_5$ glued at three vertices $\{c_1,c_2,c_3\}$ with two edges $c_1c_2,c_1c_3$ removed.
	By using a method similar to that of Section \ref{sec: gluing},
 	it can be shown that $G$ has a 3-dimensional generic realization with a PSD equilibrium stress\footnote{Since equilibrium stresses are invariant under affine transformations, we can find three generic frameworks $(K_5,p^1),(K_5,p^2),(K_5,p^3)$ with PSD equilibrium stresses $\omega^1,\omega^2,\omega^3$ respectively so that: (i) $p^1_{c_i}=p^2_{c_i}=p^3_{c_i}$ for each $i \in \{1,2,3\}$, (ii) $\omega^1_{c_1 c_2} + \omega^2_{c_1 c_2} + \omega^3_{c_1 c_2}=0$,
	(iii) $\omega^1_{c_1 c_3} + \omega^2_{c_1 c_3} + \omega^3_{c_1 c_3}=0$,
	and (iv) the framework $(G,p)$ formed by gluing all three frameworks at the vertices $c_1,c_2,c_3$ and deleting the edges $c_1c_2,c_1c_3$ is regular. The obtained framework will have a PSD equilibrium stress $\omega = \overline{\omega}^1 + \overline{\omega}^2 + \overline{\omega}^3$,
	where $\overline{\omega}^i$ is the extension of $\omega^i$ to the edges of $G + c_1c_2 + c_1 c_3$.}. Hence we may suppose both $G[A]$ and $G[B]$ are connected. 
 	
\begin{figure}[ht]
	\begin{center}
		\begin{tikzpicture}[scale=0.7]
			\node[vertex] (a1) at (0.866,-2.5) {};
			\node[vertex] (a2) at (-0.866,-2.5) {};
			
			\node[vertex] (b1) at (1.732,2) {};
			\node[vertex] (b2) at (2.6,0.5) {};
			
			\node[vertex] (c1) at (-1.732,2) {};
			\node[vertex] (c2) at (-2.6,0.5) {};
			
			\node[vertex] (m1) at (0,1) {};			
			\node[vertex] (m2) at (0.866,-0.5) {};
			\node[vertex] (m3) at (-0.866,-0.5) {};
	
			\draw[edge] (m1)edge(a1);
			\draw[edge] (m1)edge(a2);			
			\draw[edge] (m2)edge(a1);
			\draw[edge] (m2)edge(a2);			
			\draw[edge] (m3)edge(a1);
			\draw[edge] (m3)edge(a2);
			
			\draw[edge] (m1)edge(b1);
			\draw[edge] (m1)edge(b2);			
			\draw[edge] (m2)edge(b1);
			\draw[edge] (m2)edge(b2);			
			\draw[edge] (m3)edge(b1);
			\draw[edge] (m3)edge(b2);
	
			\draw[edge] (m1)edge(c1);
			\draw[edge] (m1)edge(c2);			
			\draw[edge] (m2)edge(c1);
			\draw[edge] (m2)edge(c2);		
			\draw[edge] (m3)edge(c1);
			\draw[edge] (m3)edge(c2);
			
			\draw[edge] (a1)edge(a2);
			\draw[edge] (b1)edge(b2);
			\draw[edge] (c1)edge(c2);
			
			\draw[edge] (m3)edge(m2);
			
\node [rectangle,draw=white, fill=white] (a) at (0,-4) {(a)};
		\end{tikzpicture}
\hspace{1.5cm}
\begin{tikzpicture}[very thick,scale=1]
	\node[vertex] (L1) at (-1,-0.5) {};
			\node[vertex] (L2) at (-1,0.5) {};
			\node[vertex] (C1) at (0,-1) {};
			\node[vertex] (C2) at (0,0) {};
			\node[vertex] (C3) at (0,1) {};
			\node[vertex] (R1) at (1,-1) {};
			\node[vertex] (R2) at (1,0) {};
			\node[vertex] (R3) at (1,1) {};
	
			\draw[edge] (L1)edge(C1);
			\draw[edge] (L1)edge(C2);
			\draw[edge] (L1)edge(C3);
			
			\draw[edge] (L2)edge(C1);
			\draw[edge] (L2)edge(C2);
			\draw[edge] (L2)edge(C3);
			
			
			\draw[edge] (L1)edge(L2);
			
			
			
			\draw[edge] (R1)edge(C1);
			\draw[edge] (R1)edge(C2);
			\draw[edge] (R1)edge(C3);
			
			\draw[edge] (R2)edge(C1);
			\draw[edge] (R2)edge(C2);
			\draw[edge] (R2)edge(C3);
			
			\draw[edge] (R3)edge(C1);
			\draw[edge] (R3)edge(C2);
			\draw[edge] (R3)edge(C3);
			
			\draw[edge] (R1)edge(R2);
			\draw[edge] (R2)edge(R3);
			\path[edge] (R1) edge [bend right] node {} (R3);	
			
\node [rectangle,draw=white, fill=white] (b) at (0,-2.5) {(b)};
	\end{tikzpicture}
	\end{center}
	\caption{(a) A graph formed from gluing three copies of $K_5$ at three vertices and then deleting two edges in their intersection. (b) A 3-rigid 3-circuit.}
	\label{fig:3k5s}
\end{figure}

\begin{claim}
	If $A=\{a_1,a_2,a_3\}$ and $B=\{b_1,b_2,b_3\}$,
	then $G$ has a 3-dimensional generic realization with a PSD equilibrium stress.
\end{claim}

\begin{proof}
	Note that $|E^c| = 14$ and $|E^c(A,B)| = 9$.
	If $|E^c[C]|=1$ then $G$ is a deleted 3-sum of two smaller graphs.
	The result now follows from \cite[Lemma 17(a)]{grasegger2020flexible}, Lemma \ref{lem: psd clique sum} and the fact that all 3-circuits on 7 or fewer vertices support a PSD equilibrium stress (see Lemma~\ref{lemma: d circuit d+4 vertices}).
	
	Now suppose $|E^c[C]| \in \{2,3\}$.
	Since $|A|=|B|$, we may assume, without loss of generality, that the number of non-edges with an end in $A$ is less than the number of non-edges with an end in $B$;
	we shall define these sets as $E^c_A := E^c[A \cup C] \setminus E^c[C]$ and $E^c_B := E^c[B \cup C] \setminus E^c[C]$.
	We now have three possible cases;
	$|E^c_A|=0$, $|E^c_A|=|E^c_B|=1$, or $|E^c_A|=1$ and $|E^c_B|=2$.
	
	Suppose $|E^c_A|=0$.
	Since $G[A \cup C]$ cannot be 3-dependent,
	we must have $|E^c_B|=2$ and $|E^c[C]|=3$.
	By checking the possible non-edge combinations,
	we note that either no vertex of $C$ is a node and $G$ can be formed from the 3-rigid 3-circuit described in Figure \ref{fig:3k5s}(b) by a 1-extension (and hence we are done by Lemmas \ref{lem:1ext} and \ref{lem:d+5circcut}),
	or $C$ contains a node adjacent to only one vertex in $B$.
	As the only graph that satisfies the latter condition contains a double-banana subgraph (i.e.~the flexible 3-circuit formed by the deleted 2-sum of two copies of $K_5$), which can be found by deleting the node in $C$, we are done by Lemma \ref{lem: psd clique sum}.
	
%	\begin{figure}[ht]
%	\begin{center}
%		\begin{tikzpicture}
%			\node[vertex] (L1) at (-1,-0.5) {};
%			\node[vertex] (L2) at (-1,0.5) {};
%			\node[vertex] (C1) at (0,-1) {};
%			\node[vertex] (C2) at (0,0) {};
%			\node[vertex] (C3) at (0,1) {};
%			\node[vertex] (R1) at (1,-1) {};
%			\node[vertex] (R2) at (1,0) {};
%			\node[vertex] (R3) at (1,1) {};
%	
%			\draw[edge] (L1)edge(C1);
%%			\draw[edge] (L1)edge(C3);
			
%			\draw[edge] (L2)edge(C1);
%			\draw[edge] (L2)edge(C2);
%			\draw[edge] (L2)edge(C3);
			
			
%			\draw[edge] (L1)edge(L2);
			
			
			
%			\draw[edge] (R1)edge(C1);
%			\draw[edge] (R1)edge(C2);
%			\draw[edge] (R1)edge(C3);
			
%			\draw[edge] (R2)edge(C1);
%			\draw[edge] (R2)edge(C2);
%			\draw[edge] (R2)edge(C3);
			
%			\draw[edge] (R3)edge(C1);
%			\draw[edge] (R3)edge(C2);
%			\draw[edge] (R3)edge(C3);
			
%			\draw[edge] (R1)edge(R2);
%			\draw[edge] (R2)edge(R3);
%			\path[edge] (R1) edge [bend right] node {} (R3);		
%		\end{tikzpicture}
%	\end{center}
%	\caption{A 3-rigid 3-circuit.}
%	\label{fig:cir1}
%\end{figure}
	
	Now suppose $|E^c_A|=|E^c_B|=1$ (and hence $|E^c[C]|=3$).
	If the non-edges in $E_A^c$ and $E_B^c$ share an end then $G$ will contain a double-banana subgraph, so we may assume otherwise.
 	By checking all the remaining non-edge combinations,
 	we see that we can always 1-reduction to a node in $A$ that adds an edge between vertices in $C$,
	then apply another 1-reduction to a node in $B$ that adds an edge between vertices in $C$,
	and end up with the graph $H_3$.
%  	that do not cause any vertex to have degree 3 or less or there to exist a $K_5$ subgraph,
% 	we see that there are three possibilities: (i) both $A$ and $B$ have a single node each, (ii) $A$ (respectively, $B$) has a single node and $B$ (respectively, $A$) has two nodes that are not adjacent, or (iii) both $A$ and $B$ have two nodes that are not adjacent.
	By Lemma \ref{lem: psd clique sum},
	$H_3$ has a PSD equilibrium stress,
	and by observation of the corresponding stress matrix we note it must have rank at least 2.
	The result now follows from Lemma \ref{lem:1ext}.
	
	Finally,
	suppose that $|E^c_A|=1$ and $|E^c_B|=2$ (and hence $|E^c[C]|=2$).
	By relabelling we may assume $c_1 c_2 , c_2 c_3 \in E^c[C]$ (i.e.~$c_1 c_3 \in E$) and $a_1$ is a node.
	If $a_1 c_2$ is a non-edge then $G[A \cup C]$ contains a copy of $K_5$,
	hence we may choose a non-edge $e \in \{c_1 c_2 , c_2 c_3\}$ so that both end points of $e$ are neighbours of $a_1$ in $G$.
	First suppose $G$ has two non-edges $b_i c_x, b_j c_x$ for distinct $b_i,b_j$.
	We must have $c_x \neq c_2$,
	as otherwise $G[B \cup C]$ will contain a copy of $K_5$.
	If $c_x$ is not a node, then $G$ is a deleted 3-sum of the globally 3-rigid graphs $K_6-\{e,f\}$ (see Theorem~\ref{thm:tibor}) and $K_5$;
	hence $G$ will have a PSD equilibrium stress by Lemma \ref{lem: psd clique sum}.
	If $c_x$ is a node then $G-c_x$ is the 2-sum of two copies of $K_5$;
	hence $G$ will have a PSD equilibrium stress by Lemma \ref{lem: psd clique sum}.
	Now suppose $G$ does not have two vertices in $B$ that are adjacent to the same vertex in the complement of $G$.
	Define $G' := G- a_1 +e$.
	If $E^c_B = \{b_i b_j , b_k c_\ell\}$ for distinct $i,j,k$,
	then the 1-reduction $G'-b_i + b_k c_\ell$ of $G'$ is $H_3$;
	hence the results follows from our previous observations of $H_3$ and Lemma \ref{lem:1ext}.
	If $E^c_B = \{b_i c_x, b_j c_y\}$ for distinct $i,j$ and distinct $x,y$,
	then $G'$ is the 3-sum of a copy of $K_5$ and the globally 3-rigid 3-circuit $K_{B \cup C} - E^c_B$ (see Theorem~\ref{thm:tibor}).
	Hence by Lemma \ref{lem: psd clique sum},
	$G$ has a PSD equilibrium stress.
\end{proof}



\begin{claim}
	If $A=\{a_1,a_2\}$ and $B=\{b_1,b_2,b_3,b_4\}$
	then $G$ has a 3-dimensional generic realization with a PSD equilibrium stress.
\end{claim}

\begin{proof}
	We note that $a_1a_2 \in E$ and $a_1c_i,a_2c_i \in E$ for each $i \in \{1,2,3\}$,
	as otherwise $a_1$ and $a_2$ would have a degree of 3 or less in $G$.
	If $G[C]$ has 3 edges, then $G[A\cup C]$ would be $K_5$ and so $G$ would not be a $3$-circuit.
	If $G[C]$ has 2 edges then $G$ is the 3-sum of $K_5$ and another 3-circuit with 7 vertices by \cite[Lemma 17(a)]{grasegger2020flexible},
	and hence $G$ will have a 3-dimensional generic realization with a PSD equilibrium stress by Lemmas \ref{lem: psd clique sum} and  \ref{lem:d+5circcut}.
	Suppose that $G[C]$ has either no edges or 1 edge.
	Applying a 1-reduction at either $a_1$ or $a_2$ and then applying a 0-reduction to the remaining vertex in $A$ is equivalent to deleting both $a_1$ and $a_2$ and adding an edge between two vertices in $C$. For brevity we refer to this process as an \emph{$A$-move}.
	
	Suppose that there exists an $A$-move that gives a graph with minimum degree 2.
	We can check all the possible cases where this happens by observing that $G$ has 6 non-edges with both ends in $B \cup C$,
	and at least two non-edges must have both ends in $C$.
	In every case we see that $G$ would contain either $K_5$ or $K_6- \{e,f\}$ as a subgraph, contradicting that $G$ is a 3-circuit.
	Hence we may assume that any $A$-move produces a graph with minimum degree~3.
	
	Now suppose that every $A$-move produces a graph with minimal degree 3.
	As $G$ is a 3-circuit,
	any vertex of degree 3 of $G'$ must lie in $C$.
	By checking the various assignments of non-edges between vertices in $B$ and $C$ we see that $G[C]$ must contain no edges;
	any possible graph where every $A$-move gives a graph with minimum degree 3 and $G[C]$ contains an edge would force $G$ to contain either $K_5$ or the 3-circuit $K_6-\{e,f\}$.
	This leaves the two possible 3-rigid 3-circuits given in Figure \ref{fig:amove}.
	The graph on the left has a vertex that we can apply a 1-reduction to so as to obtain the graph in Figure \ref{fig:3k5s}(b). We can verify that the claim holds for the remaining graph on the right in a similar manner as in Lemma~\ref{lemma: 6 regular}.\footnote{Let $G=(V,E)$ be the graph defined as follows. Put $V=\{a_1,a_2,b_1,b_2,b_3,b_4,c_1,c_2,c_3\}$ and   $E_2=\{a_1a_2,a_1c_1,a_1c_2,a_1c_3,a_2c_1,a_2c_2,a_2c_3,b_1b_2,b_1b_3,b_1b_4,b_2b_3,b_2b_4,b_3b_4,b_1c_1,b_1c_2,b_2c_1,b_2c_2,b_2c_3,b_3c_1,b_3c_3,b_4c_2,b_4c_3\}$. Define $(G,p)$ in $\mathbb{R}^3$ by putting $p(a_1)=(-42, -45, -40)$, $p(a_2)=(44, 48, 
  44)$, $p(b_1)=(9, -1, -7)$, $p(b_2)=(-8, -8, 
  3)$, $p(b_3)=(-1, -4, -5)$, $p(b_4)=(3, -7, 3)$, $p(c_1)=(1, -1, 9)$, $p(c_2)=(-3, -3, -4)$ and $p(c_3)=(-5, -10, -6)$. Given this realisation it is simple for the reader to verify that $(G_i,p)$ is infinitesimally rigid in $\mathbb{R}^3$ and that the unique equilibrium stress of $(G,p)$ has a PSD stress matrix of rank 4. Since $G$ is not globally 3-rigid, it follows that a sufficiently nearby generic framework $(G,q)$ has a rank 4 PSD equilibrium stress.}
	

\begin{figure}[ht]
	\begin{center}
		\begin{tikzpicture}
			\node[vertex] (L1) at (-1,-0.5) {};
			\node[vertex] (L2) at (-1,0.5) {};
			\node[vertex] (C1) at (0,-1) {};
			\node[vertex] (C2) at (0,0) {};
			\node[vertex] (C3) at (0,1) {};
			\node[vertex] (R1) at (1,-1.5) {};
			\node[vertex] (R2) at (1,-0.5) {};
			\node[vertex] (R3) at (1,0.5) {};
			\node[vertex] (R4) at (1,1.5) {};
	
			\draw[edge] (L1)edge(C1);
			\draw[edge] (L1)edge(C2);
			\draw[edge] (L1)edge(C3);
			
			\draw[edge] (L2)edge(C1);
			\draw[edge] (L2)edge(C2);
			\draw[edge] (L2)edge(C3);
			
			\draw[edge] (L1)edge(L2);
			
			\draw[edge] (R1)edge(C1);
			\draw[edge] (R1)edge(C2);
			%\draw[edge] (R1)edge(C3);
			
			\draw[edge] (R2)edge(C1);
			\draw[edge] (R2)edge(C2);
			\draw[edge] (R2)edge(C3);
			
			\draw[edge] (R3)edge(C1);
			\draw[edge] (R3)edge(C2);
			\draw[edge] (R3)edge(C3);
			
			%\draw[edge] (R4)edge(C1);
			%\draw[edge] (R4)edge(C2);
			\draw[edge] (R4)edge(C3);
			
			\draw[edge] (R1)edge(R2);
			\draw[edge] (R2)edge(R3);
			\path[edge] (R3)edge(R4);	
			\path[edge] (R3) edge [bend left] node {} (R1);	
			\path[edge] (R4) edge [bend left] node {} (R2);	
			\path[edge] (R4) edge [bend left] node {} (R1);	
		\end{tikzpicture}\qquad\qquad%
		\begin{tikzpicture}
			\node[vertex] (L1) at (-1,-0.5) {};
			\node[vertex] (L2) at (-1,0.5) {};
			\node[vertex] (C1) at (0,-1) {};
			\node[vertex] (C2) at (0,0) {};
			\node[vertex] (C3) at (0,1) {};
			\node[vertex] (R1) at (1,-1.5) {};
			\node[vertex] (R2) at (1,-0.5) {};
			\node[vertex] (R3) at (1,0.5) {};
			\node[vertex] (R4) at (1,1.5) {};
	
			\draw[edge] (L1)edge(C1);
			\draw[edge] (L1)edge(C2);
			\draw[edge] (L1)edge(C3);
			
			\draw[edge] (L2)edge(C1);
			\draw[edge] (L2)edge(C2);
			\draw[edge] (L2)edge(C3);
			
			\draw[edge] (L1)edge(L2);
			
			\draw[edge] (R1)edge(C1);
			\draw[edge] (R1)edge(C2);
			%\draw[edge] (R1)edge(C3);
			
			\draw[edge] (R2)edge(C1);
			%\draw[edge] (R2)edge(C2);
			\draw[edge] (R2)edge(C3);
			
			\draw[edge] (R3)edge(C1);
			\draw[edge] (R3)edge(C2);
			\draw[edge] (R3)edge(C3);
			
			%\draw[edge] (R4)edge(C1);
			\draw[edge] (R4)edge(C2);
			\draw[edge] (R4)edge(C3);
			
			\draw[edge] (R1)edge(R2);
			\draw[edge] (R2)edge(R3);
			\path[edge] (R3)edge(R4);	
			\path[edge] (R3) edge [bend left] node {} (R1);	
			\path[edge] (R4) edge [bend left] node {} (R2);	
			\path[edge] (R4) edge [bend left] node {} (R1);	
		\end{tikzpicture}%\qquad\qquad%
% 		\begin{tikzpicture}
% 			\node[vertex] (L1) at (-1,-0.5) {};
% 			\node[vertex] (L2) at (-1,0.5) {};
% 			\node[vertex] (C1) at (0,-1) {};
% 			\node[vertex] (C2) at (0,0) {};
% 			\node[vertex] (C3) at (0,1) {};
% 			\node[vertex] (R1) at (1,-1.5) {};
% 			\node[vertex] (R2) at (1,-0.5) {};
% 			\node[vertex] (R3) at (1,0.5) {};
% 			\node[vertex] (R4) at (1,1.5) {};
	
% 			\draw[edge] (L1)edge(C1);
% 			\draw[edge] (L1)edge(C2);
% 			\draw[edge] (L1)edge(C3);
			
% 			\draw[edge] (L2)edge(C1);
% 			\draw[edge] (L2)edge(C2);
% 			\draw[edge] (L2)edge(C3);
			
% 			\draw[edge] (L1)edge(L2);
			
% 			\draw[edge] (R1)edge(C1);
% 			\draw[edge] (R1)edge(C2);
% 			%\draw[edge] (R1)edge(C3);
			
% 			\draw[edge] (R2)edge(C1);
% 			\draw[edge] (R2)edge(C2);
% 			\draw[edge] (R2)edge(C3);
			
% 			%\draw[edge] (R3)edge(C1);
% 			\draw[edge] (R3)edge(C2);
% 			\draw[edge] (R3)edge(C3);
			
% 			%\draw[edge] (R4)edge(C1);
% 			\draw[edge] (R4)edge(C2);
% 			\draw[edge] (R4)edge(C3);
			
% 			\draw[edge] (R1)edge(R2);
% 			\draw[edge] (R2)edge(R3);
% 			\path[edge] (R3)edge(R4);	
% 			\path[edge] (R3) edge [bend left] node {} (R1);	
% 			\path[edge] (R4) edge [bend left] node {} (R2);	
% 			\path[edge] (R4) edge [bend left] node {} (R1);	
% 		\end{tikzpicture}
	\end{center}
	\caption{The only two possible graphs that $G$ can be if every $A$-move gives a graph with minimal degree 3.}
	\label{fig:amove}
\end{figure}

% \begin{figure}[ht]
% 	\begin{center}
% 		\begin{tikzpicture}
% 			\node[vertex] (L1) at (-1,-0.5) {};
% 			\node[vertex] (L2) at (-1,0.5) {};
% 			\node[vertex] (C1) at (0,-1) {};
% 			\node[greenvertex] (C2) at (0,0) {};
% 			\node[greenvertex] (C3) at (0,1) {};
% 			\node[vertex] (R1) at (1,-1.5) {};
% 			\node[greenvertex] (R2) at (1,-0.5) {};
% 			\node[redvertex] (R3) at (1,0.5) {};
% 			\node[redvertex] (R4) at (1,1.5) {};
	
% 			\draw[edge] (L1)edge(C1);
% 			\draw[edge] (L1)edge(C2);
% 			\draw[edge] (L1)edge(C3);
			
% 			\draw[edge] (L2)edge(C1);
% 			\draw[edge] (L2)edge(C2);
% 			\draw[edge] (L2)edge(C3);
			
			
% 			\draw[edge] (L1)edge(L2);
			
			
% 			\path[edge] (C1)edge(C2);
			
			
% 			\draw[edge] (R1)edge(C1);
% 			\draw[edge] (R1)edge(C2);
% 			\draw[edge] (R1)edge(C3);
			
% 			\draw[edge] (R2)edge(C1);
% 			\draw[edge] (R2)edge(C2);
% 			\draw[edge] (R2)edge(C3);
			
% 			\draw[edge] (R3)edge(C2);
% 			\draw[edge] (R3)edge(C3);
			
% 			\draw[edge] (R4)edge(C2);
% 			\draw[edge] (R4)edge(C3);
			
% 			\draw[edge] (R1)edge(R2);
% 			\draw[edge] (R2)edge(R3);
% 			\path[edge] (R3)edge(R4);	
% 			\path[edge] (R4) edge [bend left] node {} (R2);	
			
% 			\node [rectangle,draw=white, fill=white] (a) at (0,-3) {(a)};
% 		\end{tikzpicture}\qquad\qquad%
% 		\begin{tikzpicture}
% 			\node[vertex] (L1) at (-1,-0.5) {};
% 			\node[vertex] (L2) at (-1,0.5) {};
% 			\node[vertex] (C1) at (0,-1) {};
% 			\node[vertex] (C2) at (0,0) {};
% 			\node[vertex] (C3) at (0,1) {};
% 			\node[vertex] (R1) at (1,-1.5) {};
% 			\node[vertex] (R2) at (1,-0.5) {};
% 			\node[vertex] (R3) at (1,0.5) {};
% 			\node[redvertex] (R4) at (1,1.5) {};
	
% 			\draw[edge] (L1)edge(C1);
% 			\draw[edge] (L1)edge(C2);
% 			\draw[edge] (L1)edge(C3);
			
% 			\draw[edge] (L2)edge(C1);
% 			\draw[edge] (L2)edge(C2);
% 			\draw[edge] (L2)edge(C3);
			
			
% 			\draw[edge] (L1)edge(L2);
				
			
% 			\draw[edge] (R1)edge(C1);
% 			\draw[edge] (R1)edge(C2);
% 			\draw[edge] (R1)edge(C3);
			
% 			\draw[edge] (R2)edge(C1);
% 			\draw[edge] (R2)edge(C2);
% 			\draw[edge] (R2)edge(C3);
			
% 			\draw[edge] (R3)edge(C1);
% 			\draw[edge] (R3)edge(C2);
% 			\draw[edge] (R3)edge(C3);
			
% 			\draw[edge] (R4)edge(C3);
			
% 			\draw[edge] (R1)edge(R2);
% 			\draw[edge] (R2)edge(R3);
% 			\path[edge] (R3)edge(R4);	
% 			\path[edge] (R4) edge [bend left] node {} (R1);	
% 			\path[edge] (R4) edge [bend left] node {} (R2);	
% 			%\path[edge] (R4) edge [bend left] node {} (R3);
% 			\path[edge, red] (R3) edge [bend left] node {} (R1);	
			
% 			\node [rectangle,draw=white, fill=white] (b) at (0,-3) {(b)};
% 		\end{tikzpicture}
% 	\end{center}
% 	\caption{(a) A 3-rigid 3-circuit that can be formed by a 3-sum of $K_5$ and $H_3$ (vertices of $K_5$ only in red, vertices of both $K_5$ and $H_3$ in green, vertices of $H_3$ only in black.).
% 	(b) Ignoring the red edge, a 3-rigid 3-circuit that can be formed from the 3-rigid 3-circuit in Figure \ref{fig:3k5s}(b) by a 1-extension.}
% 	\label{fig:k5h3}
% \end{figure}

\begin{figure}[ht]
	\begin{center}
		\begin{tikzpicture}
			\node[vertex] (L1) at (-1,-0.5) {};
			\node[vertex] (L2) at (-1,0.5) {};
			\node[vertex] (C1) at (0,-1) {};
			\node[vertex] (C2) at (0,0) {};
			\node[vertex] (C3) at (0,1) {};
			\node[vertex] (R1) at (1,-1.5) {};
			\node[vertex] (R2) at (1,-0.5) {};
			\node[vertex] (R3) at (1,0.5) {};
			\node[redvertex] (R4) at (1,1.5) {};
	
			\draw[edge] (L1)edge(C1);
			\draw[edge] (L1)edge(C2);
			\draw[edge] (L1)edge(C3);
			
			\draw[edge] (L2)edge(C1);
			\draw[edge] (L2)edge(C2);
			\draw[edge] (L2)edge(C3);
			
			
			\draw[edge] (L1)edge(L2);
				
			
			\draw[edge] (R1)edge(C1);
			\draw[edge] (R1)edge(C2);
			\draw[edge] (R1)edge(C3);
			
			\draw[edge] (R2)edge(C1);
			\draw[edge] (R2)edge(C2);
			\draw[edge] (R2)edge(C3);
			
			\draw[edge] (R3)edge(C1);
			\draw[edge] (R3)edge(C2);
			\draw[edge] (R3)edge(C3);
			
			\draw[edge] (R4)edge(C3);
			
			\draw[edge] (R1)edge(R2);
			\draw[edge] (R2)edge(R3);
			\path[edge] (R3)edge(R4);	
			\path[edge] (R4) edge [bend left] node {} (R1);	
			\path[edge] (R4) edge [bend left] node {} (R2);	
			%\path[edge] (R4) edge [bend left] node {} (R3);
			\path[edge, red] (R3) edge [bend left] node {} (R1);	
			
			\node [rectangle,draw=white, fill=white] (a) at (0,-2) {(a)};
		\end{tikzpicture}\qquad\qquad%
		\begin{tikzpicture}
			\node[vertex] (L1) at (-1,-0.5) {};
			\node[vertex] (L2) at (-1,0.5) {};
			\node[vertex] (C1) at (0,-1) {};
			\node[vertex] (C2) at (0,0) {};
			\node[vertex] (C3) at (0,1) {};
			\node[bluevertex] (R1) at (1,-1.5) {};
			\node[vertex] (R2) at (1,-0.5) {};
			\node[vertex] (R3) at (1,0.5) {};
			\node[redvertex] (R4) at (1,1.5) {};
	
			\draw[edge] (L1)edge(C1);
			\draw[edge] (L1)edge(C2);
			\draw[edge] (L1)edge(C3);
			
			\draw[edge] (L2)edge(C1);
			\draw[edge] (L2)edge(C2);
			\draw[edge] (L2)edge(C3);
			
			
			\draw[edge] (L1)edge(L2);
			
			\path[edge] (C1)edge(C2);
			
			
			\draw[edge] (R1)edge(C1);
			\draw[edge] (R1)edge(C2);
			%\draw[edge] (R1)edge(C3);
			
			\draw[edge,cyan] (R2)edge(C1);
			\draw[edge] (R2)edge(C2);
			\draw[edge] (R2)edge(C3);
			
			\draw[edge] (R3)edge(C1);
			\draw[edge] (R3)edge(C2);
			\draw[edge] (R3)edge(C3);
			
			\draw[edge] (R4)edge(C1);
			%\draw[edge] (R4)edge(C2);
			\draw[edge] (R4)edge(C3);
			
			\draw[edge] (R1)edge(R2);
			\draw[edge] (R2)edge(R3);
			\path[edge] (R3)edge(R4);	
			\path[edge] (R4) edge [bend left] node {} (R2);	
			\path[edge] (R3) edge [bend left] node {} (R1);
			
			
			\path[edge,red] (C1) edge [bend left] node {} (C3);	
			
			\node [rectangle,draw=white, fill=white] (c) at (0,-2) {(b)};
		\end{tikzpicture}\qquad\qquad%
		\begin{tikzpicture}
			\node[vertex] (L1) at (-1,-0.5) {};
			\node[vertex] (L2) at (-1,0.5) {};
			\node[vertex] (C1) at (0,-1) {};
			\node[vertex] (C2) at (0,0) {};
			\node[vertex] (C3) at (0,1) {};
			\node[bluevertex] (R1) at (1,-1.5) {};
			\node[vertex] (R2) at (1,-0.5) {};
			\node[vertex] (R3) at (1,0.5) {};
			\node[redvertex] (R4) at (1,1.5) {};
	
			\draw[edge] (L1)edge(C1);
			\draw[edge] (L1)edge(C2);
			\draw[edge] (L1)edge(C3);
			
			\draw[edge] (L2)edge(C1);
			\draw[edge] (L2)edge(C2);
			\draw[edge] (L2)edge(C3);
			
			
			\draw[edge] (L1)edge(L2);
			
			\path[edge] (C1)edge(C2);
			\path[edge,red] (C2)edge(C3);
			
			\draw[edge] (R1)edge(C1);
			\draw[edge] (R1)edge(C2);
			%\draw[edge] (R1)edge(C3);
			
			\draw[edge] (R2)edge(C1);
			\draw[edge] (R2)edge(C2);
			\draw[edge] (R2)edge(C3);
			
			\draw[edge] (R3)edge(C1);
			\draw[edge] (R3)edge(C2);
			\draw[edge] (R3)edge(C3);
			
			%\draw[edge] (R4)edge(C1);
			\draw[edge] (R4)edge(C2);
			\draw[edge] (R4)edge(C3);
			
			\draw[edge] (R1)edge(R2);
			\draw[edge,cyan] (R2)edge(R3);
			\path[edge] (R3)edge(R4);	
			\path[edge] (R4) edge [bend left] node {} (R2);	
			\path[edge] (R3) edge [bend left] node {} (R1);	
			
			\node [rectangle,draw=white, fill=white] (c) at (0,-2) {(c)};
		\end{tikzpicture}
	\end{center}
	\caption{(a) Ignoring the red edge, a 3-rigid 3-circuit that can be formed from the 3-rigid 3-circuit in Figure \ref{fig:3k5s}(b) by a 1-extension. (b)--(c) Ignoring the red and blue edges, two graphs that can be formed from $H_3$ by two consecutive 1-extensions.}
	\label{fig:amove2}
\end{figure}

Hence, using the handshaking lemma, we may assume that $G$ has an $A$-move that produces a graph $G'$ with minimal degree 4.
%;by the hand-shaking lemma, we know $G'$ cannot have a higher minimal degree.
	If $G'$ is globally 3-rigid the result follows from Theorem \ref{thm: gen ur} and Lemma \ref{lem:1ext},
	so we may suppose $G'$ is not globally 3-rigid.
	By an easy case-by-case check of graphs on 7 vertices with minimum degree 4 and $16 (= 3\cdot 7 -5)$ edges, we see that we must have $G'=H_3$.
	As we are assuming $G$ has no separating set of size 3 with more than 1 edge,
	it follows that $G$ must be one of the three graphs depicted in Figure \ref{fig:amove2};
	we can see this by systematically applying reverse $A$-moves to $H_3$.
% 	Figure \ref{fig:k5h3}(a) is the 3-sum of $K_5$ with $H_3$,
% 	so has a 3-dimensional PSD stress by Lemma \ref{lem: psd clique sum}.
	We can obtain the 3-rigid 3-circuit in Figure~\ref{fig:3k5s}(b) from the graph in Figure~\ref{fig:amove2}(a) by applying a 1-reduction at the red vertex and adding the red edge, hence it will also have a 3-dimensional PSD equilibrium stress by Lemmas~\ref{lem:1ext} and~\ref{lem:d+5circcut}.
	For the other two graphs in Figure \ref{fig:amove2}, we can apply a 1-reduction at the red vertex to add the red edge and then a 1-reduction at the blue vertex that adds the blue edge to obtain $H_3$. Hence Lemmas \ref{lem:1ext} and \ref{lem:d+5circcut} complete the proof.
\end{proof}
The above claims cover all possibilities and hence complete the proof.
\end{proof}




% \begin{figure}[ht]
% 	\begin{center}
% 		\begin{tikzpicture}
% 			\node[vertex] (L1) at (-1,-1) {};
% 			\node[vertex] (L2) at (-1,0) {};
% 			\node[vertex] (L3) at (-1,1) {};
% 			\node[vertex] (C1) at (0,-1) {};
% 			\node[vertex] (C2) at (0,0) {};
% 			\node[vertex] (C3) at (0,1) {};
% 			\node[vertex] (R1) at (1,-1) {};
% 			\node[vertex] (R2) at (1,0) {};
% 			\node[vertex] (R3) at (1,1) {};
	
% 			\draw[edge] (L1)edge(C1);
% 			\draw[edge] (L1)edge(C2);
% 			\draw[edge] (L1)edge(C3);
			
% 			\draw[edge] (L2)edge(C1);
% 			\draw[edge] (L2)edge(C2);
% 			\draw[edge] (L2)edge(C3);
			
% 			\draw[edge] (L3)edge(C1);
% 			\draw[edge] (L3)edge(C2);
% 			\draw[edge] (L3)edge(C3);
			
% 			\draw[edge] (L1)edge(L2);
% 			\draw[edge] (L2)edge(L3);
% 			\path[edge] (L3) edge [bend right] node {} (L1);
			
			
			
% 			\draw[edge] (R1)edge(C1);
% 			\draw[edge] (R1)edge(C3);
			
% 			\draw[edge] (R2)edge(C1);
% 			\draw[edge] (R2)edge(C2);
% 			\draw[edge] (R2)edge(C3);
			
% 			\draw[edge] (R3)edge(C1);
% 			\draw[edge] (R3)edge(C3);
			
% 			\draw[edge] (R1)edge(R2);
% 			\draw[edge] (R2)edge(R3);
% 			\path[edge] (R1) edge [bend right] node {} (R3);
% 		\end{tikzpicture}
% 	\end{center}
% 	\caption{A 3-rigid 3-circuit that can be formed from $K_5$ by a 3-dimensional 0-extension followed by two 3-dimensional 1-extensions.}
% 	\label{fig:cir2}
% \end{figure}


\end{appendix}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Support information, if any,             %%
%% should be provided in the                %%
%% Acknowledgements section.                %%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{acks}[Acknowledgments]
This paper arose as part of the Fields Institute 
Thematic Program on Geometric constraint systems, 
framework rigidity, and distance geometry. LT thanks 
Bill Jackson for discussions about globally rigid $d$-circuits.
\end{acks}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Funding information, if any,             %%
%% should be provided in the                %%
%% funding section.                         %%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{funding}
DIB was partially supported by a Mathematical Sciences
Postdoctoral Research Fellowship from the US NSF, grant DMS-1802902.
SD was partially supported by the Austrian Science Fund (FWF): P31888.
AN was partially supported by the Heilbronn Institute for
Mathematical Research. SJG was partially supported by US NSF grant 
DMS-1564473. MS was partially supported by US
NSF grant DMS-1564480 and US NSF grant DMS-1563234. 

\end{funding}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%                  The Bibliography                       %%
%%                                                         %%
%%  imsart-???.bst  will be used to                        %%
%%  create a .BBL file for submission.                     %%
%%                                                         %%
%%  Note that the displayed Bibliography will not          %%
%%  necessarily be rendered by Latex exactly as specified  %%
%%  in the online Instructions for Authors.                %%
%%                                                         %%
%%  MR numbers will be added by VTeX.                      %%
%%                                                         %%
%%  Use \cite{...} to cite references in text.             %%
%%                                                         %%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%% if your bibliography is in bibtex format, uncomment commands:
\bibliographystyle{imsart-number} % Style BST file (imsart-number.bst or imsart-nameyear.bst)
\bibliography{mltRigid}       % Bibliography file (usually '*.bib')
\end{document}
